A discontinuous Galerkin method for nonlinear biharmonic Schr\"{o}dinger equations

This paper proposes and analyzes a fully discrete scheme that discretizes space with an ultra-weak local discontinuous Galerkin scheme and time with the Crank--Nicolson method for the nonlinear biharmonic Schr\"odinger equation. We first rewrite the problem into a system with a second-order spatial derivative and then apply the ultra-weak discontinuous Galerkin method to the system. The proposed scheme is more computationally efficient compared with the local discontinuous Galerkin method because of fewer auxiliary variables, and unconditionally stable without any penalty terms; it also preserves the mass and Hamiltonian conservation that are important properties of the nonlinear biharmonic Schr\"odinger equation. We also derive optimal L2-error estimates of the semi-discrete scheme that measure both the solution and the auxiliary variable with general nonlinear terms. Several numerical studies demonstrate and support our theoretical findings.

==> Conclusion.tex <==
%!TEX root = fourth_schrodinger.tex
\section{Brief Conclusions and Discussions}\label{conclusion} 
In conclusion, we have developed and analyzed an ultra-weak local DG method for nonlinear biharmonic Schr\"{o}dinger equations.  We extend the LDG scheme and introduce a second-order spatial derivative as an auxiliary variable.  This maneuver reduces the storage for the variables to be solved hence enhances the computational efficiency.  We have proved and demonstrated the stability of the scheme for the special projection operators; moreover, we also obtain optimal $L^2$-error estimates under these settings.  Our numerical experiments demonstrate the theoretical findings and present the rich and complex spatial-temporal dynamics of these linear/nonlinear problems.  A possible and natural future direct can be the extension of the current work to multi-dimensions, there we need to construct special projections to achieve the optimal error estimates; the problems with nonlocal nonlinearity also deserve academic attention.  Finally, one can also try to establish the error estimates for more general numerical fluxes.  We leave all these to future works.  

==> error_estimate.tex <==
%!TEX root = fourth_schrodinger.tex
\section{Error Estimates}\label{sec_error_estimate}
We proceed to derive error estimates of the DG scheme (\ref{DG_scheme1})-(\ref{DG_scheme2}) for the nonlinear biharmonic Schr\"{o}dinger equation (\ref{schrodinger_4th}). In Section \ref{projection}, we review some projections and inequalities that are essential for our proof.  Section \ref{prior} presents the 
{\it a priori} error estimates needed to evaluate the nonlinear terms. The error estimates in the $L^2$-norm are given from Section \ref{initial_error} to Section \ref{error_sec}.  In the estimates, we denote by $C$ a generic positive constant which is independent of $h$ but may vary from line to line.

\subsection{Projections}\label{projection}
Consider the conventional $L^2$-projection $P_h$ into $V_h^q$ such that for any $u\in H^{q+1}(I)$: 
\[\int_{I_j} (P_hu - u)v_h \ dx = 0, \ \ \forall v_h\in \mathcal{P}^q(I_j),\ \ q\geq 0.\]
Let us define the Gauss-Radau projections $P^{\pm}_h$ into $V_h^q$ such that for any $u\in H^{q+1}(I)$ and $q\geq 2$ 
\begin{align}
&\int_{I_j} (P^{\pm}_h u - u)v_h\ dx = 0,\ \ \forall v_h\in \mathcal{P}^{q-2}(I_j),\nonumber\\
& P_h^{+}u(x_{j-\frac{1}{2}}^+) = u(x_{j-\frac{1}{2}}), \ \ (P_h^{+}u)_x(x_{j-\frac{1}{2}}^+) = u_x(x_{j-\frac{1}{2}}),\label{proj1}\\
& P_h^{-}u(x_{j+\frac{1}{2}}^-) = u(x_{j+\frac{1}{2}}), \ \ (P_h^{-}u)_x(x_{j+\frac{1}{2}}^-) = u_x(x_{j+\frac{1}{2}}).\label{proj2}
\end{align}
When $q = 1$, the Gauss--Radau projections are defined only by (\ref{proj1}) and (\ref{proj2}).
For each projection, the following inequality holds (see e.g., \cite{ciarlet2002finite})
\begin{equation}\label{projrel}
\|u - Q_hu\|_{L^2(I_j)} + h\|u - Q_hu\|_{L^\infty(I_j)} + h^{\frac{1}{2}}\|u - Q_hu\|_{L^2(\Gamma_h)} \leq Ch^{q+1},
\end{equation}
where $Q_h = P_h, P^{\pm}_h$, and $\Gamma_h$ denotes the set of boundary points of the element $I_j$.  

\subsection{A priori error estimate}\label{prior} 
Let us denote
\begin{align*}
e_u &= u - u_h = u - P_h^{+} u + P_h^{+} u - u_h =: \eta_u + \xi_u,\\
e_w &= w - w_h = w - P_h^{-} w + P_h^{-} w - w_h =: \eta_w + \xi_w,\\
e_{ut} &= u_t - u_{ht} = u_t - P_h^{+} u_t + P_h^{+} u_t - u_{ht} =: \eta_{ut} + \xi_{ut}.
\end{align*}
To deal with the nonlinearity in problem (\ref{schrodinger_4th}), we make an a priori error estimate assumption %(restrict the following--\textcolor{red}{I have a doubt on this estimate/assumption.  Now $h$ is fixed, how one guarantees this inequality holds for all time $t$? Probably a remark on the global existence or a priori estimates is needed here.)}
\begin{equation}\label{prior3}
\|e_u\|_{L^2(I_j)} +\|e_{ut}\|_{L^2(I_j)} \leq h, 
\end{equation}
which will be verified in Section \ref{verification_priori}.
Further by the inverse inequality, we have
\begin{equation}\label{prior2}
\|e_u\|_{L^\infty(I_j)} +\|e_{ut}\|_{L^\infty(I_j)} \leq C,
\end{equation}
where the constant $C$ depends on the exact solution $u$ and the total time $T$, but not $h$. 
%and this implies that 
%\begin{equation*}\label{prior1}
%\|\xi_u\|_{L^2(I_j)} \leq h, \ \ %\|\xi_{ut}\|_{L^2(I_j)} \leq h.
%\end{equation*}

%\textcolor{red}{The above assumptions can be verified by the optimal error estimates (\ref{error_est}) \cite{chen2019ultra},--I am confused by the logic!}\textcolor{magenta}{and the details will be given in Section \ref{verification_priori}}.


\subsection{Error estimates for initial conditions}\label{initial_error}
This section is devoted to the analysis of the initial error estimates, which plays an essential role in the proof of optimal error estimates of the DG scheme (\ref{DG_scheme1})-(\ref{DG_scheme2}). Motivated by \cite{zhang2021local}, we choose the initial approximation to be the solution of a linear steady-state problem.  We then have the following lemma.

\begin{lemma}\label{lemma1}
Suppose that the numerical initial condition of the DG scheme (\ref{DG_scheme1})-(\ref{DG_scheme2}) is chosen as the DG approximation with numerical fluxes (\ref{fluxa}) to a linear steady-state problem
	\begin{equation}\label{steady_state}
	iu + u_{xxxx} = iu_0 + u_{0xxxx},
	\end{equation}
	where $u_0$ is the initial value of $u$, and periodic boundary conditions are considered. Further, denote $w = u_{xx}$, then the DG approximation for (\ref{steady_state}) is given as
	\begin{multline}\label{DG_schemes1}
	\int_{ I_j}  i u_h\phi + w_h\phi_{xx} - (iu_0 + u_{0xxxx})\phi\ dx\\
	=  -\widetilde{w_{hx}} \phi^-\big|_{j+\frac{1}{2}} + \widetilde{w_{hx}} \phi^+\big|_{j-\frac{1}{2}} + \widetilde{w_h}\phi_x^-\big|_{j+\frac{1}{2}} - \widetilde{w_h}\phi_x^+\big|_{j-\frac{1}{2}}  ,
	\end{multline}
	and
	\begin{equation}\label{DG_schemes2}
	\int_{ I_j}w_h\psi - u_h\psi_{xx}\ dx 
	= \widehat{u_{hx}}\psi^-\big|_{j+\frac{1}{2}} -\widehat{u_{hx}}\psi^+\big|_{j-\frac{1}{2}} - \widehat{u_h}\psi_x^-\Big|_{j+\frac{1}{2}} + \widehat{u_h}\psi_x^+\Big|_{j-\frac{1}{2}},
	\end{equation}
	for all $\phi, \psi \in V_h^q, q\geq1$.
	We then have the following optimal initial error estimates for time-dependent nonlinear Schr\"{o}dinger equation (\ref{schrodinger_4th})
	\begin{equation*}\label{esti_ic}
	\|\xi_u(x,0)\|_{L^2(I)} +\|\xi_{ut}(x,0)\|_{L^2(I)} +  \|\xi_w(x,0)\|_{L^2(I)} \leq Ch^{q+1},
	\end{equation*}
	where $C$ is a positive constant depends on $q$, $\|F'\|_{W^{2,\infty}}$ and $\|u\|_{L^\infty}$, but not $h$.
\end{lemma}

\begin{proof}
Let us consider the DG approximation (\ref{DG_schemes1})-(\ref{DG_schemes2}) for the numerical initial condition first. By the Galerkin orthogonality, we have the error identities 
\begin{align}
&\int_{ I_j}  i e_{u}\phi \ dx + \mathcal{B}_j^1(e_w,\phi) = 0,\label{error_s1}\\
&\int_{I_j} e_w\psi \ dx + \mathcal{B}_j^2(e_u, \psi) = 0,\label{error_s2}
\end{align}
where $e_u = u(x,0) - u_h$ and $e_w = w(x,0) - w_h$,
\begin{equation}
\mathcal{B}_j^1(e_w,\phi) = \int_{I_j} \!e_w\phi_{xx} dx - e_w^-\phi_x^-\big|_{x_{j+\frac{1}{2}}}\! + e_w^-\phi_x^+\big|_{x_{j-\frac{1}{2}}} \!+ e_{wx}^-\phi^-\big|_{x_{j+\frac{1}{2}}} - e_{wx}^-\phi^+\big|_{x_{j-\frac{1}{2}}},\label{B1}
\end{equation}
and
\begin{equation}
\mathcal{B}_j^2(e_u,\psi) = \!\int_{I_j} \!- e_u\psi_{xx}dx - e_{ux}^+\psi^-\big|_{x_{j+\frac{1}{2}}} \!\!+ e_{ux}^+\psi^+\big|_{x_{j-\frac{1}{2}}} \!\!+ e_u^+\psi_x^{-}\big|_{x_{j+\frac{1}{2}}} \!- e_u^+\psi_x^{+}\big|_{x_{j-\frac{1}{2}}}\label{B2}.
\end{equation}
Taking the complex conjugate of (\ref{error_s1})-(\ref{error_s2}) gives
	\begin{align}
	&\int_{ I_j}  -i e_{u}^\ast\phi^\ast \ dx + \mathcal{B}_j^1(e_w^\ast,\phi^\ast) = 0,\label{error_si1}\\
	&\int_{I_j} e_w^\ast\psi^\ast \ dx + \mathcal{B}_j^2(e_u^\ast, \psi^\ast) = 0.\label{error_si2}
	\end{align}
Choosing $\phi = \xi_u^\ast$ in (\ref{error_s1}) and (\ref{error_si1}), $\psi = \xi_w^\ast$ in (\ref{error_s2}) and (\ref{error_si2}), and adding them together, then summing them over all cells $I_j$ yields 
\begin{align}
&\int_{ I_j}  i e_{u}\xi_u^\ast + e_w\xi_w^\ast \ dx+\mathcal{B}_j^1(e_w,\xi_u^\ast) + \mathcal{B}_j^2(e_u, \xi_w^\ast) = 0,\label{e1}\\
&\int_{ I_j}  -i e_{u}^\ast\xi_u + e_w^\ast\xi_w \ dx + \mathcal{B}_j^1(e_w^\ast,\xi_u) + \mathcal{B}_j^2(e_u^\ast, \xi_w) = 0.\label{e2}
\end{align}
Subtracting (\ref{e1}) from (\ref{e2}) gives us
	\begin{multline}\label{ini1}
	2i\sum_j \int_{I_j} |\xi_u|^2  +\mbox{Re}(\eta_u\xi_u^\ast)+  \mbox{Im}(\eta_w\xi_w^\ast)\ dx \\
	+ \sum_j\mathcal{B}_j^1(e_w,\xi_u^\ast)+\mathcal{B}_j^2(e_u,\xi_w^\ast) - \mathcal{B}_j^1(e_w^\ast,\xi_u) - \mathcal{B}_j^2(e_u^\ast,\xi_w) = 0.
	\end{multline}
By property of projection operators (\ref{projrel}) and numerical fluxes (\ref{fluxa}), one reduces (\ref{ini1}) into
	\[2i\sum_j \int_{I_j} |\xi_u|^2  +\mbox{Re}(\eta_u\xi_u^\ast)+  \mbox{Im}(\eta_w\xi_w^\ast)\ dx = 0,\]
and this yields
	\begin{equation}\label{s_est_1}
	\|\xi_u(x,0)\|_{L^2(I)}^2 \leq Ch^{q+1}\left(\|\xi_u(x,0)\|_{L^2(I)} + \|\xi_w(x,0)\|_{L^2(I)}\right).
	\end{equation}
	Similarly, adding (\ref{e1}) and (\ref{e2}) up, and then combining the result with (\ref{projrel}), we infer from the definition of numerical fluxes (\ref{fluxa}) that
	%\begin{equation}
	%\sum_j\int_{I_j}|\xi_w|^2 + 2\mbox{Re}(\eta_w\xi_w^\ast) - 2\mbox{Im}(\eta_u\xi_u^\ast)\ dx = 0,
	%\end{equation}
%which indicates
	\begin{equation}\label{s_est_2}
	\|\xi_w(x,0)\|_{L^2(I)}^2 \leq Ch^{q+1}\left(\|\xi_u(x,0)\|_{L^2(I)} + \|\xi_w(x,0)\|_{L^2(I)}\right).
	\end{equation}
	Combing (\ref{s_est_1})-(\ref{s_est_2}) and using Young's inequality, we obtain
	\begin{equation}\label{s_est_3}
	\|\xi_u(x,0)\|_{L^2(I)} + \|\xi_w(x,0)\|_{L^2(I)} \leq Ch^{q+1}.
	\end{equation}

{Next, we estimate $\|\xi_{ut}(x,0)\|_{L^2(I)}$ by using the relation between the time dependent equation (6) and steady state equation (39).  To this end, we start from the initial error equation for the time-dependent problem (\ref{DG_scheme1})}
	\[\int_{I_j} ie_{ut}\phi\ dx + \mathcal{B}_j^1(e_w,\phi) + \int_{I_j} u F'(|u|^2)\phi - u_hF'(|u_h|^2)\phi\ dx = 0,\]
	where $\mathcal{B}_j^1$ is defined in (\ref{B1}).
	Subtracting this identity from (\ref{error_s1}) gives
	\[\int_{I_j} ie_{ut}\phi - ie_{u}\phi + u F'(|u|^2)\phi - u_hF'(|u_h|^2)\phi\ dx = 0.\]
	Choosing $\phi = \xi_{ut}^\ast$ and summing it over all cells $I_j$, we arrive at
	\begin{equation}\label{i_xiut}
	\int_{I} |\xi_{ut}|^2\ dx = \sum_j\int_{I_j} -\eta_{ut}\xi_{ut}^\ast + e_u\xi_{ut}^\ast +i\left(u F'(|u|^2)\xi_{ut}^\ast - u_hF'(|u_h|^2)\xi_{ut}^\ast\right)\ dx.
	\end{equation}
For the right-hand side, we apply the property (\ref{projrel}) of the projection operator $P_h^+$ and (\ref{s_est_3}) to estimate
\begin{equation}\label{e11}
		\Big|\sum_j\int_{I_j} -\eta_{ut}(x,0)\xi_{ut}^\ast(x,0) + e_u(x,0)\xi_{ut}^\ast(x,0)\ dx\Big| \leq Ch^{q+1}\|\xi_{ut}(x,0)\|_{L^2(I)},
		\end{equation}
while for the nonlinear terms we have from the Taylor expansion that
 \begin{equation}\label{taylor}
 F'(|u_h|^2) = F'(|u|^2) + F''(|u|^2)\gamma+ \frac{1}{2}F'''(|\hat{u}|^2)\gamma^2,
 \end{equation}
 where $|\hat{u}|^2$ is between $|u|^2$ and $|u_h|^2$, and
 \begin{equation}\label{gamma}
 \gamma := |u_h|^2 - |u|^2  = u_hu_h^{\ast} - uu^\ast = (u - e_u)(u^\ast- e_u^\ast) - uu^\ast = |e_u|^2 - 2\mbox{Re}(u^\ast e_u).
 \end{equation}
 
 Finally, we obtain
 \begin{align}
 &\Big|\sum_j\int_{I_j} i\left(u F'(|u|^2) - u_hF'(|u_h|^2)\right)\xi_{ut}^\ast\ dx\Big|\nonumber\\
 \leq &  \Big|\sum_j\int_{I_j} u\left(-F''(|u|^2)\gamma - \frac{1}{2}F'''(|\hat{u}|^2)\gamma^2\right)\xi_{ut}^\ast\ dx\Big|\nonumber\\
 &+ \Big|\sum_j\int_{I_j} e_u\left(F'(|u|^2) + F''(|u|^2)\gamma + \frac{1}{2}F'''(|\hat{u}|^2)\gamma^2\right)\xi_{ut}^\ast\ dx\Big|\nonumber\\
 \leq & Ch^{q+1}\|\xi_{ut}(x,0)\|_{L^2(I)},\label{e12}
 \end{align}
where $C$ is dependent of $\|F'\|_{W^{2,\infty}(I)}$, $\|u\|_{L^\infty(I)}$, but not $h$. Finally, combining (\ref{i_xiut}), (\ref{e11}) with (\ref{e12}) yields $\|\xi_{ut}(x,0)\|_{L^2(I)} \leq Ch^{q+1}$, and this completes the proof.
\end{proof}

%\textcolor{red}{Any remarks?} \textcolor{magenta}{No} \textcolor{red}{Fine, but it is always not a bad to remark/comment/rephrase/explain your mathematical results whenever they are available} \textcolor{magenta}{Let us leave it here this time, I don't know how to comment here ...}

\subsection{Optimal error estimates for $t > 0$}\label{error_sec}
We are now ready to present error estimates for the DG scheme (\ref{DG_scheme1})-(\ref{DG_scheme2}) with the numerical fluxes (\ref{fluxa}).  In particular, we shall show that the estimates are optimal in $L^2$-norm.
\begin{truth}\label{them2}
Let $(u,w)$ be a smooth solution of system (\ref{system_2nd}), and $(u_h, w_h)\in V^q_h\times V_h^q, q\geq1$ be the numerical solution of the DG scheme (\ref{DG_scheme1})-(\ref{DG_scheme2}) with the smooth initial data computing by (\ref{steady_state}) along with periodic boundary conditions and the numerical fluxes (\ref{fluxa}), then we have the following error estimates :
	\begin{equation}\label{error_est}
	\|e_u(x,T)\|_{L^2(I)} + \|e_w(x,T)\|_{L^2(I)} + \|e_{ut}(x,T)\|_{L^2(I)} \leq Ch^{q+1},
	\end{equation}
	where $C$ is a positive constant that depends on $q$, $\|F'\|_{W^{3,\infty}}$, $\|u\|_{L^\infty}$, $\left|\left|u_t\right|\right|_{L^\infty}$ and $T$, but not $h$.
\end{truth}
\begin{proof}
Our proof consists of three steps: i) the estimate of $d\|\xi_u\|_{L^2(I_j)}/dt$, ii) the estimate of $d\|\xi_w\|_{L^2(I_j)}/dt$, and iii) the estimate of $d\|\xi_{ut}\|_{L^2(I_j)}/dt$.
	
\textbf{Step one}: %estimate of $d\|\xi_u\|_{L^2(I_j)}/dt$. 
By the DG scheme (\ref{DG_scheme1}) and the Galerkin orthogonality, we have the following for any $(\phi,\psi) \in V_h^q\times V_h^q$
	\begin{align}
	&i\int_{I_j} e_{ut} \phi\ dx+ \int_{I_j}uF'(|u|^2)\phi - u_hF'(|u_h|^2)\phi\ dx + \mathcal{B}_j^1(e_w,\phi) = 0,\label{erroru1}\\
	&\int_{I_j} e_w\psi \ dx  + \mathcal{B}_j^2(e_u,\psi) = 0 ,\label{erroru2}
	\end{align}
where $\mathcal{B}_j^1$ and $\mathcal{B}_j^2$ are defined in (\ref{B1}) and (\ref{B2}), respectively.  In light of (\ref{erroru1})-(\ref{erroru2}), we obtain 
	\begin{align}
	&i\int_{I_j} e_{ut}^\ast \phi^\ast\ dx -\int_{I_j} u^\ast F'(|u|^2)\phi^\ast - u_h^{\ast}F'(|u_h|^2)\phi^\ast\ dx - \mathcal{B}_j^1(e_w^\ast,\phi^\ast) = 0,\label{erroru1i}\\
	&-\int_{I_j} e_w^\ast\psi^\ast \ dx  - \mathcal{B}_j^2(e_u^\ast,\psi^\ast) = 0.\label{erroru2i}
	\end{align}
Then choosing $\phi = \xi_u^\ast$ and $\psi = \xi_w^\ast$ in (\ref{erroru1})-(\ref{erroru2i}), adding them together and summing over all cells $I_j$ yields
	%\begin{multline}\label{error_sum}
	%i\sum_j\int_{I_j} e_{ut}\xi_{u}^\ast + e_{ut}^\ast\xi_u \ dx + \int_{I_j} uF'(|u|^2)\xi_u^\ast -u^\ast F'(|u|^2)\xi_u\ dx+ \mathcal{B}_j^2(e_u,\xi_w^\ast) \\- \mathcal{B}_j^2(e_u^\ast, \xi_w) - \int_{I_j} u^\ast F'(|u_h|^2)\xi_u - u_h^{\ast}F'(|u_h|^2)\xi_u \ dx + \mathcal{B}_j^1(e_w,\xi_u^\ast) - \mathcal{B}_j^1(e_w^\ast,\xi_u) = 0.
	%\end{multline}
	\begin{equation}\label{xiu}
	\frac{d}{dt}\sum_j\int_{I_j} |\xi_u|^2\ dx = \Lambda_1 + \Lambda_2 + \Lambda_3,
	\end{equation}
	where we have used the relations $e_u = \eta_u + \xi_u$, $e_w = \eta_w + \xi_w$, and
	\begin{align*}
	\Lambda_1 &=: \sum_j\int_{I_j} -2\mbox{Re}(\eta_{ut}\xi_u^\ast) \  - 2\mbox{Im}(\eta_w\xi_w^\ast)dx,\\
	\Lambda_2 &=: i\sum_j \mathcal{B}_j^2(e_u,\xi_w^\ast) - \mathcal{B}_j^2(e_u^\ast,\xi_w) + \mathcal{B}_j^1(e_w,\xi_u^\ast) - \mathcal{B}_j^1(e_w^\ast,\xi_u), \\
	\Lambda_3 &=: \sum_j\int_{I_j} -2F'(|u|^2)\mbox{Im}(u\xi_u^\ast)  +  2F'(|u_h|^2)\mbox{Im}(u_h\xi_u^\ast),
	\end{align*}
 are to be estimated separately.
	
	From the property (\ref{projrel}) of the projection operators, we get
	\begin{equation}\label{lambda1}
	|\Lambda_1| \leq Ch^{q+1} \big(\|\xi_u\|_{L^2(I)} + \|\xi_w\|_{L^2(I)}\big),
	\end{equation}
	and the same analysis as in Theorem \ref{them1} leads us to 
	\begin{equation}\label{lambda2}
	|\Lambda_2| = 0.
	\end{equation}
	To estimate $\Lambda_3$, we first rewrite it as
	\begin{equation*}
	\Lambda_3 = -2\sum_j \big(F'(|u|^2) -F'(|u_h|^2) \big)\mbox{Im}(u\xi_u^\ast) +F'(|u_h|^2)\mbox{Im}(e_u\xi_u^\ast).
	\end{equation*}
	It can be further rewritten as follows thanks to (\ref{taylor}) and (\ref{gamma}) 
	\begin{equation*}
	\Lambda_3 = 2(\Lambda_{31} + \Lambda_{32} ),
	\end{equation*}
	where
	\[\Lambda_{31} = \sum_j \int_{I_j}\Big( F''(|u|^2)\gamma
	+ \frac{1}{2}F'''(|\hat{u}|^2)\gamma^2\Big)\mbox{Im}(u\xi_u^\ast)\ dx \]
	and
	\[\Lambda_{32} = -\sum_j\int_{I_j}\Big(F'(|u|^2) + F''(|u|^2)\gamma+ \frac{1}{2}F'''(|\hat{u}|^2)\gamma^2\Big)\mbox{Im}(e_u\xi_u^\ast)\ dx.\]
	We first have 
	\[\int_{I_j}\!\! |\gamma\mbox{Im}(u\xi_u^\ast)|  dx \leq C\left(\|u\|_{L^\infty(I_j)} \|e_u\|_{L^\infty(I_j)} + \|u\|^2_{L^\infty(I_j)}\!\right)\left(\|\xi_u\|_{L^2(I_j)}^2 + \|\eta_u\|_{L^2(I_j)}^2\!\right),\]
	hence
	\begin{multline*}
	\Lambda_{31} \!\leq\! C\Big(\|F''\|_{L^\infty(I_j)} + \|\gamma\|_{L^\infty(I_j)}\|F'''\|_{L^\infty(I_j)}\Big)\cdot\\
	\left(\|u\|_{L^\infty(I_j)} \|e_u\|_{L^\infty(I_j)} + \|u\|^2_{L^\infty(I_j)}\!\right)
	\Big(\|\xi_u\|_{L^2(I)}^2 + \|\eta_u\|_{L^2(I)}^2\Big).
	\end{multline*}
	
	On the other hand, we have $\mbox{Im}(e_u\xi_u^\ast)  = \mbox{Im}(\eta_u\xi_u^\ast)$ since $\xi_u\xi_u^\ast = |\xi_u|^2$ is a real number, then 
	\begin{equation*}
	\Lambda_{32} \leq\! C\Big(\!\|F'\|_{L^\infty(I)}\!+ \|\gamma\|_{L^\infty(I)}\|F''\|_{L^\infty(I)} \!+ \|\gamma^2\|_{L^\infty(I)}\|F'''\|_{L^\infty(I)}\!\Big)\Big(\|\xi_u\|_{L^2(I)}^2 \!+\! \|\eta_u\|_{L^2(I)}^2\Big).
	\end{equation*}
	
Combining the bounds of $\Lambda_{31}$ and $\Lambda_{32}$ derived above, we obtain
\begin{align}\label{lambda31}
\Lambda_3 \leq C&\Bigg(\left(\|F''\|_{L^\infty(I_j)} + \|\gamma\|_{L^\infty(I_j)}\|F'''\|_{L^\infty(I_j)}\right)\cdot \left(\|u\|_{L^\infty(I_j)} \|e_u\|_{L^\infty(I_j)} + \|u\|^2_{L^\infty(I_j)}\!\right)\\ &+\|F'\|_{L^\infty(I)}+\|\gamma\|_{L^\infty(I)}\|F''\|_{L^\infty(I)} + \|\gamma^2\|_{L^\infty(I)}\|F'''\|_{L^\infty(I)}\Bigg)\cdot\Big(\|\xi_u\|_{L^2(I)}^2 + \|\eta_u\|_{L^2(I)}^2\Big),\nonumber
\end{align}
% 	\begin{multline}
% 	\Lambda_3 \leq C\Bigg(\left(\|F''\|_{L^\infty(I_j)} + \|\gamma\|_{L^\infty(I_j)}\|F'''\|_{L^\infty(I_j)}\right)\cdot \\\left(\|u\|_{L^\infty(I_j)} \|e_u\|_{L^\infty(I_j)} + \|u\|^2_{L^\infty(I_j)}\!\right) + \|F'\|_{L^\infty(I)}+\|\gamma\|_{L^\infty(I)}\|F''\|_{L^\infty(I)} \\+ \|\gamma^2\|_{L^\infty(I)}\|F'''\|_{L^\infty(I)}\Bigg)\Big(\|\xi_u\|_{L^2(I)}^2 + \|\eta_u\|_{L^2(I)}^2\Big),
% 	\end{multline}
	

% 	\begin{multline}\label{lambda31}
% 	\Lambda_3 \leq C\Bigg(\left(\|F''\|_{L^\infty(I_j)} + \|\gamma\|_{L^\infty(I_j)}\|F'''\|_{L^\infty(I_j)}\right)\cdot \\\left(\|u\|_{L^\infty(I_j)} \|e_u\|_{L^\infty(I_j)} + \|u\|^2_{L^\infty(I_j)}\!\right) + \|F'\|_{L^\infty(I)}+\|\gamma\|_{L^\infty(I)}\|F''\|_{L^\infty(I)} \\+ \|\gamma^2\|_{L^\infty(I)}\|F'''\|_{L^\infty(I)}\Bigg)\Big(\|\xi_u\|_{L^2(I)}^2 + \|\eta_u\|_{L^2(I)}^2\Big),
% 	\end{multline}
while from the a prior estimation (\ref{prior2}), we further get
\begin{equation}\label{gammae}
\|\gamma\|_{L^\infty(I)} \leq C\left(1+\|u\|_{L^\infty(I)}\right),\ \ \|\gamma^2\|_{L^2(\infty)} \leq C\left(1 + \|u\|_{L^\infty(I)} + \|u\|^2_{L^\infty(I)}\right).
\end{equation}
Then we have from (\ref{gammae}) and (\ref{lambda31}) that
\begin{equation}\label{lambda3}
|\Lambda_3| \leq C \Big(\|\xi_u\|_{L^2(I)}^2 + \|\eta_u\|_{L^2(I)}^2\Big),
\end{equation}
where $C$ depends on $\|F'\|_{W^{2,\infty}}$ and $\|u\|_{L^\infty(I)}$, but not $h$. Finally, plugging (\ref{lambda1}), (\ref{lambda2}) and (\ref{lambda3}) into (\ref{xiu}) and using Young's inequality, we have
	\begin{equation}\label{xiut}
	\frac{d}{dt}\|\xi_u\|_{L^2(I)}^2 \leq C\Big(\|\xi_u\|_{L^2(I)}^2 + \|\xi_w\|_{L^2(I)}^2 + h^{2(q+1)} \Big).
	\end{equation}
	
\textbf{Step two}: % estimate of $d\|\xi_w\|_{L^2(I_j)}/dt$. 
We differentiate (\ref{DG_scheme2}) against time and obtain for any $(\phi, \psi) \in V_h^q\times V_h^q$ that
\begin{align}
&i\int_{I_j} e_{ut} \phi\ dx+ \int_{I_j}uF'(|u|^2)\phi - u_hF'(|u_h|^2)\phi\ dx + \mathcal{B}_j^1(e_w,\phi) = 0,\label{errorw1}\\
&\int_{I_j} e_{wt}\psi \ dx  + \mathcal{B}_j^2(e_{ut},\psi) = 0 ,\label{errorw2}
\end{align}
where $\mathcal{B}_j^1$ and $\mathcal{B}_j^2$ are defined in (\ref{B1}) and (\ref{B2}), respectively. Taking the complex conjugate of (\ref{errorw1})-(\ref{errorw2}) gives us 
	\begin{align}
	&-i\int_{I_j} e^\ast_{ut} \phi^\ast\ dx+ \int_{I_j}u^\ast F'(|u|^2)\phi^\ast - u_h^{\ast}F'(|u_h|^2)\phi^\ast\ dx + \mathcal{B}_j^1(e_w^\ast,\phi^\ast) = 0,\label{errorw1i}\\
	&\int_{I_j} e^\ast_{wt}\psi^\ast \ dx  + \mathcal{B}_j^2(e^\ast_{ut},\psi^\ast) = 0 .\label{errorw2i}
	\end{align}
	Setting $\phi = \xi_{ut}^\ast$, $\psi = \xi_w^\ast$ in (\ref{errorw1})-(\ref{errorw2i}) and summing them all together over all cells $I_j$ gives
	%\begin{multline*}\label{sum2}
	%\sum_ji\int_{I_j} e_{ut} \xi_{ut}^\ast - e_{ut}^\ast \xi_{ut}\ dx + \int_{I_j} e_{wt}\xi_w^\ast + e_{wt}^\ast\xi_w \ dx  \\
	%+ \int_{I_j}uF'(|u|^2)\xi_{ut}^\ast - u_hF'(|u_h|^2)\xi_{ut}^\ast + u^\ast F'(|u|^2)\xi_{ut} - u_h^{\ast}F'(|u_h|^2)\xi_{ut}\ dx \\+ \mathcal{B}_j^1(e_w,\xi_{ut}^\ast) + \mathcal{B}_j^1(e^\ast_w,\xi_{ut})+ \mathcal{B}_j^2(e_{ut},\xi_w^\ast) + \mathcal{B}_j^2(e^\ast_{ut},\xi_w) = 0.
	%\end{multline*}
	\begin{equation}\label{xiw}
	\frac{d}{dt} \sum_j \int_{I_j} |\xi_w|^2\ dx = \Theta_1 + \Theta_2 + \Theta_3,
	\end{equation}
	where we use the relations $e_u = \eta_u + \xi_u$, $e_w = \eta_w + \xi_w$ and denote
	\begin{align*}
	\Theta_1 &:= \sum_j\int_{I_j} -2\mbox{Im}(\eta_{ut}^\ast\xi_{ut}) - 2\mbox{Re}(\eta_{wt}^\ast\xi_w)\ dx,\\
	\Theta_2 &:= -\sum_j \mathcal{B}_j^1(e_w,\xi_{ut}^\ast) + \mathcal{B}_j^1(e^\ast_w,\xi_{ut})+ \mathcal{B}_j^2(e_{ut},\xi_w^\ast) + \mathcal{B}_j^2(e^\ast_{ut},\xi_w),\\
	\Theta_3 &:= -\sum_j \int_{I_j}2F'(|u|^2)\mbox{Re}(u\xi_{ut}^\ast) - 2F'(|u_h|^2)\mbox{Re}(u_h\xi_{ut}^\ast)\ dx. 
	\end{align*}
	By similar analysis as in step one, we get
	\[|\Theta_2| = 0, \ \ 
	|\Theta_1| \leq Ch^{q+1}\Big(\|\xi_{ut}\|_{L^2(I)} + \|\xi_w\|_{L^2(I)}\Big),\]
	and 
	\[|\Theta_3| \leq C \Big(\|\xi_{ut}\|_{L^2(I)}^2 +\|\xi_{u}\|_{L^2(I)}^2 + \|\eta_u\|_{L^2(I)}^2\Big).\] 
	Plugging the above equality and inequalities into (\ref{xiw}) and using Young's inequality, we have
	\begin{equation}\label{xiwt}
	\frac{d}{dt}\|\xi_w\|_{L^2(I)}^2 \leq C\Big(\|\xi_u\|_{L^2(I)}^2 +\|\xi_{ut}\|_{L^2(I)}^2+ \|\xi_w\|_{L^2(I)}^2 + h^{2(q+1)} \Big).
	\end{equation}
	 Note that $\|\xi_{ut}\|_{L^2(I)}^2$ appears in (\ref{xiwt}) and it is unknown. To get the estimate of $d\|\xi_w\|_{L^2(I)}^2/dt$, we need to establish an inequality regarding $\|\xi_{ut}\|_{L^2(I)}^2$. 
	
	\textbf{Step three} : an inequality for $d\|\xi_{ut}\|_{L^2(I)}^2/dt$. Taking the time derivative of (\ref{DG_scheme1})-(\ref{DG_scheme2}) we get the following error equations
	\begin{align}
	&i\int_{I_j} e_{utt} \phi\ dx+ \int_{I_j}\frac{d}{dt}\Big(uF'(|u|^2)\phi - u_hF'(|u_h|^2)\Big)\phi\ dx + \mathcal{B}_j^1(e_{wt},\phi) = 0,\label{errorut1}\\
	&\int_{I_j} e_{wt}\psi \ dx  + \mathcal{B}_j^2(e_{ut},\psi) = 0 ,\label{errorut2}
	\end{align}
	for any $(\phi,\psi) \in V^q_h\times V^q_h$, and $\mathcal{B}_j^1$, $\mathcal{B}_j^2$ are defined in (\ref{B1}) and (\ref{B2}), respectively.
	 Multiplying (\ref{errorut1})-(\ref{errorut2}) by $-1$ and taking their complex conjugate, we obtain
	\begin{align}
	&i\!\!\int_{I_j} e_{utt}^\ast \phi^\ast\ dx \!-\!\!\int_{I_j} \frac{d}{dt}\Big(u^\ast F'(|u|^2)\phi^\ast - u_h^{\ast}F'(|u_h|^2)\phi^\ast\Big)\ dx - \mathcal{B}_j^1(e_{wt}^\ast,\phi^\ast) = 0,\label{errorut1i}\\
	&-\int_{I_j} e_{wt}^\ast\psi^\ast \ dx  - \mathcal{B}_j^2(e_{ut}^\ast,\psi^\ast) = 0.\label{errorut2i}
	\end{align}
	Further, choosing $\phi = \xi_{ut}^\ast$, $\psi = \xi_{wt}^\ast$ in (\ref{errorut1})-(\ref{errorut2i}), adding them together and summing over all cells $I_j$, we have
	%\begin{multline}\label{errort_sum}
	%\sum_ji\int_{I_j} e_{utt}\xi_{ut}^\ast + e_{utt}^\ast\xi_{ut} \ dx + \int_{I_j} \eta_{wt}\xi_{wt}^\ast - \eta_{wt}^\ast\xi_{wt}\ dx\\+ \int_{I_j} \frac{d}{dt}\Big(uF'(|u|^2) -u_h F'(|u_h|^2)\Big)\xi_{ut}^\ast\ dx - \int_{I_j} \frac{d}{dt}\Big(u^\ast F'(|u|^2) - u_h^{\ast}F'(|u_h|^2)\Big)\xi_{ut} \ dx \\+ \mathcal{B}_j^1(e_{wt},\xi_{ut}^\ast) - \mathcal{B}_j^1(e_{wt}^\ast,\xi_{ut})+ \mathcal{B}_j^2(e_{ut},\xi_{wt}^\ast) - \mathcal{B}_j^2(e_{ut}^\ast, \xi_{wt}) = 0.
	%\end{multline}
	\begin{equation}\label{errorut}
	\frac{d}{dt}\sum_j\int_{I_j} |\xi_{ut}|^2\ dx = W_1 + W_2 + W_3 + W_4,
	\end{equation}
	where we have used the relations $e_u = \eta_u + \xi_u$, $e_w = \eta_w + \xi_w$, and
	\begin{align*}
	W_1  &:= \sum_j\int_{I_j} -2\mbox{Re}(\eta_{utt}\xi_{ut}^\ast) \ dx,\\
	W_2 &:= i\sum_j \mathcal{B}_j^2(e_{ut},\xi_{wt}^\ast) - \mathcal{B}_j^2(e_{ut}^\ast,\xi_{wt}) + \mathcal{B}_j^1(e_{wt},\xi_{ut}^\ast) - \mathcal{B}_j^1(e_{wt}^\ast,\xi_{ut}), \\
	W_3 &:= i\sum_j \!\!\int_{I_j}\frac{d}{dt}\Big(uF'(|u|^2) \!-\! u_hF'(|u_h|^2)\Big)\xi_{ut}^\ast \!-\! \frac{d}{dt}\Big(u^\ast F'(|u|^2) \!-\! u_h^{\ast}F'(|u_h|^2)\Big)\xi_{ut} \ dx,\\
	W_4  &:= -\sum_j\int_{I_j}  2\mbox{Im}(\eta_{wt}\xi_{wt}^\ast)dx,
	\end{align*}
	which will be estimated separately. By a similar analysis as in step one, we have
	\begin{equation}\label{w2}    
    |W_1| \leq Ch^{q+1} \|\xi_{ut}\|_{L^2(I)}, \text{~and~}
    |W_2| = 0.
	\end{equation}
	 
	To estimate $W_3$, we first rewrite it as
	\begin{equation*}
	W_3 = -2(W_{31} + W_{32}),
	\end{equation*}
	where
\[W_{31}= \sum_j\int_{I_j}\big(F'(|u|^2)-F'(|u_h|^2)\big)\mbox{Im}(u_t\xi_{ut}^\ast) + F'(|u_h|^2)\mbox{Im}(e_{ut}\xi_{ut}^\ast)\ dx,\]
and
\begin{multline*}
W_{32} = \sum_j\int_{I_j}\left(F''(|u|^2)\frac{d|u|^2}{dt}-F''(|u_h|^2)\frac{d|u_h|^2}{dt}\right)\mbox{Im}(u\xi_{ut}^\ast) +F''(|u_h|^2)\frac{d|u_h|^2}{dt}\mbox{Im}(e_u\xi_{ut}^\ast)\ dx.
\end{multline*}
 
The same analysis that leads to $\Lambda_3$ gives rise to
\begin{equation*}
	W_{31} \leq C
	\Big(\|\xi_u\|_{L^2(I)}^2 + \|\xi_{ut}\|_{L^2(I)}^2+ \|\eta_u\|_{L^2(I)}^2 + \|\eta_{ut}\|_{L^2(I)}^2\Big).
	\end{equation*}
%where $C$ depends on $\|f\|_{W^{2,\infty}}$ with $f = F'$, $\|u\|_{L^\infty(I)}$, and $\|\frac{du}{dt}\|_{L^\infty(I)}$ but independent of $h$.

To estimate $W_{32}$, we find for some $|\hat{u}|^2$ between $|u|^2$ and $|u_h|^2$ that
\[F''(|u_h|^2) = F''(|u|^2) + F'''(|u|^2)\gamma+ \frac{1}{2}F^{(4)}(|\hat{u}|^2)\gamma^2,\]
where $\gamma$ is defined in (\ref{gamma}); moreover, we divide $W_{32}$ into two parts as
	\begin{equation}\label{w32}
	W_{32} = W_{32}^{(1)} + W_{32}^{(2)}, 
	\end{equation}
where
	\begin{equation*}
	W_{32}^{(1)} \!:=\!\! \sum_j\!\!\int_{I_j}\!\!\!\Bigg(\!\!-F''(|u|^2)\frac{d\gamma}{dt}-\left(\!\!F'''(|u|^2)\gamma \!+\! \frac{1}{2}F^{(4)}(|\hat{u}|^2)\gamma^2\!\right)
	\left(\!\frac{d|u|^2}{dt}\!+\!\frac{d\gamma}{dt}\right)\!\!\Bigg)\mbox{Im}(u\xi_{ut}^\ast)\ dx,
	\end{equation*}
	\begin{equation*}
	W_{32}^{(2)}\!: =\! \sum_{j}\int_{I_j}\left(F''(|u|^2) + F'''(|u|^2)\gamma + \frac{1}{2}F^{(4)}(|\hat{u}|^2)\gamma^2\right)\left(\frac{d|u|^2}{dt}+\frac{d\gamma}{dt}\right)\mbox{Im}(e_u\xi_{ut}^\ast)\ dx.
	\end{equation*}
In light of the definition of $\gamma$ and estimate (\ref{prior2}), we obtain
	\begin{multline}\label{w311}
	|W_{32}^{(1)}| \leq C\Bigg(\|F''\|_{L^\infty(I)}\Big(1+\|u\|_{L^\infty(I)}+\left|\left|\frac{du}{dt}\right|\right|_{L^\infty(I)}\Big)+\|F'''\|_{L^\infty(I)}\\ \left(1+\|u\|_{L^\infty(I)}\right)+\|F^{(4)}\|_{L^\infty(I)}\|\gamma\|_{L^\infty(I)}\left(1+\|u\|_{L^\infty(I)}\right)\Bigg)\|u\|_{L^\infty(I)}\\
	\cdot\left(\left|\left|\frac{d|u|^2}{dt}\right|\right|_{L^\infty(I)} \!\!+\left|\left|\frac{d\gamma}{dt}\right|\right|_{L^\infty(I)}  \right)
	\left(\|\xi_{ut}\|_{L^2(I)}^2 +\|\xi_u\|_{L^2(I)}^2 + \|\eta_u\|_{L^2(I)}^2+\|\eta_{ut}\|_{L^2(I)}^2\right),
	\end{multline}
	and
	\begin{multline}\label{w312}
	|W_{32}^{(2)}| \leq C\left(\|F''\|_{L^\infty(I)}+\|F'''\|_{L^\infty(I)}\|\gamma\|_{L^\infty(I)}+\|F^{(4)}\|_{L^\infty(I)}\|\gamma^2\|_{L^\infty(I)}\right)\\
	\cdot\left(\left|\left|\frac{d|u|^2}{dt}\right|\right|_{L^\infty(I)} + \left|\left|\frac{d\gamma}{dt}\right|\right|_{L^\infty(I)}\right)
	\left(\|\xi_{u}\|^2_{L^2(I)} + \|\xi_{ut}\|_{L^2(I)}^2 +\|\eta_u\|_{L^2(I)}^2 \right).
	\end{multline}
	In addition, in light of the definition of $\gamma$ in (\ref{gamma}) and estimate (\ref{prior2}), we have
	\begin{equation}\label{gammate}
	\left|\left|\frac{d\gamma}{dt}\right|\right|_{L^\infty(I)} \leq C\left(1 + \|u\|_{L^\infty(I)} + \left|\left|\frac{du}{dt}\right|\right|_{L^\infty(I)}\right).
	\end{equation}
	Plugging (\ref{gammae}) and (\ref{gammate}) into (\ref{w311})-(\ref{w312}), we apply (\ref{w32}) to obtain
	\begin{equation}\label{w3}
	|W_3| \leq C\left(\|\xi_{u}\|^2_{L^2(I)} + \|\xi_{ut}\|_{L^2(I)}^2+h^{2(q+1)}\right),
	\end{equation}
	where $C$ is a positive constant which depends on $\|F'\|_{W^{3,\infty}(I)}$, $\|u\|_{L^\infty(I)}$, and $\left|\left|\frac{d u}{d t}\right|\right|_{L^\infty(I)}$, but not $h$. 
	Substituting (\ref{w2})-(\ref{w3}) into (\ref{errorut}) and using Young's inequality, we obtain
	\begin{equation}\label{xiut1}
	\frac{d}{dt} \|\xi_{ut}\|_{L^2(I)}^2 \leq C\left(\|\xi_{u}\|^2_{L^2(I)} + \|\xi_{ut}\|_{L^2(I)}^2+h^{2(q+1)}\right) + |W_4|.
	\end{equation}
	Collecting (\ref{xiut}), (\ref{xiwt}) and (\ref{xiut1}) leads us to
	\begin{multline*}
	\frac{d}{dt}\left(\|\xi_{u}\|_{L^2(I)}^2 +\|\xi_{w}\|_{L^2(I)}^2 +\|\xi_{ut}\|_{L^2(I)}^2 \right)  \\ \leq C \left(\|\xi_{u}\|_{L^2(I)}^2 +\|\xi_{w}\|_{L^2(I)}^2+ \|\xi_{ut}\|_{L^2(I)}^2 \right) + Ch^{2(q+1)} + |W_4|.
	\end{multline*}
    Now, we integrate this inequality from $0$ to $T$ to find that
\begin{align}\label{final1}
&\|\xi_{u}(x,T)\|_{L^2(I)}^2 +\|\xi_{w}(x,T)\|_{L^2(I)}^2 +\|\xi_{ut}(x,T)\|_{L^2(I)}^2 \nonumber\\  
\leq& \|\xi_{u}(x,0)\|_{L^2(I)}^2 +\|\xi_{w}(x,0)\|_{L^2(I)}^2 +\|\xi_{ut}(x,0)\|_{L^2(I)}^2 \nonumber\\
&+ C\int_0^T \|\xi_{u}\|_{L^2(I)}^2 +\|\xi_{w}\|_{L^2(I)}^2+ \|\xi_{ut}\|_{L^2(I)}^2\  dt + Ch^{2(q+1)} + \int_0^T |W_4|\ dt.     
\end{align}    

For $\int_0^T |W_4| dt$, we have from the integration by parts in time that
	\begin{align}\label{w4}
	&\int_0^T |W_4|\ dt = \sum_j\int_{I_j}\int_0^T |2\mbox{Im}(\eta_{wt}\xi_{wt}^\ast)|dt dx \\
	 \leq& \sum_j\int_{I_j} \Big(\big|2\mbox{Im}(\eta_{wt}(x,T)\xi_{w}^\ast(x,T))\big| + \big|2\mbox{Im}(\eta_{wt}(x,0)\xi_{w}^\ast(x,0))\big|+ Ch^{2(q+1)} + C\int_0^T \|\xi_{w}\|_{L^2(I)}^2dt\Big)\ dx.\nonumber
	\end{align}
	Plugging (\ref{w4}) into (\ref{final1}), we invoke Young's inequality and Lemma \ref{lemma1} to find 
	\begin{align}\label{final2}
	&\|\xi_{u}(x,T)\|_{L^2(I)}^2 +\|\xi_{w}(x,T)\|_{L^2(I)}^2 +\|\xi_{ut}(x,T)\|_{L^2(I)}^2\nonumber\\
\leq& C\int_0^T \|\xi_{u}\|_{L^2(I)}^2 +\|\xi_{w}\|_{L^2(I)}^2+ \|\xi_{ut}\|_{L^2(I)}^2\  dt + Ch^{2(q+1)} + \frac{1}{2}\|\xi_w(x,T)\|_{L^2(I)}^2.
	\end{align}
	Finally, applying Gronwall's inequality to (\ref{final2}) gives rise to
	\[\|\xi_{u}(x,T)\|_{L^2(I)}^2 +\|\xi_{w}(x,T)\|_{L^2(I)}^2 +\|\xi_{ut}(x,T)\|_{L^2(I)}^2 \leq Ch^{2(q+1)},\]
 and this collects the error estimate (\ref{error_est}) thanks to the triangle inequality and the property {(\ref{projrel})} of Gauss--Radau projection.
\end{proof}

\begin{remark}
{\color{red}For the case $F'(\vert u\vert^2) \equiv \mbox{constant}$, one can obtain the same error estimates without assuming (\ref{prior3}). %Here, we use the estimation of $\Lambda_3$ in (\ref{xiu}) as an example. Let $u_s := su + (1-s)u_h$, we obtain
%\begin{equation*}
%\begin{aligned}
%\vert\Lambda_3\vert = & \big\vert\sum_j\int_{I_j} -\vert u\vert^{2\sigma}(u\xi_u^\ast - u^\ast \xi_u)  +  \vert u_h\vert^{2\sigma}(u_h\xi_u^\ast - u_h^\ast\xi_u) \ dx\big\vert\\
%\leq &\big\vert\sum_j\int_{I_j} \int_0^1 \frac{d}{ds}\left(|u_s|^{2\sigma}u_s\right)ds\ \xi_u^\ast \ dx \big\vert + \big\vert\sum_j\int_{I_j} \int_0^1 \frac{d}{ds}\left(|u_s^\ast|^{2\sigma}u_s^\ast\right)ds\ \xi_u \ dx \big\vert  \\
%\leq & (2\sigma+1)\Big(\sum_j\int_{I_j}\int_0^1 \vert u_s\vert^{2\sigma}\vert u-u_h\vert ds\ \vert\xi_u^\ast\vert\ dx\big\vert + \sum_j\int_{I_j}\int_0^1 \vert u_s^\ast\vert^{2\sigma}\vert u^\ast-u_h^\ast\vert ds\ \vert\xi_u\vert\ dx \Big)\\
%= & (2\sigma+1)\Big(\sum_j\int_{I_j}\vert u + (1-\hat{s})(\eta_u+\xi_u)\vert^{2\sigma} \vert \eta_u + \xi_u\vert \vert\xi_u\vert \\
%& + \vert u^\ast + (1-\hat{s})(\eta_u^\ast+\xi_u^\ast)\vert^{2\sigma} \vert \eta_u^\ast + \xi_u^\ast\vert \vert\xi_u\vert\Big)\ dx \\
%\leq & (2\sigma+1)\Big(\|u+(1-\hat{s})(\eta_u+\xi_u)\|_{L^\infty(I)}^{2\sigma} (\|\eta_u\|_{L^2(I)} +\|\xi_u\|_{L^2(I)} )\|\xi_u^\ast\|_{L^2(I)} \\
%& + \|u^\ast+(1-\hat{s})(\eta_u^\ast+\xi_u^\ast)\|_{L^\infty(I)}^{2\sigma} (\|\eta_u^\ast\|_{L^2(I)} +\|\xi_u^\ast\|_{L^2(I)} )\|\xi_u\|_{L^2(I)}\Big)\\
%\leq & C\big(1 + h^{-\sigma}\|\xi_u\|_{L^2(I)}^{2\sigma}\big)\big(h^{k+1} + \|\xi_u\|_{L^2(I)}\big)\|\xi_u\|_{L^2(I)} 
%\end{aligned}
%\end{equation*}	
%
}
\end{remark}

\subsection{Verification of the a priori error estimate} \label{verification_priori}
We are now left to verify the a priori error estimate assumption (\ref{prior3}).  To see this, we first find that 
(\ref{prior3}) is true at $t = 0$ thanks to Lemma \ref{them1}.  To show it for all $t>0$, we argue by contradiction. Suppose that (\ref{prior3}) fails before $T$, there exist some $t_\ast\in(0,T)$ such that $t_\ast = \mbox{inf}\{t:\Vert(u - u_h)(\cdot,t)\Vert_{L^2(I)}  + \Vert(u_t - u_{ht})(\cdot,t)\Vert_{L^2(I)} > h\}$.
By the continuity of $\|(u-u_h)(\cdot,t)\|_{L^2(I)} + \|(u_t-u_{ht})(\cdot,t)\|_{L^2(I)}$, we have $h = \|(u - u_h )(\cdot,t_\ast )\|_{L^2(I)} + \|(u_t - u_{ht})(\cdot,t_\ast )\|_{L^2(I)}$. On the other hand, $(\ref{prior3})$ holds for $0 \leq t \leq t_\ast$, thus from Theorem \ref{them2}, we have $\|(u - u_h)(\cdot,t_\ast )\|_{L^2(I)} +  \|(u_t - u_{ht})(\cdot,t_\ast )\|_{L^2(I)}\leq Ch^{q+1}$
, which is a contradiction if $q \geq 1$. Therefore, we have $\|(u - u_h)(\cdot,t)\|_{L^2(I)}  + \|(u_t - u_{ht})(\cdot,t)\|_{L^2(I)}\leq h$ for all $0 \leq t \leq T$. Now we have completed the verification of (\ref{prior3}). % \textcolor{blue}{Suppose that (\ref{prior3}) fails before $T$, then there exists a (finite or infinite) sequence $\{t_n\}\subset(0,T)$ such that $\Vert(u - u_h)(\cdot,t_n)\Vert_{L^2} > h$ for each $n$.  Let us denote $t_*:=\inf\{t_n\}$}.


	 
	 
	 

==> formulations.tex <==


%!TEX root = fourth_schrodinger.tex
\section{Semi-discrete DG Formulation and Stability}\label{sec_formula}
We choose $\kappa = 1$ in (\ref{problem}) and consider on the following nonlinear biharmonic Schr\"{o}dinger equation  
\begin{equation}\label{schrodinger_4th}
i u_{t}  + u_{xxxx}  = - uF'(|u|^2) ,\quad { x}\in I = (x_a,x_b),\quad t\geq 0,
\end{equation}
coupled with initial and periodic boundary conditions.  This choice is made for demonstration simplicity and the DG method developed here applies to the cases when $\kappa$ takes other values; moreover, our scheme cooperates with general boundary conditions, while the error estimates in Section \ref{sec_error_estimate} requires different technical tools and might become more complicated. We further assume that $F(|u|^2) \geq 0$ to guarantee the positivity of the Hamiltonian associated with (\ref{schrodinger_4th}).%In this work, we only work on the periodic boundary conditions.

To derive a DG formulation for (\ref{schrodinger_4th}), we denote $w: = u_{xx}$ and collect the following second-order system
\begin{equation}\label{system_2nd}
\left\{
\begin{aligned}
iu_t & = -w_{xx} - uF'(|u|^2), \\
 w &=  u_{xx}.
\end{aligned}
\right.
\end{equation}
Note that any solution to (\ref{system_2nd}) formally satisfies the conservation of mass and Hamiltonian
\[{M(t)=M(0),\ \  H(t)=H(0),\ \ \forall t>0},\]
where the mass and Hamiltonian are given by
\[M(t):= \int_I |u|^2\ dx,\quad \text{and}\quad H(t) := \int_I |w|^2 + F(|u|^2) \ dx.\]

%\begin{align}
%M(t) & := \int_I |u|^2\ dx,\label{mass}\\
%H(t) & := \int_I |w|^2 + F(|u|^2) \ dx. \label{energy}
%\end{align}


\subsection{Semi-discrete DG formulation}\label{semi_form}
We first present the DG scheme for (\ref{schrodinger_4th}) through the reformulation (\ref{system_2nd}).  Discretize the domain $I$ by non-overlapping cells $I_j$ such that 
\[I = \cup_j I_j = \cup_j(x_{j-\frac{1}{2}}, x_{j+\frac{1}{2}}), \ \ j = 1,\cdots,n,\]
where
\[x_{\frac{1}{2}} = x_a, \ x_{n+\frac{1}{2}} = x_b, \ x_j = \frac{1}{2}(x_{j-\frac{1}{2}} + x_{j+\frac{1}{2}}), \ h_j = x_{j+\frac{1}{2}} - x_{j-\frac{1}{2}}, \ h = \max_j{h_j},\]
and a mesh regularity $\frac{h}{\min h_j} < {\beta}$ is applied throughout the paper with $\beta>0$ being fixed during the mesh refinement.  On each element $I_j$, we approximate $(u,w)$ by $(u_h, w_h)$, each belonging to the following space of piecewise polynomial of degree $q (\geq1)$ 
\[V_h^q: = \{v_h(x, t), v_h(x, t)\in\mathcal{P}^q( I_j), x\in I_j, t\geq 0\}.\]
Let us further denote
\[\eta^{\pm}(x) := \lim_{\epsilon\rightarrow 0^{\pm}}\eta(x + \epsilon),\]
and introduce the conventional notations for averages and jumps
\[\{v_h\} = \frac{1}{2}(v_h^- + v_h^+), \ \ [v_h] = v_h^- - v_h^+.\]

To seek approximation of the second-order system, on each element $ I_j$ we choose test functions $\phi, \psi \in V_h^q$ and apply them to the first and the second equation in (\ref{system_2nd}), respectively.  An integration by parts leads us to the following integral systems
\begin{equation}\label{DG_scheme1}
\int_{ I_j}  i u_{ht}\phi + w_h\phi_{xx} + u_hF'(|u_h|^2)\phi\ dx 
=  -\widetilde{w_{hx}} \phi^-\big|_{j+\frac{1}{2}} + \widetilde{w_{hx}} \phi^+\big|_{j-\frac{1}{2}} + \widetilde{w_h}\phi_x^-\big|_{j+\frac{1}{2}} - \widetilde{w_h}\phi_x^+\big|_{j-\frac{1}{2}}  ,
\end{equation}
and
\begin{equation}\label{DG_scheme2}
\int_{ I_j}w_h\psi - u_h\psi_{xx}\ dx 
= \widehat{u_{hx}}\psi^-\big|_{j+\frac{1}{2}} -\widehat{u_{hx}}\psi^+\big|_{j-\frac{1}{2}} - \widehat{u_h}\psi_x^-\Big|_{j+\frac{1}{2}} + \widehat{u_h}\psi_x^+\Big|_{j-\frac{1}{2}} ,
\end{equation}
where $\widetilde{w_{hx}}$, $\widetilde{w_h}$, $\widehat{u_{hx}}$ and $\widehat{u_h}$ are numerical fluxes at cell boundaries.  {Note that $q = 0$ is not an option as it yields inconsistency in the scheme}. %Note that (\ref{DG_scheme1}) and (\ref{DG_scheme2}) can be rewritten equivalently in weak formulations by performing another integration by parts back as
%\begin{multline*}
%\int_{ I_j}  i u_{ht}\phi - w_{hx}\phi_{x} + u_hF'(|u_h|^2)\phi\ dx \\
%=  -\widetilde{w_x} \phi^-\big|_{j+\frac{1}{2}} + \widetilde{w_x} \phi^+\big|_{j-\frac{1}{2}} + (\widetilde{w}-w_h^-)\phi_x^-\big|_{j+\frac{1}{2}} - (\widetilde{w}-w^{h,+})\phi_x^+\big|_{j-\frac{1}{2}}  ,
%\end{multline*}
%and
%\begin{multline*}
%\int_{ I_j}w_h\psi + u_{hx}\psi_{x}\ dx \\
%= \widehat{u_x}\psi^-\big|_{j+\frac{1}{2}} -\widehat{u_x}\psi^+\big|_{j-\frac{1}{2}} - (\widehat{u}-u_h^-)\psi_x^-\Big|_{j+\frac{1}{2}} + (\widehat{u}-u_h^-)\psi_x^+\Big|_{j-\frac{1}{2}}.
%\end{multline*}
Based on the periodic boundary condition, we sum up over all cells $I_j$ for the DG schemes (\ref{DG_scheme1}) and (\ref{DG_scheme2}) and collect
\begin{align*}
\mathcal{A}_1(u_h, w_h, \phi)  + \int_I u_hF'(|u_h|^2)\phi\ dx &= 0,\\
\mathcal{A}_2(u_h,w_h,\psi) &= 0,
\end{align*}
where
\begin{align}
\mathcal{A}_1(u_h, w_h, \phi) &:= \int_I iu_{ht} \phi + w_h\phi_{xx} \ dx + \sum_j \left(\widetilde{w_{hx}}[\phi] - \widetilde{w_h}[\phi_x]\right)\big|_{j+\frac{1}{2}},\label{A1}\\
\mathcal{A}_2(u_h, w_h, \psi) &:= \int_I w_h\psi - u_h\psi_{xx}\ dx - \sum_j \left(\widehat{u_{hx}}[\psi] - \widehat{u_h}[\psi_x]\right)\big|_{x_{j+\frac{1}{2}}}.\label{A2}
\end{align}

To complete the DG formulations, we specify the numerical fluxes $\widetilde{w_{hx}}$, $\widetilde{w_h}$, $\widehat{u_{hx}}$ and $\widehat{u_h}$ at the cell boundaries by choosing
\begin{equation}\label{flux1}
\widehat{u_h} = \alpha_1 u_h^+ + (1-\alpha_1) u_h^-, \ \widetilde{w_{hx}} = (1-\alpha_1)w_{hx}^+ + \alpha_1 w_{hx}^-,
\end{equation}
and
\begin{equation}\label{flux2}
\widehat{u_{hx}} = \alpha_2 u_{hx}^+ + (1-\alpha_2) u_{hx}^-,\ \widetilde{w_h} = (1-\alpha_2) w_h^+ + \alpha_2 w_h^-, 
\end{equation}
where $0\leq \alpha_1, \alpha_2 \leq 1$.  In particular, when $\alpha_1 = 0 \ \mbox{or} \ 1$, $\alpha_2 = 0 \ \mbox{or} \ 1$, we have the alternating fluxes that are also compatible with the error estimates in Sections \ref{initial_error} and \ref{error_sec}. For simplicity of analysis, we only consider the following alternating fluxes with $\alpha_1 = \alpha_2 = 1$ in (\ref{flux1}) and (\ref{flux2})
\begin{equation}\label{fluxa}
\widehat{u_h} = u_h^+,\ \ \widetilde{w_{hx}} =  w_{hx}^-, \ \ \widehat{u_{hx}} =  u_{hx}^+ ,\ \ \widetilde{w_h} = w_h^-.
\end{equation}
Howerver, the error analysis can be easily generated to other types of alternating fluxes.

\subsection{Energy conservation}\label{sec:conservation}
We now prove that the proposed scheme formulated in (\ref{DG_scheme1})-(\ref{DG_scheme2}) conserves both the discrete mass and the discrete Hamiltonian.  In particular, we show that they imply stability of the scheme as follows.

\begin{truth}\label{them1}
	(Stability) The solution of the DG scheme (\ref{DG_scheme1})-(\ref{DG_scheme2}) with numerical fluxes (\ref{flux1})-(\ref{flux2}) satisfies the following conservation laws
	\begin{align}
	M_h(t) &= \int_I |u_h|^2\ dx = M_h(0),\label{M}\\
	H_h(t) &= \int_I |w_h|^2 + F(|u_h|^2) \ dx = H_h(0).\label{E}
	\end{align}
\end{truth}
\begin{proof}
Let us first prove the mass conservation.  To this end, we choose $\phi = u_h^\ast$ in (\ref{DG_scheme1}) and $\psi = w_h^\ast$ in (\ref{DG_scheme2}), where ``$\ast$'' represents the complex conjugate.  Summing (\ref{DG_scheme1}) multiplied by $-i$ and (\ref{DG_scheme2}) multiplied by $i$ up over all cells $I_j$, we obtain
	\begin{align}
		-i\mathcal{A}_1(u_h, w_h, u_h^\ast) - i\int_I |u_h|^2F'(|u_h|^2) \ dx &= 0,\label{eq1}\\
		i\mathcal{A}_2(u_h, w_h, w_h^\ast) & = 0,\label{eq2}
	\end{align}
	where $\mathcal{A}_1$ and $\mathcal{A}_2$ are defined in (\ref{A1}) and (\ref{A2}), respectively.  We apply an integration by parts and find
\begin{equation}\label{A11}
-i\mathcal{A}_1(u_h, w_h, u_h^\ast) = \int_I u_{ht}u_h^\ast + iw_{hx}u_{hx}^\ast \ dx -i \sum_j \left(\widetilde{w_{hx}}[u_h^\ast] - \widetilde{w_h}[u_{hx}^\ast] +[w_hu_{hx}^*] \right)\big|_{j+\frac{1}{2}},
\end{equation}
and
\begin{equation}\label{A21}
i\mathcal{A}_2(u_h, w_h, w_h^\ast) = \int_Ii w_h w_h^\ast +iu_{hx}w_{hx}^\ast\ dx -i\sum_j \left(\widehat{u_{hx}}[w_h^\ast] - \widehat{u_h}[w_{hx}^\ast] + [u_hw_{hx}^\ast]\right)\big|_{x_{j+\frac{1}{2}}}.
 \end{equation}

Then, computing the complex conjugate of (\ref{eq1})-(\ref{eq2}) and adding them with the resulting two equations, we arrive at
\begin{align}\label{eq5}
0 =& i\int_I |u_h|^2F'(|u_h|^2) \ dx - i\int_I |u_h|^2F'(|u_h|^2) \ dx\nonumber\\
=& -i\mathcal{A}_1(u_h, w_h, u_h^\ast) + i\mathcal{A}_1(u_h^\ast, w_h^\ast, u_h)  + i\mathcal{A}_2(u_h, w_h, w_h^\ast) -i\mathcal{A}_2(u_h^\ast, w_h^\ast, w_h) \\
=& \frac{d}{dt}\int_I |u_h|^2 dx + 2\mbox{Im}\sum_j \left(\widetilde{w_{hx}}[u_h^\ast] - \widetilde{w_h}[u_{hx}^\ast] +[w_hu_{hx}^*]\right)\big|_{j+\frac{1}{2}} \nonumber\\
&+ 2\mbox{Im}\sum_j\left(\widehat{u_{hx}}[w_h^\ast] - \widehat{u_h}[w_{hx}^\ast] + [u_hw_{hx}^\ast]\right)\big|_{j+\frac{1}{2}}, \nonumber   
\end{align}
% \begin{multline}\label{eq5}
% 0 =  i\int_I |u_h|^2F'(|u_h|^2) \ dx - i\int_I |u_h|^2F'(|u_h|^2) \ dx\\
% = -i\mathcal{A}_1(u_h, w_h, u_h^\ast) \\+ i\mathcal{A}_1(u_h^\ast, w_h^\ast, u_h)  
% + i\mathcal{A}_2(u_h, w_h, w_h^\ast) -i\mathcal{A}_2(u_h^\ast, w_h^\ast, w_h) \\
% = \frac{d}{dt}\int_I |u_h|^2 dx + 2\mbox{Im}\sum_j \left(\widetilde{w_x}[u_h^\ast] - \widetilde{w}[u_{hx}^\ast] +[w_hu_{hx}^*]\right)\big|_{j+\frac{1}{2}} \\
% + 2\mbox{Im}\sum_j\left(\widehat{u_x}[w_h^\ast] - \widehat{u}[w_{hx}^\ast] + [u_hw_{hx}^\ast]\right)\big|_{j+\frac{1}{2}},
% 	\end{multline}
where we have used (\ref{A11})-(\ref{A21}) to derive the third identity.  Further, by using the fact
	\begin{equation}\label{fact1}
	[ab] = \big((1-\alpha) a^- + \alpha a^+ \big) [b] + \big((1-\alpha) b^+ + \alpha b^- \big)[a],\ \ \alpha \in [0,1],
	\end{equation}
	we get
\begin{align}\label{eq3}
K_1:
=& \sum_j \left([w_hu_{hx}^*]+\widehat{u_{hx}}[w_h^\ast] - \widetilde{w_h}[u_{hx}^\ast] \right)\big|_{j+\frac{1}{2}} \nonumber\\
=&\sum_j \Big(\big(\alpha_2w_h^- + (1-\alpha_2)w_h^+\big)[u_{hx}^\ast] + \big((1-\alpha_2)u_{hx}^{-,\ast} + \alpha_2u_{hx}^{+,\ast}\big)[w_h] \nonumber\\
 &+\big(\alpha_2u_{hx}^+ + (1-\alpha_2)u_{hx}^-\big)[w_h^\ast]- \big((1-\alpha_2)w_h^+ + \alpha_2 w_h^-\big)[u_{hx}^\ast]\Big)\Big|_{j+\frac{1}{2}} \nonumber\\
=& \sum_j 2\mbox{Re}\Big(\big((1-\alpha_2)u_{hx}^- + \alpha_2u_{hx}^+\big)[w_h^\ast] \Big)\Big|_{j+\frac{1}{2}},
\end{align}
	and
	\begin{equation}\label{eq4}
	K_2 \!:=\! \sum_j\! \left([u_hw_{hx}^\ast]+\widetilde{w_{hx}}[u_h^\ast] - \widehat{u_h}[w_{hx}^\ast] \right)\big|_{j+\frac{1}{2}}
	\!=\! \sum_j 2\mbox{Re}\Big(\big((1-\alpha_1)w_{hx}^+ + \alpha_1w_{hx}^-\big)[u_h^\ast] \Big)\Big|_{j+\frac{1}{2}}.
	\end{equation}
These identities indicate both $K_1$ and $K_2$ are real numbers. Plugging (\ref{eq3})-(\ref{eq4}) into (\ref{eq5}) leads to
	\[\frac{d}{dt}\int_I |u_h|^2\ dx = 0,\]
	which yields the mass conservation (\ref{M}). 
	
To prove the Hamiltonian conservation (\ref{E}), we differentiate (\ref{DG_scheme2}) against time and obtain
	\begin{equation}\label{DG_scheme2t}
	\int_{ I_j}w_{ht}\psi - u_{ht}\psi_{xx}\ dx 
	= \widehat{u_{htx}}\psi^-\big|_{j+\frac{1}{2}} -\widehat{u_{htx}}\psi^+\big|_{j-\frac{1}{2}} - \widehat{u_{ht}}\psi_x^-\Big|_{j+\frac{1}{2}} + \widehat{u_{ht}}\psi_x^+\Big|_{j-\frac{1}{2}}.
	\end{equation}
Thanks to the periodic boundary condition, summing (\ref{DG_scheme2t}) over all cells $I_j$ gives
	\[\mathcal{A}_2(u_{ht}, w_{ht}, \psi) = 0,\]
where $\mathcal{A}_2$ is defined in (\ref{A2}). Now, by choosing $\phi = u_{ht}^\ast$ in (\ref{DG_scheme1}), $\psi = w_h^\ast$ in (\ref{DG_scheme2t}) and summing them over all cells $I_j$, respectively, we get
\begin{align}
		\mathcal{A}_1(u_h,w_h,u_{ht}^\ast) + \int_I u_hF'(|u_h|^2)u_{ht}^\ast\ dx &= 0,\label{A13}\\
		\mathcal{A}_2(u_{ht}, w_{ht}, w_h^\ast) & = 0,\label{A23}
\end{align} 
where $\mathcal{A}_1$ is defined in (\ref{A1}).  Moreover, we integrate by parts and have
\begin{equation}\label{A12}
\mathcal{A}_1(u_h, w_h, u_{ht}^\ast)= \int_I iu_{ht}u_{ht}^\ast - w_{hx}u_{htx}^\ast \ dx + \sum_j \left(\widetilde{w_{hx}}[u_{ht}^\ast] - \widetilde{w_h}[u_{htx}^\ast] +[w_hu_{htx}^\ast] \right)\big|_{j+\frac{1}{2}}, 
\end{equation}
and 
\begin{equation}\label{A22}
\mathcal{A}_2(u_{ht}, w_{ht}, w_h^\ast)= \int_I w_{ht} w_h^\ast +u_{htx}w_{hx}^\ast\ dx
-\sum_j \left(\widehat{u_{htx}}[w_h^\ast] - \widehat{u_{ht}}[w_{hx}^\ast] + [u_{ht}w_{hx}^\ast]\right)\big|_{x_{j+\frac{1}{2}}}
\end{equation}

% \begin{align}
% 	\mathcal{A}_1(u_h, w_h, u_{ht}^\ast) &= \int_I iu_{ht}u_{ht}^\ast - w_{hx}u_{htx}^\ast \ dx \label{A12}\\
% 	&\hspace{1cm}+ \sum_j \left(\widetilde{w_x}[u_{ht}^\ast] - \widetilde{w}[u_{htx}^\ast] +[w_hu_{htx}^\ast] \right)\big|_{j+\frac{1}{2}},	\nonumber\\
% 	\mathcal{A}_2(u_{ht}, w_{ht}, w_h^\ast) &= \int_I w_{ht} w_h^\ast +u_{htx}w_{hx}^\ast\ dx \label{A22}\\
% 	&\hspace{1cm}-\sum_j \left(\widehat{u_{tx}}[w_h^\ast] - \widehat{u_t}[w_{hx}^\ast] + [u_{ht}w_{hx}^\ast]\right)\big|_{x_{j+\frac{1}{2}}}\nonumber.
% 	\end{align}

Then, computing the complex conjugate of (\ref{A13})-(\ref{A23}) and adding them together yields
\begin{align}\label{dG}
\frac{d}{dt}\int_I F(|u_h|^2)+ |w_h|^2\ dx 
=&- 2\mbox{Re}\sum_j  \left(\widetilde{w_{hx}}[u_{ht}^\ast] - \widetilde{w_h}[u_{htx}^\ast] +[w_hu_{htx}^\ast] \right)\big|_{j+\frac{1}{2}}\nonumber\\
&+ 2\mbox{Re}\sum_j\left(\widehat{u_{htx}}[w_h^\ast] - \widehat{u_{ht}}[w_{hx}^\ast] + [u_{ht}w_{hx}^\ast]\right)\big|_{x_{j+\frac{1}{2}}},    
\end{align}
where we have used (\ref{A12})-(\ref{A22}).
Using identity (\ref{fact1}) and the numerical fluxes (\ref{flux1})-(\ref{flux2}), we have
\begin{align}\label{eq6}
K_3:=&\sum_j \left([w_hu_{htx}^\ast]-\widetilde{w_h}[u_{htx}^\ast] - \widehat{u_{htx}}[w_h^\ast] \right)\big|_{j+\frac{1}{2}}\nonumber\\
=& -2i\sum_j \mbox{Im}\Big(\big((1-\alpha_2)u_{htx}^- + \alpha_2u_{htx}^+\big)[w_h^\ast] \Big)\Big|_{j+\frac{1}{2}},
\end{align}
and
\begin{align}\label{eq7}
K_4 :=& \sum_j \left(-[u_{ht}w_{hx}^\ast]+\widetilde{w_{hx}}[u_{ht}^\ast] + \widehat{u_{ht}}[w_{hx}^\ast] \right)\big|_{j+\frac{1}{2}}\nonumber\\
	=& 2i\sum_j \mbox{Im}\Big(\big((1-\alpha_1)w_{hx}^+ + \alpha_1w_{hx}^-\big)[u_{ht}^\ast] \Big)\Big|_{j+\frac{1}{2}}.
\end{align}
Again, these identities indicate both $K_3$ and $K_4$ are pure imaginary numbers.  Finally, substituting (\ref{eq6}) and (\ref{eq7}) into (\ref{dG}) leads us to 
\[\frac{d}{dt}\int_I F(|u_h|^2)+ |w_h|^2\ dx = 0,\]
and this collects the Hamiltonian conservation (\ref{E}).
\end{proof}




==> introduction.tex <==


%!TEX root = fourth_schrodinger.tex
\section{Introduction}
Nonlinear biharmonic Schr\"{o}dinger equations arise commonly from the study of the propagation of intense laser beams, quantum mechanics, nonlinear optical fibers, propagation of electromagnetic beams in plasma, and many other applications (see \cite{lam1977self, agrawal2000nonlinear, ben2000dispersion, cui2007well,karpman1996stabilization, karpman2000stability, pausader2009cubic} and references therein). In this paper, we consider the nonlinear biharmonic Schr\"{o}dinger equations over an interval 
\begin{equation}\label{problem}
iu_{t} + \kappa u_{xxxx} + uF'(|u|^2) = 0, \ \ (x,t)\in (x_a,x_b)\times(0,T], 
\end{equation}
with periodic boundary condition and initial condition $u(x,0) = u_0(x)$, where $u(x,t)$ is a complex function of space-time variable $(x,t)$ with $|u|$ being its {Euclidean length}, {$i = \sqrt{-1}$ is the imaginary number}, % the subscripts ``$t$" and ``$x$" represent the derivatives with respective to $t$ and $x$, respectively, 
$F'(y) = \frac{dF}{dy}$ is a real function that measures the medium nonlinearity, and $\kappa$ is a real constant {dependent on the physical relevance}. Problem (\ref{problem}) is a special case, $\zeta = 0$, of the nonlienar Schr\"{o}dinger equation with high-order dispersion term (\ref{full_problem}).
\begin{equation}\label{full_problem}
iu_{t} + \zeta u_{xx} + \kappa u_{xxxx} + uF'(|u|^2) = 0. 
\end{equation}
Problem (\ref{full_problem}) was introduced in \cite{karpman1996stabilization,karpman2000stability} to take into account the role of small fourth-order dispersion terms in the propagation of intense laser beams in a bulk medium.  There are many researchers in the past a few years concerned with local and global well-posedness and formation of singularities for both problem (\ref{problem}) and (\ref{full_problem}). For example, when $\kappa < 0$ and $F'(|u|^2) = |u|^{2\sigma}$ with $\sigma$ being a positive integer. \cite{karpman1996stabilization,karpman2000stability} have shown that the waveguide solutions of equation (\ref{full_problem}) are stable for all $\kappa < 0$ when $\sigma \leq 2$ and also stable for $\kappa \ll -1$ when $2 <\sigma<4$, but unstable for all $\kappa < 0$ when $\sigma \geq 4$. (\ref{problem}) admits a very similar result with (\ref{full_problem}), \cite{ilan2002self, baruch2011singular} proved that for $\kappa > 0$, (\ref{problem}) with $F'(|u|^2) = |u|^{2\sigma}$ is defocusing and exists globally, but when $\kappa < 0$, it is focusing and there exists a critical exponent $\sigma = 4$ that determines the blow-ups and global existence subject to the ($L^2$) size of the initial data. 

This paper presents and analyzes a fully discrete ultra-weak local discontinuous Galerkin scheme with the Crank--Nicolson time discretization for the nonlinear biharmonic Schr\"{o}dinger equation (\ref{problem}). The proposed scheme is implicit in time, unconditionally stable and preserves the mass and Hamiltonian associated with the problem at a discrete level.
 
 Before proceeding further, we want to note that various numerical methods have been proposed to solve nonlinear Schr\"{o}dinger equations (\ref{full_problem}) for $\kappa = 0$ in literature, such as the finite difference methods \cite{akrivis1993finite,chang1995finite,besse2004relaxation,bao2013optimal}, the time-splitting pseudospectral methods \cite{bao2003numerical,robinson1993numerical,pathria1990pseudo}, the finite element methods \cite{akrivis1991fully,karakashian1999space,dag1999quadratic} and the discontinuous Galerkin (DG) methods \cite{xu2012optimal, chen2019ultra, zhang2021local}, just to name a few.  However, very few numerical methods consider problem (\ref{full_problem}) with $\kappa \neq 0$ in the literature.  Xiao et al. \cite{xiao2019conservative} propose a conservative linearly-implicit difference scheme for the modified Zakharov system.  This method has a high-order space fractional quantum correction but it converges only second order in space.  Zhang and Su \cite{zhang2021conservative} improve the convergence of this method to fourth order in space by developing an linearly implicit compact difference scheme for Quantum Zakharov System.  Baruch et al. \cite{baruch2010singular,baruch2010ring} investigate singular solutions and ring-type singular solutions of the biharmonic nonlinear Schr\"{o}dinger equations (\ref{problem}) by adaptive grid methods and static grid redistribution methods, respectively.  \textcolor{red}{No numerical analysis is presented therein to test the numerical methods such as their stability, convergence, etc.  Nonetheless, we want to highlight that nonlinear Schr\"{o}dinger equations with higher-order dispersive term (\ref{full_problem}) not only plays an important role in the physical model description, such as the quantum effect in the propagation of Langmuir waves in plasma, but also brings interesting mathematical effect, such as stabilization of soliton instabilities.  It is worth, theoretically and practically, developing stable and efficient numerical methods for better understanding the dynamics within nonlinear biharmonic Schr\"{o}dinger equations.} 


%{\color{red}Before proceeding further, we want to note that various numerical methods have been proposed to solve nonlinear Schr\"{o}dinger equations (\ref{full_problem}) \textcolor{blue}{(see \cite{chang1999difference,pathria1990pseudo,dag1999quadratic,karakashian1998space,chen2019ultra,zhang2021local,fan2008generalized,lu2005conservative,lu2008fourier,baruch2010singular,baruch2010ring,zhang2021conservative, antoine2013computational} and reference therein)--I don't understand why they are needed? You should cite properly and make sure th}.  For instance, several important finite difference schemes, such as, Crank--Nicolson finite difference method (CNFD) \cite{bao2012uniform}, relaxation finite difference method (ReFD) \cite{besse2004relaxation}, semi-implicit finite difference method (SIFD) \cite{bao2013optimal} are implemented and analyzed.  In particular, CNFD uses the second-order centered difference scheme for spatial discretization and the Crank--Nicolson scheme for time discretization, and ReFD makes a second-order approximation to the nonlinear term at each time level $t_n$, while SIFD applies the leap-frog scheme for the nonlinear term in time discretization. Both CNFD and ReFD preserve the mass and the energy associated with the problem. However, the convergence order of all these three schemes was low.  \cite{pathria1990pseudo} introduced pseudo-spectral split-step methods for general NLS equations: for the case that conserves the mass in the discretized system, it requires the formation of expensive convolution sums; for the case which considerably reduces the execution costs, it sacrifices the invariance property. In addition, \cite{baruch2010singular} used an adaptive grid method to investigate singular solutions of the biharmonic nonlinear Schr\"{o}dinger equations. \cite{baruch2010ring} adopted the static grid redistribution method to study the ring-type singular solutions of the biharmonic nonlinear Schr\"{o}dinger equations.  We also want to note that many finite element methods have been proposed to solve nonlinear Schr\"{o}dinger equations, such as quadratic B-spline method (see \cite{dag1999quadratic}), there the Galerkin finite-element method for numerical solution based on quadratic B-spline as both shape and weight functions was investigated; \cite{karakashian1998space,chen2019ultra,zhang2021local,fan2008generalized,lu2005conservative,lu2008fourier} and reference therein developed
%	discontinuous Galerkin methods to solve nonlinear Schr\"{o}dinger equation.  For example, \cite{xu2012optimal} gave the proof of error estimates about the linear Schr\"{o}dinger equation with local discontinuous Galerkin method. \cite{chen2019ultra} developed an ultra-weak discontinuous Galerkin method with global projection operator for one-dimensional nonlinear Schr\"{o}dinger equation.}

In this paper, we develop a stable and computationally favored ultra-weak local DG method to solve nonlinear biharmonic Schr\"{o}dinger equation. The reason for us to establish DG methods is because of its flexibility in handling geometry, provable convergence properties, accommodating $h$-$p$ adaptivity, and high parallel efficiency.  DG method was first designed by Reed and Hill \cite{reed1973triangular} to solve a problem arising from first-order neutron transport subject to a conservation law.  This finite-element method applies a piecewise polynomial basis for both the numerical and test function, and it was originally designed to deal with the first spatial derivative only (see, e.g., \cite{reed1973triangular,cockburn1989tvb,cockburn1989kutta,cockburn1989tvb,cockburn1998runge} for detailed discussions). The original DG method has developed in several directions over the past few decades.  For instance, Cockburn and Shu \cite{cockburn1998local} proposed the so-called local discontinuous Galerkin (LDG) method to solve a wide class of nonlinear convection-diffusion equations with high-order spatial derivatives.  By introducing auxiliary variables that reduce the original problem into a lower-order system, typically with first-order spatial derivatives, the LDG methods ensure the stability of the scheme by suitable numerical fluxes embedded with the resulting system.  See \cite{dong2009analysis,xu2012optimal,yan2002local} and reference therein for recent developments of the LDG method. Another streamline of development is motivated by the urge to solve high-order problems, and this includes the ultra-weak discontinuous Galerkin method (UWDG) introduced by \cite{despres1994formulation} for linear elliptic PDEs.  The idea of the UWDG method is to shift all the spatial derivatives through integration by parts to the test function in the weak formulation, and the stability of the scheme is guaranteed by certain numerical fluxes and additional internal penalty terms when necessary.  See \cite{cessenat1998application,shu2016discontinuous,cheng2008discontinuous,bona2013conservative} and the reference therein for the application and further development of the UWDG method.  

In this work,  motivated by \cite{tao2020ultraweak, tao2021discontinuous}, we develop a DG method by combining the LDG and UWDG methods and then test this new hybrid scheme for the high-order nonlinear biharmonic Schr\"{o}dinger equations in the form of (\ref{problem}).  To this end, we introduce a second-order spatial derivative as an auxiliary variable to reduce the fourth-order problem to a system with second-order in space.  This allows us to ensure the stability of the proposed scheme through the integration by parts and a suitable choice of numerical fluxes.  Moreover, {compared with the LDG method, only one auxiliary variable is needed within the new approach and this reduces the memory requirement and the computational cost.  Furthermore, compared with the UWDG method, our approach guarantees its stability without requiring internal penalty terms, and this also improves the robustness of this new scheme.}    
%Then apply the integration by parts for each equation twice and choose the suitable numerical fluxes to ensure stability. 

% Our scheme admits the following properties:
% \begin{itemize}
% 	\item Compared with the LDG method: only one auxiliary variable $w = u_{xx}$ is needed, thus reducing the memory requirement and the computational cost,

% 	\item Compared with the UWDG method: the stability of the scheme can be guaranteed by suitable numerical fluxes, no internal penalty terms are required.
% \end{itemize}

The rest of the paper is organized as follows.  We first present the governing equations and their DG formulation in Section \ref{sec_formula}.  Then we study and discuss the stability of our proposed scheme.  Section \ref{sec_error_estimate} introduces some projection operators and derives the optimal $L^2$-error estimates for semi-discrete scheme through an auxiliary equation and suitable numerical fluxes.  Then we present the fully discrete ultra-weak local DG coupled with the Crank--Nicolson time discretization, and prove its mass and Hamiltonian conserving properties in Section \ref{sec_time_dis}.  An arbitrary high order spectral deferred correction time integrator is also presented in this section.  A few numerical experiments in both $1$D and $2$D that demonstrate and verify the theoretical findings are shown in Section \ref{sec_numerical}.  Section \ref{conclusion} concludes this paper with a brief discussion of our future directions.


==> numerical_experiment.tex <==
%!TEX root = fourth_schrodinger.tex
\section{Time Discretization}\label{sec_time_dis}
{In this section we extend the semi-discrete ultra-weak local DG method to the fully discrete method which can also conserve the mass and the Hamiltonian.
	
\subsection{Crank--Nicholson time discretization}\label{sec_cn}
In this section, we discuss the Crank--Nicholson time scheme and show the mass and Hamiltonian conservation property of the corresponding fully time discrete scheme. To this end, we introduce the following two operators which will be used throughout the next contents.
\[ \mbox{Central difference operator}: \delta u^n = \frac{u^{n+1} - u^{n-1}}{2\Delta t},\]
\[\mbox{Average value operator}: \bar{\delta} u^n = \frac{u^{n+1} + u^{n-1}}{2}.\]
The fully discrete approximation $u^n_h = u(\cdot,t_n)$ of problem (\ref{system_2nd}) is given as follows

\begin{align}
	& \int_{K} i\delta u_h^n \phi + \bar{\delta} w_h^n \Delta \phi + \bar{\delta} u_h^n \frac{F(|u_h^{n+1}|^2)- F(|u^{n-1}_h|^2)}{|u_h^{n+1}|^2 - |u_h^{n-1}|^2} \phi\ d{\bf x} \nonumber\\
	&\hspace{4cm}= - \bar{\delta}\widetilde{w_{hx}^n} \phi^-|_{j+\frac{1}{2}} + \bar{\delta}\widetilde{w_{hx}^n} \phi^+|_{j-\frac{1}{2}} + \bar{\delta}\widetilde{w_h^n}\phi_x^-|_{j+\frac{1}{2}} - \bar{\delta}\widetilde{w_h^n}\phi_x^+|_{j-\frac{1}{2}},\label{fully1} \\
	& \int_{I_j} w^{n+1}_h \psi - u_h^{n+1}\psi_{xx}\ dx = \widehat{u_{hx}^{n+1}}\psi^{-}|_{j+\frac{1}{2}}-\widehat{u_{hx}^{n+1}}\psi^{+}|_{j-\frac{1}{2}} - \widehat{u_{h}^{n+1}}\psi_x^{-}|_{j+\frac{1}{2}} + \widehat{u_{h}^{n+1}}\psi_x^{+}|_{j-\frac{1}{2}},\label{fully2}\\
	& \int_{I_j} w^{n-1}_h \psi - u_h^{n-1}\psi_{xx}\ dx = \widehat{u_{hx}^{n-1}}\psi^{-}|_{j+\frac{1}{2}}-\widehat{u_{hx}^{n-1}}\psi^{+}|_{j-\frac{1}{2}} - \widehat{u_{h}^{n-1}}\psi_x^{-}|_{j+\frac{1}{2}} + \widehat{u_{h}^{n-1}}\psi_x^{+}|_{j-\frac{1}{2}},\label{fully3}
	\end{align}
	for all test functions $\phi, \psi\in V_h^q,$ and the numerical fluxes are defined in (\ref{fluxa}). We then have the following conservation property.
	\begin{truth}
	 For all $n$, the solution to the fully discrete ultra-weak LDG scheme (\ref{fully1})--(\ref{fully3}) conserves the discrete mass
		\begin{equation}\label{discrete_mass}
		M_h^{n+1} := \frac{1}{2}\sum_j\int_{I_j} \vert u_h^n\vert + \vert u_h^{n+1}\vert\ dx, 
		\end{equation}
		and the discrete Hamiltonian
		\begin{equation}\label{discrete_H}
		H_h^{n+1} := \frac{1}{2}\sum_j\int_{I_j} \vert w_h^n\vert + \vert w_h^{n+1}\vert  + F(|u_h^{n+1}|^2) + F(|u_h^n|^2)\  dx.
		\end{equation}
	\end{truth}
	\begin{proof}
		To prove the fully discrete mass conservation (\ref{discrete_mass}), we choose the test function $\phi = \bar{\delta} u_h^{n,\ast}$ in (\ref{fully1}) to obtain
		\begin{align}\label{fully11}
		&\int_{I_j} i\delta u_h^n \bar{\delta} u_h^{n,\ast} + \bar{\delta} w_h^n \bar{\delta} u_{hxx}^{n,\ast} + \bar{\delta} u_h^n \frac{F(|u_h^{n+1}|^2)- F(|u^{n-1}_h|^2)}{|u_h^{n+1}|^2 - |u_h^{n-1}|^2} \bar{\delta} u_h^{n,\ast}\ dx \nonumber \\
		=& - \bar{\delta}\widetilde{w_{hx}^n} \bar{\delta} u_h^{n,\ast, -}|_{j+\frac{1}{2}} + \bar{\delta}\widetilde{w_{hx}^n} \bar{\delta} u_h^{n,\ast,+}|_{j-\frac{1}{2}} + \bar{\delta}\widetilde{w_h^n}\bar{\delta} u_{hx}^{n,\ast,-}|_{j+\frac{1}{2}} - \bar{\delta}\widetilde{w_h^n}\bar{\delta} u_{hx}^{n,\ast,+}|_{j-\frac{1}{2}}, 
		\end{align}
		and the test function $\psi = \bar{\delta} w_h^{n,\ast}/2$ in (\ref{fully2}) and (\ref{fully3}) to generate
{
		\begin{align}\label{full2_1}
	&\int_{I_j} (w^{n+1}_h \bar{\delta} w_h^{n,\ast} - u_h^{n+1}\bar{\delta} w_{hxx}^{n,\ast})/2 \ dx\nonumber \\
		=&\  (\widehat{u_{hx}^{n+1}}\bar{\delta} w_h^{n,\ast-} |_{j+\frac{1}{2}}-\widehat{u_{hx}^{n+1}}\bar{\delta} w_h^{n,\ast,+} |_{j-\frac{1}{2}} - \widehat{u_{h}^{n+1}}\bar{\delta} w_{hx}^{n,\ast,-} |_{j+\frac{1}{2}} + \widehat{u_{h}^{n+1}}\bar{\delta} w_{hx}^{n,\ast,+} |_{j-\frac{1}{2}})/2,
		\end{align}
		and
		\begin{align}\label{fully3_1}
		&\int_{I_j} w^{n-1}_h( \bar{\delta} w_h^{n,\ast} - u_h^{n-1}\bar{\delta} w_{hxx}^{n,\ast})/2 \ dx \nonumber\\
		=&\  (\widehat{u_{hx}^{n-1}}\bar{\delta} w_h^{n,\ast-} |_{j+\frac{1}{2}}-\widehat{u_{hx}^{n-1}}\bar{\delta} w_h^{n,\ast,+} |_{j-\frac{1}{2}} - \widehat{u_{h}^{n-1}}\bar{\delta} w_{hx}^{n,\ast,-} |_{j+\frac{1}{2}} + \widehat{u_{h}^{n-1}}\bar{\delta} w_{hx}^{n,\ast,+} |_{j-\frac{1}{2}})/2.
		\end{align}}
		Adding (\ref{full2_1}) to (\ref{fully3_1}), we have
		\begin{align}\label{fully23}
		&\int_{I_j} \bar{\delta} w^n_h \bar{\delta} w_h^{n,\ast} - \bar{\delta} u^n_h\bar{\delta} w_{hxx}^{n,\ast} \ dx \nonumber\\
		=& \  \bar{\delta}\widehat{u_{hx}^{n}}\bar{\delta} w_h^{n,\ast-} |_{j+\frac{1}{2}}-\bar{\delta}\widehat{u_{hx}^{n}}\bar{\delta} w_h^{n,\ast,+} |_{j-\frac{1}{2}} - \bar{\delta}\widehat{u_{h}^{n}}\bar{\delta} w_{hx}^{n,\ast,-} |_{j+\frac{1}{2}} + \bar{\delta}\widehat{u_{h}^{n}}\bar{\delta} w_{hx}^{n,\ast,+} |_{j-\frac{1}{2}}.
		\end{align}
		For the resulting equations (\ref{fully11}) and (\ref{fully23}), by the same analysis that leads to the conservation of the semi-discrete mass (\ref{M}) in Section \ref{sec:conservation}, we can obtain
		\begin{equation}\label{discrete_M_eq}
		2\times \frac{1}{2\Delta t} \bigg[ \sum_j\int_{I_j} \frac{\vert u_h^{n+1}\vert + \vert u_h^{n}\vert}{2} - \frac{\vert u_h^n\vert + \vert u_h^{n-1}\vert}{2}\ dx\bigg] = 0.
		\end{equation}
		Combining (\ref{discrete_M_eq}) and the definition of $M_h^n$ in (\ref{discrete_mass}), we have $M_h^{n+1} = M_h^{n}$ for all $n$. This illustrates
		the fully discrete mass is conserved by using the fully discrete scheme (\ref{fully1})--(\ref{fully3}).
		
		For the fully discrete Hamiltonian conservation (\ref{discrete_H}), we let the test function $\phi = \delta u_h^{n,\ast}$ in (\ref{fully1}) to get
		\begin{align}\label{fully1_2}
		&\int_{I_j} i\delta u_h^n \delta u_h^{n,\ast} + \bar{\delta} w_h^n \delta u_{hxx}^{n,\ast} + \bar{\delta} u_h^n \frac{F(|u_h^{n+1}|^2)- F(|u^{n-1}_h|^2)}{|u_h^{n+1}|^2 - |u_h^{n-1}|^2} \delta u_h^{n,\ast}\ dx \nonumber \\
		=&- \bar{\delta}\widetilde{w_{hx}^n} \delta u_h^{n,\ast, -}|_{j+\frac{1}{2}} + \bar{\delta}\widetilde{w_{hx}^n} \delta u_h^{n,\ast,+}|_{j-\frac{1}{2}} + \bar{\delta}\widetilde{w_h^n}\delta u_{hx}^{n,\ast,-}|_{j+\frac{1}{2}} - \bar{\delta}\widetilde{w_h^n}\delta u_{hx}^{n,\ast,+}|_{j-\frac{1}{2}},
		\end{align}
		%	then take the conjugate of the above equation to get
		%	\begin{multline*}
		%	\int_{I_j} -i\delta u_h^{n,\ast} \delta u_h^{n} + \bar{\delta} u_h^{n,\ast} \delta u_{hxx}^{n} + \bar{\delta} u_h^{n,\ast} \frac{F(|u_h^{n+1}|^2) F'(|u^{n-1}_h|^2)}{|u_h^{n+1}|^2 - |u_h^{n-1}|^2} \delta u_h^{n}\ dx \\
		%	= - \bar{\delta}\widetilde{w_{hx}^{n,\ast}} \delta u_h^{n, -}|_{j+\frac{1}{2}} + \bar{\delta}\widetilde{w_{hx}^{n,\ast}} \delta u_h^{n,+}|_{j-\frac{1}{2}} + \bar{\delta}\widetilde{w_h^{n,\ast}}\delta u_{hx}^{n,-}|_{j+\frac{1}{2}} - \bar{\delta}\widetilde{w_h^{n,\ast}}\delta u_{hx}^{n,+}|_{j-\frac{1}{2}}.
		%	\end{multline*}
		In (\ref{fully2}) and (\ref{fully3}), we choose the test function $\psi = \bar{\delta}w^{n,\ast}_h/(2\Delta t)$ to obtain
		\begin{align}
		&\int_{I_j} (w^{n+1}_h \bar{\delta} w_h^{n,\ast}- u_h^{n+1}\bar{\delta} w_{hxx}^{n,\ast})/(2\Delta t)\ dx \nonumber\\
		=& \  (\widehat{u_{hx}^{n+1}}\bar{\delta} w_h^{n,\ast-}|_{j+\frac{1}{2}}-\widehat{u_{hx}^{n+1}}\bar{\delta} w_h^{n,\ast,+}|_{j-\frac{1}{2}} - \widehat{u_{h}^{n+1}}\bar{\delta} w_{hx}^{n,\ast,-}|_{j+\frac{1}{2}} + \widehat{u_{h}^{n+1}}\bar{\delta} w_{hx}^{n,\ast,+}|_{j-\frac{1}{2}})/(2\Delta t),\label{fully2_2}\\
		&\int_{I_j} (w^{n-1}_h \bar{\delta} w_h^{n,\ast} - u_h^{n-1}\bar{\delta} w_{hxx}^{n,\ast})/(2\Delta t)\ dx\nonumber \\
		=& \ (\widehat{u_{hx}^{n-1}}\bar{\delta} w_h^{n,\ast,-}|_{j+\frac{1}{2}}-\widehat{u_{hx}^{n-1}}\bar{\delta} w_h^{n,\ast,+}|_{j-\frac{1}{2}} - \widehat{u_{h}^{n-1}}\bar{\delta} w_{hx}^{n,\ast,-}|_{j+\frac{1}{2}} + \widehat{u_{h}^{n-1}}\bar{\delta} w_{hx}^{n,\ast,+}|_{j-\frac{1}{2}})/(2\Delta t),\label{fully3_2}
		\end{align}
		and subtracting (\ref{fully2_2}) from (\ref{fully3_2}) yields
		\begin{align}\label{discrete_H_1}
		&\int_{I_j} \delta w^{n}_h \bar{\delta} w_h^{n,\ast} - \delta u_h^{n}\bar{\delta} w_{hxx}^{n,\ast}\ dx \nonumber\\
		= &\ \delta\widehat{ u_{hx}^{n}}\bar{\delta} w_h^{n,\ast,-}|_{j+\frac{1}{2}}-\delta\widehat{u_{hx}^{n}}\bar{\delta} w_h^{n,\ast,+}|_{j-\frac{1}{2}} - \delta\widehat{u_{h}^{n}}\bar{\delta} w_{hx}^{n,\ast,-}|_{j+\frac{1}{2}} + \delta\widehat{u_{h}^{n}}\bar{\delta} w_{hx}^{n,\ast,+}|_{j-\frac{1}{2}}.
		\end{align}
		%	and its conjugate
		%	\begin{multline*}
		%	\int_{I_j} \delta w^{n,\ast}_h \frac{\bar{\delta} w_h^n}{\Delta t} - \delta u_h^{n,\ast}\frac{\bar{\delta} w_{hxx}^n}{\Delta t}\ dx \\
		%	= \delta\widehat{ u_{hx}^{n,\ast}}\frac{\bar{\delta} w_h^{n,-}}{\Delta t}|_{j+\frac{1}{2}}-\delta\widehat{u_{hx}^{n,\ast}}\frac{\bar{\delta} w_h^{n,+}}{\Delta t}|_{j-\frac{1}{2}} - \delta\widehat{u_{h}^{n,\ast}}\frac{\bar{\delta} w_{hx}^{n,-}}{\Delta t}|_{j+\frac{1}{2}} + \delta\widehat{u_{h}^{n,\ast}}\frac{\bar{\delta} w_{hx}^{n,+}}{\Delta t}|_{j-\frac{1}{2}}.
		%	\end{multline*}
		For the resulting equations (\ref{fully1_2}) and (\ref{discrete_H_1}), by utilizing the same analysis for the conservation of the semi-discrete Hamiltonian (\ref{E}) in Section \ref{sec:conservation}, we arrive at
		\begin{multline}\label{fully_H1}
		2\times\frac{1}{2\Delta t} \Big[\sum_j\int_{I_j} \frac{\vert w_h^{n+1}\vert + \vert w_h^{n}\vert}{2} - \frac{\vert w_h^n\vert + \vert w_h^{n-1}\vert}{2} \\+ \frac{F(|u_h^{n+1}|^2) + F(|u_h^n|^2)}{2} - \frac{F(|u_h^{n}|^2) + F(|u_h^{n-1}|^2)}{2}\ dx\Big] = 0.
		\end{multline}
		From (\ref{fully_H1}) and the definition of $H_h^n$ in (\ref{discrete_H}), we that have $H_h^{n+1} = H_h^{n}$ for all $n$, and this verifies that the fully discrete Hamiltonian is conserved by using the fully discrete scheme (\ref{fully1})--(\ref{fully3}).
	\end{proof}
	
	The fully discrete scheme (\ref{fully1}) -- (\ref{fully3}) results in the following nonlinear algebraic equation
	\[{\bf U}^{n+1} = \mathcal{L}({\bf U}^{n-1}, {\bf U}^{n+1}) + \mathcal{N}({\bf U}^{n-1}, {\bf U}^{n+1}),\]
	where ${\bf U}$ containing the degrees of freedom for $u_h$, $\mathcal{L}({\bf U}^{n-1}, {\bf U}^{n+1}) $ is a linear function of ${\bf U}^{n-1}, {\bf U}^{n+1}$, and $\mathcal{N}({\bf U}^{n-1}, {\bf U}^{n+1})$ is a nonlinear function of ${\bf U}^{n}, {\bf U}^{n+1}$. In the implementation, we use Newton method to find ${\bf U}^{n+1}$ for each time level $t_{n+1}$. Since the second order central difference is used on time discretization and we mainly concern the effect of the spatial discretization, we use the time step $\Delta t = \mbox{cfl}\times h^4$ to guarantee that the error will be dominated by the spatial discretization when using the Crank--Nicholson time integrator for the numerical experiments.
	
	In what follows, we also present another popular time-stepping algorithm for the semi-discrete problem and compare the mass and the Hamiltonian evolution history in the numerical experiments with the fully discrete scheme coupled with Crank--Nicholson time scheme proposed in Section \ref{sec_cn}.
}

\subsection{The spectral deferred correction (SDC) time-stepping algorithm} 
{We now describe} an SDC method to solve the semi-discrete problem generated by scheme (\ref{DG_scheme1})--(\ref{DG_scheme2}).  This method builds on the low-order time-stepping scheme, and then iterative corrections on a defect equation to obtain the desired order of accuracy (see e.g., \cite{dutt2000spectral,hagstrom2007spectral}).  We extend \cite{zhang2021beam} by applying it to the nonlinear problems in this paper.  In what follows, we present the SDC algorithm for the problems with both linear and nonlinear terms for completeness.  An essential step for this purpose is to use an implicit method for the linear terms but an explicit method for the nonlinear terms. 

To illustrate this idea, let us consider a generic ODE system as follows
\begin{equation*}
\left\{
\begin{aligned}
&y_t = Ay + G(y), \ \ t\in(0,T],\\
&y(0) = y_0,
\end{aligned}
\right.
\end{equation*}
where $y_0, y(t)\in \mathbb{C}^l$, $A\in M_{l\times l}(\mathbb{C})$  and $G: \mathbb{C}^l \rightarrow \mathbb{C}^l$ is a nonlinear function. Suppose the time interval $[0,T]$ is partitioned into $N_t$ subintervals as $0 = t_0 < t_1 < \cdots < t_n < \cdots < \cdots < t_{N_t} = T$. Denote $\Delta t_n := t_{n+1} - t_n$ and $y_n := y(t_n)$, then our SDC time stepping algorithm proceeds as follows:
%{\fontfamily{qcr}\selectfont %qtm	qcr
%This text uses a different font typeface
%\begin{itemize}
%	\item Input: $y^1_{n,0} = y_n$, $t_n$, $t_{n+1}$, $m$, $J$,
%	\item Compute $m$ Gauss-Radau points $\tau_i\in (t_n, t_{n+1}]$ and set $\tau_0 = t_n$, $k_i = \tau_i - \tau_{i-1}$,
%	\item Compute the initial approximation
%	\begin{itemize}
%		\item For $i = 1, \cdots, m$
%		\begin{itemize}
%\item [1.] Solve $y_{n,i}^1 = y_{n,i-1}^1 + %k_i\left(Ay_{n,i}^1 + G(y_{n,{i-1}}^1)\right)$,
%\end{itemize}
%\end{itemize}
%\item Compute successive corrections
%\begin{itemize}
%	\item For $j = 1, \cdots, J$
%	  \begin{itemize}
%	 \item[--] Initialize $\epsilon_{n,0}^j = 0$, $\delta_{n,0}^j = 0$,
%	\item[--] For $i = 1, \cdots, m$
%	\begin{itemize}
%	\item [1.] Compute $\epsilon_{n,i}^j = y_n - y_{n,i}^{j} + I_{n,0}^{n,i} (Ay^{j}(\tau)+G(y^j(\tau)))$,
%	\item [2.] Compute intermediate function value $\bar{y} = y_{n,i-1}^j + \delta_{n,i-1}^j$,
%	\item [3.] Compute intermediate nonlinear function value $\bar{G} = G(\bar{y})$,
%	\item [2.] Solve $\delta_{n,i}^{j} \!=\! \delta_{n,i-1}^j + k_iA\delta_{n,i}^j + (\epsilon_{n,i}^j - \epsilon_{n,i-1}^j) + k_i\left(\!G(\bar{y}) \!-\! G(y_{n,i-1}^j)\!\right)\!\!,$
%	\item[3.] Update $y_{n,i}^{j+1} = y_{n,i}^j + \delta_{n,i}^j$,
%	\end{itemize}		
%\end{itemize}
%\end{itemize}
%\item Return $y^{J+1}_{n,m}$.
%\end{itemize}
%}

\setalgorithmicfont{\footnotesize}

\begin{algorithm}
	\caption{SDC time stepping algorithm }
	\begin{algorithmic}[1]
		\STATE Input: $y^1_{n,0} = y_n$, $t_n$, $t_{n+1}$, $m$, $J$
		\STATE Compute $m$ Gauss-Radau points $\tau_i\in (t_n, t_{n+1}]$ and set $\tau_0 = t_n$, $k_i = \tau_i - \tau_{i-1}$
		\FOR{$i = 1, \cdots, m$}
		\STATE Solve $y_{n,i}^1 = y_{n,i-1}^1 + k_i\left(Ay_{n,i}^1 + G(y_{n,{i-1}}^1)\right)$,\COMMENT{Compute the initial approximation}
		\ENDFOR
		\FOR{$j = 1, \cdots, J$}
		\STATE Initialize $\epsilon_{n,0}^j = 0$, $\delta_{n,0}^j = 0$
		\FOR{$i = 1, \cdots, m$}
		\STATE Compute $\epsilon_{n,i}^j = y_n - y_{n,i}^{j} + I_{n,0}^{n,i} (Ay^{j}(\tau)+G(y^j(\tau)))$
		\STATE Compute intermediate function value $\bar{y} = y_{n,i-1}^j + \delta_{n,i-1}^j$
		\STATE Compute intermediate nonlinear function value $\bar{G} = G(\bar{y})$
		\STATE Solve $\delta_{n,i}^{j} = \delta_{n,i-1}^j + k_iA\delta_{n,i}^j + (\epsilon_{n,i}^j - \epsilon_{n,i-1}^j) + k_i\left(G(\bar{y})- G(y_{n,i-1}^j)\right)$
		\STATE Update $y_{n,i}^{j+1} = y_{n,i}^j + \delta_{n,i}^j$
		\ENDFOR
		\ENDFOR
		\STATE \textbf{return} $y^{J+1}_{n,m}$
	\end{algorithmic}
\end{algorithm}
{In this algorithm, $I_{n,0}^{n,i}(Ay^j(\tau) + G(y^j(\tau)))$ denotes the integral of the $(m-1)$-th degree interpolating polynomial on the $m$ nodes $(\tau_i, Ay_{n,i}^j + G(y_{n,i}^j))_{i = 1}^m$ over the subinterval $[t_n, \tau_i]$, and it is the numerical quadrature approximation of $\int_{t_n}^{\tau_i} Ay^j(\tau) + G(y^j(\tau)) d\tau$.} For all the experiments, we set $m = 5$ and $J = 15$ so that the convergence order in time ($2m-1$) is larger than the convergence order in space ($4th$ order in space).   Moreover, we fix the time step as $\Delta t = 0.1$ when using the SDC scheme. 

%{\color{red} Though it is easy to construct an arbitrarily high-order SDC scheme in the temporal space, such scheme does not conserve energy in general.  Therefore, in what follows, we discuss the the energy-conserving Crank--Nicholson scheme, even if only a second order in time space is expected.}

\section{Numerical Simulations}\label{sec_numerical}

In this section, we present several numerical experiments to illustrate and support the convergence of the proposed DG scheme in Section \ref{sec_formula}. Through these studies, We use a standard modal basis formulation and the alternating flux (\ref{fluxa}) for the conciseness of demonstration.% and without loss of generality.

%For simplicity of the implementation, we use $L^2$ projection for the numerical initial condition of $u_h$, and then we use (\ref{}) to solve the numerical initial condition of $w_h$. We then implement the DG method (\ref{DG_scheme1})-(\ref{DG_scheme2}) with the alternating fluxes (\ref{}) and use the SDC time integrator introduced in Section~\ref{}. 

 
 \subsection{Linear problem}\label{liner_sec}
We first consider the biharmonic Schr\"{o}dinger equation with $F'(|u|^2) = 1$, 
\begin{equation}\label{eg1}
iu_t + u_{xxxx} + u = 0, \ \ (x,t) \in [0, 4\pi]\times(0, 1],
\end{equation} 
subject to periodic boundary condition and initial condition
\[u(x,0) = \cos(x) + i \sin(x).\]
Note that this PDE has the following exact solution 
\[u(x,t) = \cos(x + 2t) + i\sin(x + 2t).\]

We uniformly discretize the spatial interval through vertices $x_j = jh$, $j = 0,\cdots ,N$, $h = 4\pi/N$.   Throughout the studies we present results by considering the degree of the approximation space of $u_h$ and $w_h$ being $q = (1,2,3)$.

From Table \ref{linear_u} to Table \ref{linear_w}, we present the $L^2$ and $L^\infty$ errors for the real and imaginary parts of $u$ and $w$, respectively.  We also include the corresponding numerical orders of accuracy subject to the variation of $q$ and $N$. {There are several conclusions we can make out from these tables.}  First of all, the proposed scheme consistently gives the optimal $(q + 1)$-th order of the accuracy across the choices of size $N$ and the error norms.  Moreover, there are infinitesimal differences between the $L^2$ errors of the real and imaginary parts of both $u$ and $w$.  Indeed, their differences are at the order of $10^{-12}$ and we skip presenting them therein.  %\textcolor{red}{For $L^\infty$ errors, we observe a larger difference between the real and the imaginary parts for both $u$ and $w$ when $N$ is small.-rewrite}\textcolor{magenta}{can you help here? I want to express is that the are some differences between the errors of the real part and the imaginary part of $u$ (same observation for w) when $N$ is small. The reason I put here is that the errors in the table are almost the same for the real part and the imaginary part, I am worried about the readers misunderstand they are the exact same functions for the real part and the imaginary part, but they are not. Or we can delete this part (red color) since it is not important. }
			
\begin{table}
 	\footnotesize
 	\begin{center}
 		\scalebox{1.0}{
 			\begin{tabular}{c c c c c c c c c c}
 				\hline
 				~ & ~ &  $\mbox{Re}(u)$ &~ &~&~& $\mbox{Im}(u)$& ~ & ~ & ~\\
 				\cline{3-6} \cline{7-10}
 				$q$ & $N$ & $L^2$ error & order & $L^\infty$ error & order  & $L^2$ error & order & $L^\infty$ error & order \\
 				\hline
 				1& 10 & 1.01e-00& --& 4.47e-01& -- &1.01e-00 & -- & 4.54e-01 & --\\
 				~& 20 & 3.28e-01& 1.62& 1.47e-01& 1.60& 3.28e-01 & 1.62 & 1.43e-01 & 1.67\\
 				~& 40 & 8.78e-02& 1.90& 3.71e-02& 1.99&8.78e-02  & 1.90 & 3.71e-02 & 1.94\\
 				~& 80 & 2.23e-02& 1.97& 9.20e-03& 2.01&2.23e-02  & 1.97 & 9.20e-03 & 2.01\\
 				~& 160 & 5.61e-03& 1.99& 2.27e-03& 2.02&5.61e-03  & 1.99 & 2.27e-03 & 2.02\\
 				~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~\\
 				2& 10 & 6.68e-02& --& 3.06e-02& -- &6.68e-02 & -- & 2.98e-02 & --\\
 				~& 20 & 7.57e-03& 3.14& 3.89e-03& 2.97& 7.57e-03 & 3.14 & 3.76e-03 & 2.99\\
 				~& 40 & 9.24e-04& 3.03& 5.19e-04& 2.91&9.24e-04  & 3.03 & 5.19e-04 & 2.86\\
 				~& 80 & 1.15e-04& 3.01& 6.73e-05& 2.95&1.15e-04  & 3.01 & 6.73e-05 & 2.95\\
 				~& 160 & 1.43e-05& 3.00& 8.57e-06& 2.97&1.43e-05  & 3.00 & 8.57e-06 & 2.97\\
 				~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~\\
 				3& 10 & 4.06e-03& --& 2.35e-03& -- &4.06e-03 & -- & 2.27e-03 & --\\
 				~& 20 & 2.49e-04& 4.03& 1.39e-04& 4.08& 2.49e-04 & 4.03 & 1.44e-04 & 3.98\\
 				~& 40 & 1.55e-05& 4.01& 8.87e-06& 3.97&1.55e-05  & 4.01 & 8.87e-06 & 4.02\\
 				~& 80 & 9.67e-07& 4.00& 5.54e-07& 4.00&9.67e-07  & 4.00 & 5.54e-07 & 4.00\\
 				~& 160 & 6.06e-08& 4.00& 3.50e-08& 3.98&6.06e-08  & 4.00 & 3.57e-08 & 3.96\\
 				\hline
 			\end{tabular}
 		}
 	\end{center}
 	\caption{\scriptsize{We present the $L^2/L^\infty$ errors and the corresponding convergence rates for $u$ (the real part $\mbox{Re}(u)$ and the imaginary part $\mbox{Im}(u)$) for problem (\ref{eg1}) using $\mathcal{P}^q$ polynomials.  The interval is divided into $N$ uniform cells, and the terminal computational time $T = 1$.}  These results present the optimal convergence which is robust to the error norm.}\label{linear_u}
 \end{table}
 
 
 
 \begin{table}
 	\footnotesize
 	\begin{center}
 		\scalebox{1.0}{
 			\begin{tabular}{c c c c c c c c c c}
 				\hline
 				~ & ~ &  $\mbox{Re}(w)$ &~ &~&~& $\mbox{Im}(w)$& ~ & ~ & ~\\
 				\cline{3-6} \cline{7-10}
 				$q$ & $N$ & $L^2$ error & order & $L^\infty$ error & order  & $L^2$ error & order & $L^\infty$ error & order \\
 				\hline
 				1& 10 & 1.37e-00& --& 5.49e-01& -- &1.37e-00 & -- & 5.76e-01 & --\\
 				~& 20 & 3.19e-01& 2.10& 1.58e-01& 1.79& 3.19e-01 & 2.10 & 1.54e-01 & 1.90\\
 				~& 40 & 9.10e-02& 1.81& 4.33e-02& 1.87&9.10e-02  & 1.81 & 4.33e-02 & 1.83\\
 				~& 80 & 2.39e-02& 1.93& 1.11e-02& 1.96&2.39e-02  & 1.93 & 1.11e-02 & 1.96\\
 				~& 160 & 6.08e-03&1.97& 2.80e-03& 1.99 &6.08e-03  & 1.97 & 2.80e-03 & 1.99\\
 				~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~  & ~\\
 				2& 10 & 7.39e-02& --& 4.92e-02& -- &7.39e-02 & -- & 4.74e-02 & --\\
 				~& 20 & 7.58e-03& 3.29& 5.01e-03& 3.30& 7.58e-03 & 3.29 & 4.83e-03 & 3.29\\
 				~& 40 & 9.24e-04& 3.04& 5.95e-04& 3.07&9.24e-04  & 3.04 & 5.95e-04 & 3.02\\
 				~& 80 & 1.15e-04& 3.01& 7.22e-05& 3.04&1.15e-04  & 3.01 & 7.22e-05 & 3.04\\
 				~& 160 & 1.43e-05&3.00& 8.88e-06& 3.02&1.43e-05  & 3.00 & 8.88e-06 & 3.02\\
 				~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~\\
 				3& 10 & 4.06e-03& --& 2.43e-03& -- &4.06e-03 & -- & 2.50e-03 & --\\
 				~& 20 & 2.49e-04& 4.03& 1.44e-04& 4.08& 2.49e-04 & 4.03 & 1.43e-04 & 4.13\\
 				~& 40 & 1.55e-05& 4.01& 8.91e-06& 4.02 &1.55e-05  & 4.01 & 8.91e-06 & 4.00\\
 				~& 80 & 9.67e-07& 4.00& 5.54e-07& 4.01&9.67e-07  & 4.00 & 5.54e-07 & 4.01\\
 				~& 160 & 6.06e-08& 4.00& 3.57e-08& 3.96&6.06e-08  & 4.00 & 3.53e-08 & 3.97\\
 				\hline
 			\end{tabular}
 		}
 	\end{center}
 	\caption{\scriptsize{This table presents the errors and the corresponding convergence rates for $w$ in problem (\ref{eg1}).  All are chosen to be the same as in Table \ref{linear_u}.}}\label{linear_w}
 \end{table}

%The numerical results at time $t = 1000$ are shown in Figure \ref{uw}. From this figure, we observe that the numerical results profiles match with exact solutions very well. We also present both the numerical mass (\ref{M}) and the numerical Hamiltonian (\ref{E}) trajectories of the proposed DG scheme for problem (\ref{eg1}) in Figure \ref{mass_hamitonian_linear}.  In particular, we show the results for the approximation degree $q = 2$ until the final time $T = 100$ with $N = 80$. We note that the magnitude of the discrete mass error and the discrete Hamiltonian error is smaller than $10^{-7}$. Since the SDC time integrator is energy dissipating, we conclude that the proposed DG scheme conserves the discrete mass and the discrete Hamiltonian. 

 The numerical mass (\ref{M}) and the numerical Hamiltonian (\ref{E}) trajectories of the proposed ultra-weak LDG scheme for problem (\ref{eg1}) are presented in Figure \ref{mass_hamitonian_linear} with both SDC and Crank--Nicholson time integrators.  In particular, we show the results for the approximation degree $q = 2$ until the final time $T = 100$ with $N = 40$. We note that the numerical mass and Hamiltonian are conserved by the conservative scheme (Crank--Nicholson time integrator).  Though the numercal mass and Hamiltonian are not conserved by the SDC time integrator, the magnitude of the numerical mass error is samller than $10^{-5}$ and the numerical Hamiltonian error is smaller than $10^{-3}$.


\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.45\textwidth]{M_evo.png}
	\includegraphics[width=0.45\textwidth]{H_evo.png}
	\caption{The left plots $M_h(t)-M_h(0)$ for problem (\ref{eg1}) using $\mathcal{P}^2$ polynomial on a uniform mesh of $N = 40$ up to a terminal time $T=100$, while the right plots $H_h(t)-H_h(0)$ under the same setting.
	}\label{mass_hamitonian_linear}
\end{figure}

%\begin{figure}[htbp]
%	\centering
%	\includegraphics[width=0.45\textwidth]{ur}
%	\includegraphics[width=0.45\textwidth]{ui}\\
%	\includegraphics[width=0.45\textwidth]{wr}
%	\includegraphics[width=0.45\textwidth]{wi}
%	\caption{Snapshots of numerical and exact solutions of problem (\ref{eg1}) at time $t = 1000$, where the numerical solutions are obtained using $\mathcal{P}^2$ polynomial on a uniform mesh of $N = 80$.  These plots provide evident support for the proposed scheme on approximating the exact solution, even up to a significantly long time.
%	}\label{uw}
%\end{figure}
 
 \subsection{Defocusing nonlinear problem}\label{defocusing_sec}
  We provide another set of studies that examine the effectiveness and theoretical convergence order of the proposed ultra-weak LDG scheme for a defocusing nonlinear biharmonic Schr\"{o}dinger equation with $F'(|u|^2) = |u|^2 + |u|^4$,
 \begin{equation}\label{defocusing}
 iu_{t} + u_{xxxx} + u|u|^2 + u|u|^4 = 0,\ \ (x,t)\in[0, 4\pi]\times(0,1],
 \end{equation}
 subject to periodic boundary condition and initial condition
 \[u(x,0) = \cos(x) + i\sin(x).\]
Such initial and boundary data introduce an exact solution for this problem and it reads 
 \[u(x,t) = \cos(x + 3t) + i\sin(x + 3t).\]
 We use the same spatial discretization as those in Section \ref{liner_sec} and display the $L^2$ and $L^\infty$ errors for the real part and the imaginary part of both $u$ and $w$ from Tables \ref{u_defocusing} to Table \ref{w_defocusing}. We observe similar results as those for the linear biharmonic Schr\"{o}dinger equations in Section \ref{liner_sec}. Specifically, we note an optimal convergence $q + 1$ for both the real part and the imaginary part of $u$ and $w$. %Again, for the $L^2$ errors, we do not have a significant difference between the real part and the imaginary part for either $u$ or $w$, and for the $L^\infty$ errors, there is a noticeable difference between the real and the imaginary part of both $u$ and $w$ when $N$ is small.
 
%Finally, Figure \ref{mass_defocusing} presents the snapshots of the numerical solution $u_h$ at $t = 1000$ and the evolution of the discrete mass errors. Here, we choose the approximation degree $q = 2$ and the number of cells $N = 80$.  From this figure, we observe that our numerical solutions match very well with the exact solution and the discrete mass is conserved with a discrete error up to a magnitude less than $10^{-7}$.  Moreover, the fact that a discrete SDC time integrator is energy-dissipating is also observed therein.

Finally, Figure \ref{uw_non} presents the snapshots of the numerical solution $u_h$ and $w_h$ at $t = 1000$. Here, we choose the approximation degree $q = 2$ and the number of cells $N = 80$.  From this figure, we observe that our numerical solutions match very well with the exact solution.

			
  \begin{table}
 	\footnotesize
 	\begin{center}
 		\scalebox{1.0}{
 			\begin{tabular}{c c c c c c c c c c c}
 				\hline
 				~ & ~ &  $\mbox{Re}(u)$ &~ &~ &~&~& $\mbox{Im}(u)$& ~ & ~ & ~\\
 				\cline{3-6} \cline{8-11}
 				$q$ & $N$ & $L^2$ error & order & $L^\infty$ error & order & ~ & $L^2$ error & order & $L^\infty$ error & order \\
 				\hline
 				1& 10 & 4.63e-01& --& 2.07e-01& -- & ~ &4.63e-01 & -- & 1.99e-01 & --\\
 				~& 20 & 2.47e-01& 0.91& 1.10e-01& 0.91& ~& 2.47e-01 & 0.91 & 1.12e-01 & 0.83\\
 				~& 40 & 8.16e-02& 1.60& 3.44e-02& 1.68& ~ &8.16e-02  & 1.60 & 3.44e-02 & 1.70\\
 				~& 80 & 2.19e-02& 1.90& 9.01e-03& 1.93& ~ &2.19e-02  & 1.90 & 9.01e-03 & 1.93\\
 				~& 160 & 5.58e-03& 1.97& 2.26e-03& 1.99& ~ &5.58e-03  & 1.97 & 2.26e-03 & 1.99\\
 				~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~\\
 				2& 10 & 6.42e-02& --& 2.95e-02& -- & ~ &6.42e-02 & -- & 2.88e-02 & --\\
 				~& 20 & 7.57e-03& 3.08& 3.80e-03& 2.96& ~& 7.57e-03 & 3.08 & 3.86e-03 & 2.90\\
 				~& 40 & 9.24e-04& 3.04& 5.20e-04& 2.87& ~ &9.24e-04  & 3.04 & 5.20e-04 & 2.89\\
 				~& 80 & 1.15e-04& 3.01& 6.72e-05& 2.95& ~ &1.15e-04  & 3.01 & 6.72e-05 & 2.95\\
 				~& 160 & 1.43e-05& 3.00& 8.57e-06& 2.97& ~ &1.43e-05  & 3.00 & 8.57e-06 & 2.97\\
 				~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~\\
 				3& 10 & 4.01e-03& --& 2.28e-03& -- & ~ &4.01e-03 & -- & 2.34e-03 & --\\
 				~& 20 & 2.49e-04& 4.01& 1.43e-04& 4.00& ~& 2.49e-04 & 4.01& 1.41e-04 & 4.06\\
 				~& 40 & 1.55e-05& 4.01& 8.89e-06& 4.00& ~ &1.55e-05  & 4.01 & 8.89e-06 & 3.98\\
 				~& 80 & 9.67e-07& 4.00& 5.53e-07& 4.01& ~ &9.67e-07  & 4.00 & 5.53e-07 & 4.01\\
 				~& 160 & 6.06e-08& 4.00& 3.54e-08& 3.96& ~ &6.06e-08  & 4.00 & 3.52e-08 & 3.97\\
 				\hline
 			\end{tabular}
 		}
 			\end{center}
 	\caption{\scriptsize{Errors and the corresponding convergence rates for $u$ of problem (\ref{defocusing}) using $\mathcal{P}^q$ polynomials on a uniform mesh of $N$ cells up to terminal time $T = 1$.  This table adds additional evidence that supports the optimal and robust convergence of the proposed scheme.}}\label{u_defocusing}
 \end{table}
 
\begin{table}
	\footnotesize
	\begin{center}
		\scalebox{1.0}{
			\begin{tabular}{c c c c c c c c c c c}
				\hline
				~ & ~ &  $\mbox{Re}(w)$ &~ &~ &~&~& $\mbox{Im}(w)$& ~ & ~ & ~\\
				\cline{3-6} \cline{8-11}
				$q$ & $N$ & $L^2$ error & order & $L^\infty$ error & order & ~ & $L^2$ error & order & $L^\infty$ error & order \\
				\hline
				1& 10 & 1.17e-00& --& 6.38e-01& -- & ~ &1.17e-00 & -- & 6.17e-01 & --\\
				~& 20 & 2.45e-01& 2.25& 1.21e-01& 2.40& ~& 2.45e-01 & 2.25 & 1.26e-01 & 2.29\\
				~& 40 & 8.50e-02& 1.53& 4.09e-02& 1.57& ~ &8.50e-02  & 1.53 & 4.09e-02 & 1.62\\
				~& 80 & 2.35e-02& 1.86& 1.10e-02& 1.90& ~ &2.35e-02  & 1.86 & 1.10e-02 & 1.90\\
				~& 160 & 6.06e-03& 1.95& 2.79e-03& 1.98& ~ &6.06e-03  & 1.95 & 2.79e-03 & 1.98\\
				~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~\\
				2& 10 & 6.69e-02& --& 3.88e-02& -- & ~ &6.69e-02 & -- & 4.07e-02 & --\\
				~& 20 & 7.53e-03& 3.15& 4.90e-03& 2.99& ~& 7.53e-03 & 3.15 & 4.93e-03 & 3.04\\
				~& 40 & 9.24e-04& 3.03& 5.96e-04& 3.04& ~ &9.24e-04  & 3.03 & 5.96e-04 & 3.05\\
				~& 80 & 1.15e-04& 3.01& 7.21e-05& 3.05& ~ &1.15e-04  & 3.01 & 7.21e-05 & 3.05\\
				~& 160 & 1.43e-05& 3.00& 8.88e-06& 3.02& ~ &1.43e-05  & 3.00 & 8.88e-06 & 3.02\\
				~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~\\
				3& 10 & 3.34e-03& --& 1.68e-03& -- & ~ &3.34e-03 & -- & 1.65e-03 & --\\
				~& 20 & 2.34e-04& 3.83& 1.27e-04& 3.72& ~& 2.34e-04 & 3.83& 1.31e-04 & 3.66\\
				~& 40 & 1.53e-05& 3.94& 8.67e-06& 3.87& ~ &1.53e-05  & 3.94 & 8.67e-06 & 3.91\\
				~& 80 & 9.64e-07& 3.98& 5.50e-07& 3.98& ~ &9.64e-07  & 3.98 & 5.50e-07 & 3.98\\
				~& 160 & 6.06e-08& 3.99& 3.49e-08& 3.98& ~ &6.05e-08  & 3.99 & 3.50e-08 & 3.97\\
				\hline
			\end{tabular}
		}
	\end{center}
	\caption{\scriptsize{Errors and the corresponding convergence rates for $w$,  both real part $\mbox{Re}(w)$ and imaginary part $\mbox{Im}(w)$, in problem (\ref{defocusing}) when using $\mathcal{P}^q$ polynomials on a uniform mesh of $N(=80)$ cells.}}\label{w_defocusing}
\end{table}

%\begin{figure}[htbp]
%	\centering
%	\includegraphics[width=0.3\textwidth]{%ur_simu_1000_non}
%	\includegraphics[width=0.3\textwidth]{ui_simu_1000_non}
%	\includegraphics[width=0.3\textwidth]{conservation_mass_non}
%	\caption{We present the numerical and exact solutions for problem (\ref{defocusing}) obtained at $t = 1000$ with $\mathcal{P}^2$ polynomial on a uniform mesh of $N = 80$.  The error $M_h(t)-M_h(0)$ is maintained with a magnitude less than $2\times10^{-8}$ throughout to the end of the terminal time $T = 100$.
%	}\label{mass_defocusing}
%\end{figure}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.45\textwidth]{ur_non}
	\includegraphics[width=0.45\textwidth]{ui_non}\\
	\includegraphics[width=0.45\textwidth]{wr_non}
	\includegraphics[width=0.45\textwidth]{wi_non}
	\caption{Snapshots of numerical and exact solutions of problem (\ref{defocusing}) at time $t = 1000$, where the numerical solutions are obtained using $\mathcal{P}^2$ polynomial on a uniform mesh of $N = 80$.  These plots provide evident support for the proposed scheme on approximating the exact solution, even up to a significantly long time.
	}\label{uw_non}
\end{figure}

\subsection{Focusing nonlinear problem} 
 
 We now provide yet another set of experiments by considering nonlinear biharmonic Schr\"{o}dinger equations with an indefinite Hamiltonian.  To be specific, we test the problem
 \begin{equation*}
 iu_{t} = -u_{xxxx} - uF'(|u|^2), \ \ x\in(0,4\pi),\ \ t>0
 \end{equation*}
under three different nonlinear medium $F'(|u|^2)$:
 \[(a).\  F'(|u|^2) = -|u|^2, \ \ \ (b). \ F'(|u|^2) = -|u|^4,\ \ \ (c).\  F'(|u|^2) = -|u|^6.\]
Again, we study these problems with the same periodic boundary conditions and the following initial data as in Section \ref{defocusing_sec}
 \[u(x,0) = \cos x + i\sin x.\]
Finally, we also use the same spatial discretization as in Section \ref{liner_sec} such that the approximation order $q = 2$ and the number of cells $N = 80$.  Figure \ref{focusing} presents the temporal dynamics of the discrete solution $u_h$ under these different nonlinear medium.   From the top to the bottom we choose $F'(u) = -|u|^2$, $F'(u) = -|u|^4$ and $F'(u) = -|u|^6$, respectively. On the top panel, we evolve the solution until $T = 100$ and we find that $u_h$ is still stable up to $t \approx 30$, however, its dynamics revolve after then and a stable time-periodic profile develops afterward.  The middle panel solves the problem up to $T = 13.2$, while our numerics suggest that the solution blows up after that. On the bottom panel, we present the evolution of the solution until $T = 9.6$, and the solution also blows up after that. 
 
 \begin{figure}[htbp]
 	\centering
 	\includegraphics[width=0.45\textwidth]{ur_defocusing_2}
 	\includegraphics[width=0.45\textwidth]{ui_defocusing_2}\\
 		\includegraphics[width=0.45\textwidth]{ur_defocusing_4}
 	\includegraphics[width=0.45\textwidth]{ui_defocusing_4}\\
 		\includegraphics[width=0.45\textwidth]{ur_defocusing_6}
 	\includegraphics[width=0.45\textwidth]{ui_defocusing_6}
 	\caption{Spatial-temporal dynamics of the numerical solutions.  Here the non-linearity of the medium are chosen to be $F'(|u_h|^2) = -|u_h|^2, -|u_h|^4$ and $-|u_h|^6$ from the top to the bottom.  These plots readily indicate that the spatial-temporal dynamics of the problem heavily depend on the choice of the medium on one hand, and they are extremely complex which include oscillating, blow-up etc.  {\textbf{Top}}:  the real part of $u_h$ (left) and the imaginary part of $u_h$ (right) with $F'(|u_h|^2) = -|u_h|^2$. {\textbf{Middle}}: the real part of $u_h$ (left) and the imaginary part of $u_h$ (right) with $F'(|u_h|^2) = -|u_h|^4$. {\textbf{Bottom}}: the real part of $u_h$ (left) and the imaginary part of $u_h$ (right) with $F'(|u_h|^2) = -|u_h|^6$.
 	}\label{focusing}
 \end{figure}
 
 \subsection{Defocusing nonlinear problem in two dimensional space}
 

==> numerical_experiments.tex <==
%!TEX root = EDG_high_order.tex
\section{Numerical
Simulation}\label{sec_numerical}

In this section, we present numerical experiments to investigate the convergence of our method in an energy norm. The reason to use energy norm is that it is the starting point of the energy-based DG methods in establishing both stability and the rate of convergence as discussed in \cite{zhang2019energy}. We use a standard modal and in all cases we choose $\alpha_1 = \alpha_2 = \beta_1 = \beta_2 = \tau_1 = \tau_2 = 0.5$ for an upwind flux and choose $\alpha_1 = \alpha_2 = 0$ for an alternating flux. In addition, we denote the alternating flux by A.-flux, the central flux by C.-flux and the upwind flux by U.-flux.
\subsection{The spectral deferred correction (SDC) time-stepping algorithm} 

The energy-based DG method for (\ref{prob1}) is derived based on the first order in time system (\ref{system_1st}).  However, for PDEs containing higher-order spatial derivatives, classical stability analysis of explicit schemes requires an extremely small time step. This can be computationally inefficient. To alleviate this problem, we consider an SDC method. As those discussed in \cite{dutt2000spectral, hagstrom2007spectral, jacangelo2020galerkin}, the SDC methods are based on low order time-stepping methods, and then iteratively correct a defect equation to obtain a desired order of accuracy. Consider the following ODE system
\begin{equation*}
\left\{
\begin{aligned}
&y_t = Ay + F(t), \ \ t\in[0,T],\\
&y(0) = y_0,
\end{aligned}
\right.
\end{equation*}
where $y_0, y(t)\in \mathbb{C}^l$, $A\in M_{l\times l}(\mathbb{C})$ and $F: \mathbb{R} \rightarrow \mathbb{C}^l$. Suppose the time interval $[0,T]$ is partitioned into $N_t$ subintervals as $0 = t_0 < t_1 < \cdots < t_n < \cdots < \cdots < t_{N_t} = T$. Denote $\Delta t_n := t_{n+1} - t_n$ and $y_n := y(t_n)$, we then present the SDC time stepping algorithm used in the current work as follows :
\begin{itemize}
	\item Input: $y^1_{n,0} = y_n$, $t_n$, $t_{n+1}$, $m$, $J$,
	\item Compute $m$ Gauss-Radau points $\tau_i\in (t_n, t_{n+1}]$ and set $\tau_0 = t_n$, $k_i = \tau_i - \tau_{i-1}$,
	\item Compute the initial approximation (Backward Euler is used to be the base method here)
	\begin{itemize}
		\item For $i = 1, \cdots, m$
		\begin{itemize}
			\item [1.] Solve $y_{n,i}^1 = y_{n,i-1}^1 + k_i(Ay_{n,i}^1 + F(\tau_i))$,
		\end{itemize}
	\end{itemize}
	\item Compute successive corrections
	\begin{itemize}
		\item For $j = 1, \cdots, J$
		  \begin{itemize}
		 \item[--] Initialize $\epsilon_{n,0}^j = 0$, $\delta_{n,0}^j = 0$,
		\item[--] For $i = 1, \cdots, m$
		\begin{itemize}
		\item [1.] Compute $\epsilon_{n,i}^j = y_n - y_{n,i}^{j} + I_{n,0}^{n,i} (Ay^{j}(\tau)+F(\tau))$,
		\item [2.] Solve $\delta_{n,i}^{j} = \delta_{n,i-1}^j + k_iA\delta_{n,i}^j + (\epsilon_{n,i}^j - \epsilon_{n,i-1}^j)$
		\item[3.] Update $y_{n,i}^{j+1} = y_{n,i}^j + \delta_{n,i}^j$,
		\end{itemize}		
	\end{itemize}
\end{itemize}
\item Return $y^{J+1}_{n,m}$.
\end{itemize}
Here, $I_{n,0}^{n,i}(Ay^j(\tau) + F(\tau))$ is the integral of the $(m-1)$-th degree interpolating polynomial on the $m$ nodes $(\tau_i, Ay_{n,i}^j + F(\tau_i))_{i = 1}^m$ over the subinterval $[t_n, \tau_i]$, which is the numerical quadrature approximation of
\[\int_{t_n}^{\tau_i} Ay^j(\tau) + F(\tau) d\tau.\]
Here, we have omitted the details of standard derivations of the above SDC algorithm, one can refer to \cite{jacangelo2020galerkin} and reference therein for details. For the rest of numerical experiments, we set $m = 5$, $J = 15$ to ensure the convergence order in time ($2m-1$) is lager than the convergence order in space ($6th$ order in space).

\subsection{Numerical verification}\label{simulation1d}
In this section, we verify the theoretical convergence rates for the energy-based DG method derived in Section~\ref{sec_formula} for time-dependent Euler-Bernoulli beam equations. 

\subsubsection{Time dependent uniform Euler-Bernoulli beam}\label{sec_uniform}
 Consider the following problem
\begin{equation}\label{1d_simu_uniform}
u_{tt}= -u_{xxxx}, \ \ \ x\in(0,10), \ \ t > 0,
\end{equation}
with the simply supported boundary condition $u(0,t) = u(10,t) = 0,  u_{xx}(0,t) = u_{xx}(10,t) = 0$ and with initial data so that the exact solution is given by
\begin{equation}\label{sol_1d}
u(x,t) = \sin(0.6\pi x)\sin((0.6\pi)^2 t).
\end{equation}
The discretization is performed on a uniform mesh with DG element vertices $x_i =ih,i=0,\cdots,N,h=10/N$. The problem is evolved until the final time $T = 1$ with time step size $\mathcal{O}(h)$. We present results for the degree of the approximation space of $u^h$ being $q = (4, 5, 6)$ and $v^h$ being $s$ with $s =q$ or $q-1$ or $q-2$ or $q-3$ or $q-4$. 

The energy norm errors $\left(\|v - v^h\|_{L^2}^2 + |(u - u^h)|_{H^2}^2\right)^{1/2}$ are presented from Table \ref{1d_alternating_uniform} to Table \ref{1d_upwind_uniform} with the alternating flux, the central flux and the upwind flux, respectively. We observe:
\begin{itemize}
	\item[(a).] a suboptimal convergence rate $\bar{q}$ when $s \neq q-2$ for both the central flux and the alternating flux,
	\item[(b).] a suboptimal convergence rate $\bar{q}+\frac{1}{2}$ for most of cases when $s \neq q-2$ with the upwind flux. When $(q ,s) = (5,2), (5,5), (6,3)$, we note a suboptimal convergence $\bar{q}+1$,
	\item[(c).] an optimal convergence rate $q-1$ when $s = q-2$ for all three different fluxes.
\end{itemize}

\begin{table}
	\footnotesize
	\begin{center}
		\scalebox{0.9}{
			\begin{tabular}{|c|c|c| c c c c c|}
				
				\hline
				q&s&error&N=10&N=20&N=40&N=80&N=160\\
				\hline
				%\multirow{5}{*}{4}&{0}&\multirow{5}{*}{energy}&7.69e-00(--)&5.45e-00(0.50)&8.23e-00(-.60)&7.94e-00(0.05)&7.95e-00(-.00)\\
				\multirow{5}{*}{4}&{0}&\multirow{5}{*}{energy}&5.39e-00(--)&1.44e+01(-1.42)&7.92e-00(0.87)&7.94e-00(-.01)&7.95e-00(-.00)\\
				\cline{2-2}
				%~&{1}&~&9.41e-00(--)&1.22e+01(-.38)&1.27e+01(-.06)&1.28e+01(-.01)&1.29e+01(-.00)\\
				~&{1}&~&9.83e-00(--)&1.23e+01(-.32)&1.27e+01(-.05)&1.28e+01(-.01)&1.29e+01(-.00)\\
				\cline{2-2}
				%~&{2}&~&2.19e-00(--)&1.14e-00(0.95)&4.43e-01(1.36)&1.61e-01(1.46)&5.71e-02(1.49)\\
			~&{2}&~&{1.41e-00(--)}&{1.14e-01(3.64)}&{1.06e-02(3.43)}&{1.28e-03(3.05)}&{1.59e-04(3.01)}\\
				\cline{2-2}
				%~&{3}&~&4.94e-00(--)&2.52e-00(0.97)&1.25e-00(1.01)&6.19e-01(1.01)&3.08e-01(1.01)\\
				~&{3}&~&4.78e-00(--)&2.44e-00(0.97)&1.22e-00(0.99)&0.62e-01(1.00)&3.01e-01(1.00)\\
				\cline{2-2}
				%~&{4}&~&6.55e-00(--)&3.21e-00(1.03)&1.58e-00(1.02)&7.82e-01(1.01)&3.89e-01(1.01)\\
				~&{4}&~&6.26e-00(--)&3.11e-00(1.01)&1.55e-00(1.00)&7.75e-01(1.00)&3.88e-01(1.00)\\
				\hline
				%\multirow{5}{*}{5}&{1}&\multirow{5}{*}{energy}&1.50e+01(--)&1.52e+01(-.01)&1.50e+01(0.02)&1.50e+01(0.00)&1.50e+00(0.00)\\
				\multirow{5}{*}{5}&{1}&\multirow{5}{*}{energy}&1.52e+01(--)&1.50e+01(0.02)&1.50e+01(0.01)&1.50e+01(0.02)&1.49e+00(0.00)\\
				\cline{2-2}
				%~&{2}&~&2.00e-00(--)&6.87e-01(1.54)&2.81e-01(1.29)&1.32e-01(1.09)&6.46e-02(1.03)\\
				~&{2}&~&1.84e-00(--)&6.44e-01(1.51)&2.74e-01(1.23)&1.30e-01(1.07)&6.42e-02(1.02)\\
				\cline{2-2}
				%~&{3}&~&6.92e-01(--)&7.16e-02(3.27)&6.60e-03(3.44)&5.90e-04(3.49)&5.23e-05(3.50)\\
				~&{3}&~&{1.18e-01(--)}&{4.18e-03(4.81)}&{2.61e-04(4.00)}&{1.63e-05(4.00)}&{1.02e-06(4.00)}\\
				\cline{2-2}
				%~&{4}&~&1.12e-00(--)&2.70e-01(2.06)&6.73e-02(2.01)&1.68e-02(2.00)&4.21e-03(2.00)\\
				~&{4}&~&1.03e-00(--)&2.66e-01(1.95)&6.72e-02(1.99)&1.68e-02(2.00)&4.21e-03(2.00)\\
				\cline{2-2}
				%~&{5}&~&1.42e-00(--)&3.49e-01(2.02)&8.74e-02(2.00)&2.19e-02(2.00)&5.47e-03(2.00)\\
				~&{5}&~&1.35e-00(--)&3.47e-01(1.96)&8.73e-02(1.99)&2.19e-02(2.00)&5.47e-03(2.00)\\
				\hline
				%\multirow{5}{*}{6}&{2}&\multirow{5}{*}{energy }&3.19e-00(--)&9.59e-01(1.73)&3.69e-01(1.38)&1.68e-01(1.32)&8.20e-02(1.04)\\
				\multirow{5}{*}{6}&{2}&\multirow{5}{*}{energy }&2.97e-00(--)&9.13e-01(1.70)&3.61e-01(1.34)&1.67e-01(1.12)&8.15e-02(1.03)\\
				\cline{2-2}
				%~&{3}&~&2.65e-01(--)&5.67e-02(2.23)&1.40e-02(2.01)&3.51e-03(2.00)&8.78e-04(2.00)\\
				~&{3}&~&2.33e-01(--)&5.58e-02(2.06)&1.40e-02(1.99)&3.51e-03(2.00)&8.78e-04(2.00)\\
				\cline{2-2}
				%~&{4}&~&6.67e-02(--)&9.93e-03(2.75)&9.79e-04(3.34)&8.88e-05(3.46)&7.90e-06(3.49)\\
				~&{4}&~&{9.27e-03(--)}&{1.83e-04(5.66)}&{5.72e-06(5.00)}&{1.79e-07(5.00)}&{5.58e-09(5.00)}\\
				\cline{2-2}
				%~&{5}&~&1.64e-01(--)&2.13e-02(2.94)&2.63e-03(3.02)&3.23e-04(3.02)&4.00e-05(3.01)\\
				~&{5}&~&1.56e-01(--)&2.01e-02(2.96)&2.53e-03(2.99)&3.16e-04(3.00)&3.96e-05(3.00)\\
				\cline{2-2}
				%~&{6}&~&2.16e-01(--)&2.77e-02(2.96)&3.42e-03(3.02)&4.22e-04(3.02)&5.24e-05(3.01)\\
				~&{6}&~&2.06e-01(--)&2.64e-02(2.96)&3.32e-03(2.99)&4.16e-04(3.00)&5.20e-05(3.00)\\
				\hline
			\end{tabular}
		}
	\end{center}
\caption{\scriptsize{Energy norm errors $(\|v - v^h\|_{L^2}^2 + |u-u^h|_{H^2}^2)^{1/2}$ for problem 1 (\ref{1d_simu_uniform}) when the A.-flux is used. $q$ is the degree of
		$u^h$, $s$ is the degree of  $v^h$, and $N$ is the number of the cells with uniform mesh size $h = 10/N$.}}\label{1d_alternating_uniform}
\end{table}

\begin{table}
	\footnotesize
	\begin{center}
		\scalebox{0.91}{
			\begin{tabular}{|c|c|c| c c c c c|}
				
				\hline
				q&s&error&N=10&N=20&N=40&N=80&N=160\\
				\hline
				\multirow{5}{*}{4}&{0}&\multirow{5}{*}{energy}&1.22e+01(--)&1.49e+01(-.28)&3.84e-00(1.95)&1.36e+01(-1.82)&7.98e-00(0.77)\\
				\cline{2-2}
				~&{1}&~&1.10e+01(--)&1.28e+01(-.21)&1.57e+01(-.29)&1.23e+01(0.34)&8.93e+00(0.47)\\
				\cline{2-2}
				~&{2}&~&{1.14e-00(--)}&{1.66e-01(2.78)}&{2.33e-02(2.84)}&{2.99e-03(2.96)}&{3.76e-04(2.99)}\\
				\cline{2-2}
				~&{3}&~&8.00e-00(--)&4.08e-00(0.97)&2.05e-00(0.99)&1.03e-00(1.00)&5.15e-01(1.00)\\
				\cline{2-2}
				~&{4}&~&8.01e-00(--)&4.09e-00(0.97)&2.06e-00(0.99)&1.03e-00(1.01)&5.15e-01(1.00)\\
				\hline
				\multirow{5}{*}{5}&{1}&\multirow{5}{*}{energy}&4.52e-00(--)&5.38e-00(-.02)&6.82e-00(-.03)&7.17e-00(-.07)&7.25e-00(-.02)\\
				\cline{2-2}
				~&{2}&~&4.49e-00(--)&1.39e-00(1.69)&5.12e-01(1.44)&2.26e-01(1.18)&1.09e-02(1.05)\\
				\cline{2-2}
				~&{3}&~&{6.37e-02(--)}&{2.47e-03(4.69)}&{1.36e-04(4.18)}&{8.22e-06(4.05)}&{5.10e-07(4.01)}\\
				\cline{2-2}
				~&{4}&~&1.63e-00(--)&3.99e-01(2.04)&1.01e-01(1.99)&2.52e-02(1.99)&6.31e-03(2.00)\\
				\cline{2-2}
				~&{5}&~&1.72e-00(--)&4.12e-01(2.06)&1.02e-01(2.02)&2.53e-02(2.01)&6.32e-03(2.00)\\
				\hline
				\multirow{5}{*}{6}&{2}&\multirow{5}{*}{energy }&4.58e-00(--)&1.40e-00(1.71)&5.12e-01(1.45)&2.26e-01(1.18)&1.09e-01(1.05)\\
				\cline{2-2}
				~&{3}&~&3.89e-01(--)&8.41e-02(2.21)&2.10e-02(2.00)&5.26e-03(2.00)&1.32e-04(2.00)\\
				\cline{2-2}
				~&{4}&~&{4.08e-03(--)}&{1.67e-04(4.61)}&{5.82e-06(4.84)}&{1.87e-07(4.96)}&{6.90e-09(4.99)}\\
				\cline{2-2}
				~&{5}&~&2.66e-01(--)&3.67e-02(2.86)&4.73e-03(2.96)&5.96e-04(2.99)&7.47e-05(3.00)\\
				\cline{2-2}
				~&{6}&~&2.66e-01(--)&3.67e-02(2.86)&4.73e-03(2.96)&5.96e-04(2.99)&7.47e-05(3.00)\\
				\hline
			\end{tabular}
		}
	\end{center}
	\caption{\scriptsize{Energy norm errors $(\|v - v^h\|_{L^2}^2 + |u-u^h|_{H^2}^2)^{1/2}$ for problem 1 (\ref{1d_simu_uniform}) when the C.-flux is used. $q$ is the degree of
			$u^h$, $s$ is the degree of  $v^h$, and $N$ is the number of the cells with uniform mesh size $h = 10/N$.}}
\end{table}

\begin{table}
	\footnotesize
	\begin{center}
		\scalebox{0.95}{
			\begin{tabular}{|c|c|c| c c c c c|}
				
				\hline
				q&s&error&N=10&N=20&N=40&N=80&N=160\\
				\hline
				\multirow{5}{*}{4}&{0}&\multirow{5}{*}{energy}&8.08e-00(--)&8.13e-00(-.01)&8.11e-00(0.00)&8.07e-00(0.01)&8.02e-00(0.01)\\
				\cline{2-2}
				~&{1}&~&8.03e-00(--)&6.48e-00(0.31)&4.56e-00(0.51)&2.79e-00(0.71)&1.55e-00(0.85)\\
				\cline{2-2}
				~&{2}&~&2.06e-00(--)&2.33e-01(3.15)&2.58e-02(3.17)&3.07e-03(3.07)&3.79e-04(3.02)\\
				\cline{2-2}
				~&{3}&~&2.35e-00(--)&4.20e-01(2.49)&6.75e-02(2.64)&1.86e-02(1.86)&5.24e-03(1.83)\\
				\cline{2-2}
				~&{4}&~&3.51e-00(--)&1.29e-00(1.44)&4.70e-01(1.46)&1.68e-00(1.49)&5.95e-02(1.50)\\
				\hline
				\multirow{5}{*}{5}&{1}&\multirow{5}{*}{energy}&7.50e-00(--)&6.40e-00(0.23)&4.56e-00(0.49)&2.79e-00(0.71)&1.55e-00(0.85)\\
				\cline{2-2}
				~&{2}&~&3.06e-00(--)&9.64e-01(1.67)&2.51e-01(1.94)&5.92e-02(2.08)&1.41e-02(2.07)\\
				\cline{2-2}
				~&{3}&~&9.19e-02(--)&5.63e-03(4.03)&3.55e-04(3.99)&2.22e-05(4.00)&1.39e-06(4.00)\\
				\cline{2-2}
				~&{4}&~&3.18e-01(--)&1.01e-02(4.99)&2.65e-03(1.92)&4.73e-04(2.48)&6.78e-05(2.80)\\
				\cline{2-2}
				~&{5}&~&6.19e-01(--)&5.89e-02(3.39)&5.95e-03(3.31)&6.69e-04(3.15)&7.98e-05(3.07)\\
				\hline
				\multirow{5}{*}{6}&{2}&\multirow{5}{*}{energy }&3.10e-00(--)&8.90e-01(1.80)&2.40e-01(1.89)&6.47e-02(1.89)&1.83e-02(1.82)\\
				\cline{2-2}
				~&{3}&~&6.30e-01(--)&9.33e-02(2.76)&1.17e-02(2.99)&1.44e-03(3.02)&1.78e-04(3.01)\\
				\cline{2-2}
				~&{4}&~&6.29e-03(--)&1.92e-04(5.04)&6.04e-06(4.99)&1.89e-07(5.00)&5.91e-09(5.00)\\
				\cline{2-2}
				~&{5}&~&3.84e-02(--)&1.26e-03(4.94)&9.90e-05(3.67)&9.53e-06(3.38)&6.88e-07(3.79)\\
				\cline{2-2}
				~&{6}&~&9.12e-02(--)&1.08e-02(3.08)&1.03e-03(3.39)&9.28e-05(3.47)&8.22e-06(3.50)\\
				\hline
			\end{tabular}
		}
	\end{center}
	\caption{\scriptsize{Energy norm errors $(\|v - v^h\|_{L^2}^2 + |u-u^h|_{H^2}^2)^{1/2}$ for problem 1 (\ref{1d_simu_uniform}) when the U.-flux is used. $q$ is the degree of
			$u^h$, $s$ is the degree of  $v^h$, and $N$ is the number of the cells with uniform mesh size $h = 10/N$.}}\label{1d_upwind_uniform}
\end{table}


\begin{table}
	\footnotesize
	\begin{center}
		\scalebox{0.92}{
			\begin{tabular}{|c|c| c c c c c|}
				\hline
				$L^2$ error&flux&N=10&N=20&N=40&N=80&N=160\\
				\hline
				\multirow{3}{*}{$q = 2$}&{A.-flux}&7.60e-00(--)&8.52e-00(-.16)&8.76e-00(-.04)&8.82e-00(-.01)&8.83e-00(-.00)\\
				\cline{2-2}
				~&{C.-flux}&7.60e-00(--)&8.52e-00(-.16)&8.76e-00(-.04)&8.82e-00(-.01)&8.83e-00(-.00)\\
				\cline{2-2}
				~&{U.-flux}&5.20e-00(--)&6.44e-00(-.31)&7.43e-03(-.21)&8.07e-00(-.12)&8.43e-00(-.06)\\
				\hline
				\multirow{3}{*}{$q = 3$}&{A.-flux}&3.54e-00(--)&1.01e-00(1.82)&2.44e-01(2.05)&5.99e-02(2.02)&1.49e-02(2.01)\\
				\cline{2-2}
				~&{C.-flux}&2.35e-00(--)&5.26e-01(2.16)&1.24e-01(2.09)&2.99e-02(2.05)&7.41e-03(2.01)\\
				\cline{2-2}
				~&{U.-flux}&4.30e-00(--)&3.22e-00(0.42)&2.20e-00(0.55)&1.35e-00(0.71)&7.49e-00(0.84)\\
				\hline
				%\multirow{3}{*}{$q = 4$}&{A.-flux}&1.01e-00(--)&6.13e-01(0.72)&2.43e-01(1.34)&8.83e-02(1.46)&3.14e-02(1.49)\\
				\multirow{3}{*}{$q = 4$}&{A.-flux}&1.93e-01(--)&1.27e-02(3.92)&1.27e-03(3.32)&1.46e-04(3.13)&1.77e-05(3.04)\\
				\cline{2-2}
				~&{C.-flux}&2.04e-01(--)&2.86e-02(2.84)&3.00e-03(3.25)&3.14e-04(3.26)&3.63e-05(3.11)\\
				\cline{2-2}
				~&{U.-flux}&3.43e-01(--)&4.31e-02(2.99)&4.08e-03(3.40)&3.92e-04(3.38)&4.15e-05(3.24)\\
				\hline
				%\multirow{3}{*}{$q = 5$}&{A.-flux}&2.30e-01(--)&2.41e-02(3.25)&2.23e-03(3.44)&1.99e-04(3.48)&1.77e-05(3.50)\\
				\multirow{3}{*}{$q = 5$}&{A.-flux}&1.04e-02(--)&5.74e-04(4.17)&3.55e-05(4.02)&2.21e-06(4.00)&1.38e-07(4.00)\\
				\cline{2-2}
				~&{C.-flux}&4.12e-03(--)&1.05e-04(5.29)&3.49e-06(4.92)&1.11e-07(4.98)&3.48e-09(4.99)\\
				\cline{2-2}
				~&{U.-flux}&9.27e-03(--)&1.66e-04(5.80)&2.77e-06(5.91)&4.68e-08(5.89)&8.94e-10(5.71)\\
				\hline
				%\multirow{3}{*}{$q = 6$}&{A.-flux}&5.08e-02(--)&7.62e-03(2.74)&7.51e-04(3.34)&6.81e-05(3.46)&6.06e-06(3.49)\\
				\multirow{3}{*}{$q = 6$}&{A.-flux}&9.58e-04(--)&2.85e-05(5.07)&8.92e-07(5.00)&2.79e-08(5.00)&8.72e-10(5.00)\\
				\cline{2-2}
				~&{C.-flux}&1.76e-04(--)&1.33e-05(3.72)&5.42e-07(4.62)&1.82e-08(4.90)&5.78e-10(4.97)\\
				\cline{2-2}
				~&{U.-flux}&7.72e-04(--)&2.20e-05(5.13)&6.47e-07(5.09)&1.95e-08(5.05)&5.95e-10(5.03)\\
				\hline
				%\multirow{3}{*}{$q = 7$}&{A.-flux}&7.51e-05(--)&1.19e-06(5.97)&1.87e-08(6.00)&2.92e-10(6.00)&4.61e-12(6.00)\\
				%\cline{2-2}
				%~&{C.-flux}&1.47e-05(--)&1.57e-07(6.54)&1.31e-09(6.90)&1.04e-11(6.98)&8.72e-13(3.57)\\
				%\cline{2-2}
				%~&{U.-flux}&2.87e-06(--)&2.10e-08(7.09)&1.45e-10(7.18)&1.37e-12(6.71)&1.17e-12(0.23)\\
				%\hline
			\end{tabular}
		}
	\end{center}
\caption{\scriptsize{$L^2$ errors $\|u - u^h\|_{L^2}$ for problem 1 (\ref{1d_simu_uniform}) when $s = q-2$. $q$ is the degree of $u^h$, $s$ is the degree of $v^h$, and $N$ is the number of the cells with uniform mesh size $h = 10/N$.}}\label{1d_l2_uniform}
\end{table}

\begin{table}
	\footnotesize
	\begin{center}
		\scalebox{0.9}{
			\begin{tabular}{|c|c| c c c c c|}
				\hline
				$L^2$ error&flux&N=10&N=20&N=40&N=80&N=160\\
				\hline
				\multirow{3}{*}{$q = 2$}&{A.-flux}&1.36e+01(--)&1.48e+01(-.12)&1.51e+01(-.03)&1.52e+01(-.01)&1.52e+01(-.00)\\
				\cline{2-2}
				~&{C.-flux}&1.36e+01(--)&1.48e+01(-.12)&1.51e+01(-.03)&1.52e+01(-.01)&1.52e+01(-.00)\\
				\cline{2-2}
				~&{U.-flux}&9.75e-00(--)&1.12e+01(-.20)&1.27e+01(-.18)&1.38e+01(-.12)&1.44e+01(-.07)\\
				\hline
				\multirow{3}{*}{$q = 3$}&{A.-flux}&3.55e+00(--)&1.60e+00(1.15)&4.16e-01(1.95)&1.16e-02(1.84)&2.99e-02(1.96)\\
				\cline{2-2}
				~&{C.-flux}&1.20e+01(--)&1.82e-00(2.72)&2.58e-01(2.82)&5.67e-02(2.18)&1.37e-02(2.05)\\
				\cline{2-2}
				~&{U.-flux}&8.41e-00(--)&6.79e-00(0.31)&5.25e-00(0.37)&3.68e-00(0.51)&2.27e-00(0.70)\\
				\hline
				\multirow{3}{*}{$q = 4$}&{A.-flux}&9.48e-01(--)&1.05e-01(3.18)&9.40e-03(3.48)&1.17e-03(3.01)&1.45e-04(3.00)\\
				\cline{2-2}
				~&{C.-flux}&7.72e-01(--)&1.25e-01(2.63)&1.97e-02(2.66)&2.68e-03(2.88)&3.43e-04(2.97)\\
				\cline{2-2}
				~&{U.-flux}&1.50e-00(--)&1.67e-01(3.17)&2.10e-02(2.99)&2.69e-03(2.96)&3.41e-04(2.98)\\
				\hline
				\multirow{3}{*}{$q = 5$}&{A.-flux}&1.04e-01(--)&3.85e-03(4.75)&2.39e-04(4.01)&1.49e-05(4.00)&9.32e-07(4.00)\\
				\cline{2-2}
				~&{C.-flux}&4.78e-02(--)&2.25e-03(4.41)&1.25e-04(4.18)&7.54e-06(4.05)&4.67e-07(4.01)\\
				\cline{2-2}
				~&{U.-flux}&7.07e-02(--)&5.01e-03(3.82)&3.21e-04(3.96)&2.03e-05(3.99)&1.27e-06(3.99)\\
				\hline
				\multirow{3}{*}{$q = 6$}&{A.-flux}&8.08e-03(--)&1.68e-04(5.59)&5.24e-06(5.00)&1.64e-07(5.00)&5.12e-09(5.00)\\
				\cline{2-2}
				~&{C.-flux}&3.74e-03(--)&1.53e-04(4.61)&5.33e-06(4.84)&1.72e-07(4.96)&5.41e-09(4.99)\\
				\cline{2-2}
				~&{U.-flux}&5.63e-03(--)&1.74e-04(5.01)&5.51e-06(4.98)&1.73e-07(4.99)&5.41e-09(5.00)\\
				\hline
				%\multirow{3}{*}{$q = 7$}&{A.-flux}&4.44e-04(--)&6.30e-06(6.14)&9.86e-08(6.00)&1.54e-09(6.00)&2.46e-11(5.97)\\
				%\cline{2-2}
				%~&{C.-flux}&2.91e-04(--)&3.65e-06(6.32)&5.33e-08(6.10)&8.17e-10(6.03)&1.35e-11(5.92)\\
				%\cline{2-2}
				%~&{U.-flux}&3.66e-04(--)&5.70e-06(6.00)&8.98e-08(5.99)&1.41e-09(6.00)&2.27e-11(5.95)\\
				%\hline
			\end{tabular}
		}
	\end{center}
	\caption{\scriptsize{$L^2$ errors $\|v - v^h\|_{L^2}$ for problem 1 (\ref{1d_simu_uniform}) when $s = q-2$. $q$ is the degree of $u^h$, $s$ is the degree of $v^h$, and $N$ is the number of the cells with uniform mesh size $h = 10/N$.}}\label{1d_l2_vuniform}
\end{table}

\begin{table}
	\footnotesize
	\begin{center}
		\scalebox{0.92}{
			\begin{tabular}{|c|c| c c c c c|}
				\hline
				$L^2$ error&flux&N=10&N=20&N=40&N=80&N=160\\
				\hline
				\multirow{3}{*}{$q = 2$}&{A.-flux}&3.18e-00(--)&3.18e-00(0.00)&3.18e-00(0.00)&3.18e-00(0.00)&3.18e-00(0.00)\\
				\cline{2-2}
				~&{C.-flux}&3.18e-00(--)&3.18e-00(0.00)&3.18e-00(0.00)&3.18e-00(0.00)&3.18e-00(0.00)\\
				\cline{2-2}
				~&{U.-flux}&3.18e-00(--)&3.18e-00(0.00)&3.18e-00(0.00)&3.18e-00(0.00)&3.18e-00(0.00)\\
				\hline
				\multirow{3}{*}{$q = 3$}&{A.-flux}&9.62e-00(--)&3.63e-00(1.41)&9.49e-01(1.93)&2.40e-01(1.98)&6.02e-02(2.00)\\
				\cline{2-2}
				~&{C.-flux}&2.55e-00(--)&2.35e-00(0.12)&5.12e-01(2.20)&1.22e-01(2.07)&3.01e-02(2.02)\\
				\cline{2-2}
				~&{U.-flux}&3.77e-00(--)&4.12e-00(-.13)&3.42e-00(0.27)&2.22e-00(0.62)&1.22e-00(0.86)\\
				\hline
				\multirow{3}{*}{$q = 4$}&{A.-flux}&1.05e+00(--)&4.48e-02(4.55)&4.86e-03(3.20)&5.34e-04(3.19)&6.42e-05(3.06)\\
				\cline{2-2}
				~&{C.-flux}&8.38e-01(--)&1.10e-01(2.93)&1.25e-02(3.14)&1.33e-03(3.23)&1.55e-04(3.10)\\
				\cline{2-2}
				~&{U.-flux}&1.40e-00(--)&1.62e-01(3.11)&1.49e-02(3.44)&1.48e-03(3.34)&1.64e-04(3.17)\\
				\hline
				\multirow{3}{*}{$q = 5$}&{A.-flux}&5.56e-02(--)&1.63e-03(5.09)&1.04e-04(5.97)&6.51e-06(4.00)&4.07e-07(4.00)\\
				\cline{2-2}
				~&{C.-flux}&4.20e-02(--)&1.01e-03(5.39)&5.45e-05(4.21)&3.29e-06(4.05)&2.04e-07(4.01)\\
				\cline{2-2}
				~&{U.-flux}&5.86e-02(--)&2.57e-03(4.51)&1.51e-04(4.09)&9.18e-06(4.04)&5.65e-07(4.02)\\
				\hline
				\multirow{3}{*}{$q = 6$}&{A.-flux}&4.54e-03(--)&7.33e-05(5.95)&2.29e-06(5.00)&7.15e-08(5.00)&2.23e-09(5.00)\\
				\cline{2-2}
				~&{C.-flux}&1.61e-03(--)&6.68e-05(4.59)&2.33e-06(4.84)&7.49e-08(4.96)&2.36e-09(4.99)\\
				\cline{2-2}
				~&{U.-flux}&2.82e-03(--)&8.03e-05(5.13)&2.48e-06(5.02)&7.66e-08(5.01)&2.38e-09(5.01)\\
				\hline
				%\multirow{3}{*}{$q = 7$}&{A.-flux}&1.57e-04(--)&2.75e-06(5.84)&4.30e-08(6.00)&6.72e-10(6.00)&1.08e-11(5.96)\\
				%\cline{2-2}
				%~&{C.-flux}&1.23e-04(--)&1.59e-06(6.27)&2.32e-08(6.10)&3.57e-10(6.03)&6.43e-12(5.79)\\
				%\cline{2-2}
				%~&{U.-flux}&1.62e-04(--)&2.56e-05(5.98)&3.98e-07(6.01)&6.19e-08(6.01)&1.06e-10(5.87)\\
				%\hline
			\end{tabular}
		}
	\end{center}
	\caption{\scriptsize{$H^2$ semi-norm errors $|u - u^h|_{H^2}$ for problem 1 (\ref{1d_simu_uniform}) when $s = q-2$. $q$ is the degree of $u^h$, $s$ is the degree of $v^h$, and $N$ is the number of the cells with uniform mesh size $h = 10/N$.}}\label{1d_l2_d2uniform}
\end{table}


As discussed in previous works \cite{appelo2020energy, zhang2021energy}, the accuracy analysis of our scheme is based on an energy norm. For the numerical results of problem (\ref{1d_simu_uniform}), we observe that the performance of the $L^2$ error $(\|u - u^h\|_{L^2})$ is irregular. In most of the cases with $s \neq q-2$, we observe the same convergence rate for the $L^2$ errors and the energy norm errors, but the $L^2$ errors are much smaller than the energy norm errors. Here, we also present the $L^2$ errors for $u$, $\|u - u^h\|_{L^2}$, in Table \ref{1d_l2_uniform}, $L^2$ errors for $v$, $\|v - v^h\|_{L^2}$, in Table \ref{1d_l2_vuniform} and $H^2$ semi-norm errors for $u$, $|u - u^h|_{H^2}$ in Table \ref{1d_l2_d2uniform} when $q = s-2$ with three different numerical fluxes and $q = (2,3,4,5,6)$. We observe 
\begin{itemize}
 \item[(a).] $q = 2$ leads to zero convergence for all three different fluxes and all types of errors, which agrees with the theoretical findings,

\item[(b).] an optimal convergence are observed for the $L^2$ errors of $v$ and the $H^2$ semi-norm errors of $u$ when $q\geq 3$ and the alternating flux or the central flux is used,

\item[(c).] an optimal convergence are observed for the $L^2$ errors of $v$ and the $H^2$ semi-norm errors of $u$ when $q\geq 4$ and the upwind flux is used. When $q = 3$, we only obtain a first order convergence for the $L^2$ errors of $v$ and the $H^2$ semi-norm errors of $u$,

\item[(d).] the same order of  convergence are observed for the $L^2$ errors of $u$ compared with the $L^2$ errors of $v$ and the $H^2$ semi-norm errors of $u$ in most of cases. But the $L^2$ errors of $u$ are much smaller than the other two types of error. Specially, when $q = 5$ and the upwind flux is used, we observe an optimal convergence in the $L^2$ norm errors of $u$.

\end{itemize}

\begin{figure}[htbp]
	\centering
\includegraphics[width=0.45\textwidth]{discrete_energy}
\includegraphics[width=0.45\textwidth]{energy_conserve}
\caption{The plots of discrete energy for DG solutions of (\ref{1d_simu_uniform}) with three different numerical fluxes and approximation degrees $q = 5$, $s = 3$. For the left graph, the discrete energy for the alternating flux, the central flux, the upwind flux are presented. For the right graph, the discrete energy with the alternating flux and the central flux are displayed.
}\label{discrete_energy_p}
\end{figure}

Finally, for the uniform beam problem (\ref{1d_simu_uniform}), we present the numerical energy history of the proposed energy-based DG scheme in Figure \ref{discrete_energy_p} with the central flux, the alternating flux, and the upwind flux. In particular, we show the results for the case with $q = 5$ and $s = 3$ until the final time $T = 100$ with $N = 40$. We note that the magnitude of energy error for the conservative schemes, the alternating flux and the central flux, is smaller than $10^{-7}$, therefore our conservative schemes conserve the discrete energy. Even for the dissipating scheme, the upwind flux, the discrete energy is still conserved up to $2$ digits.

\subsubsection{Time dependent nonuniform Euler-Bernoulli beam} In this section, we consider the following model
\begin{equation}\label{1d_simu_prob2}
\frac{\partial^2 u}{\partial t^2} = -\frac{\partial^2 u}{\partial x^2}\left(D(x)\frac{\partial^2 u}{\partial x^2}\right) + f(x,t),\ \ x\in(0, 10), \ \ t > 0,
\end{equation}
where $D(x) = 1 + 0.1\cos(\pi x)$. For the simplicity of description, we use the same exact solution (\ref{sol_1d}) as in Section~\ref{sec_uniform} to determine the external forcing $f(x,t)$. Note that $\frac{dD}{dx} = 0$ at $x = 0, 10$, then the simply supported boundary condition is also satisfied. We also use the same discretization as those in Section~\ref{sec_uniform} and display the energy norm errors $\left(\|v - v^h\|_{L^2}^2 + |(u - u^h)|_{H^2}^2\right)^{1/2}$ in Table \ref{variable_tab}. We observe the same results as in the constant coefficients case: an optimal convergence for the central flux and the alternating flux when $q \geq 3$; an optimal convergence for the upwind flux when $q \geq 4$ and a suboptimal convergence $q-2$ when $q = 3$; when $q = 2$, again, we don't observe any convergence, since when $s = q - 2, q = 2$ the scheme is not defined.
\begin{table}
	\footnotesize
	\begin{center}
		\scalebox{0.87}{
			\begin{tabular}{|c|c| c c c c c|}
				\hline
				energy error&flux&N=10&N=20&N=40&N=80&N=160\\
				\hline
				\multirow{3}{*}{$q = 2$}&{A.-flux}&1.37e+01(--)&1.56e+01(-.19)&1.63e+01(-.06)&1.65e+01(-.02)&1.66e+01(-.00)\\
				\cline{2-2}
				~&{C.-flux}&1.38e+01(--)&1.58e+01(-.19)&1.64e+01(-.06)&1.65e+01(-.01)&1.66e+01(-.00)\\
				\cline{2-2}
				~&{U.-flux}&1.02e+01(--)&1.16e+01(-.19)&1.31e+01(-.17)&1.43e+01(-.13)&1.52e+01(-.09)\\
				\hline
				\multirow{3}{*}{$q = 3$}&{A.-flux}&9.90e-00(--)&3.80e-00(1.38)&1.03e-00(1.88)&2.65e-01(1.96)&6.67e-02(1.99)\\
				\cline{2-2}
				~&{C.-flux}&1.17e+01(--)&3.03e-00(1.95)&5.65e-01(2.42)&1.33e-01(2.08)&3.28e-02(2.02)\\
				\cline{2-2}
				~&{U.-flux}&9.13e-00(--)&7.83e-00(0.22)&6.14e-00(0.35)&4.21e-00(0.54)&2.53e-00(0.73)\\
				\hline
				%\multirow{3}{*}{$q = 4$}&{A.-flux}&2.31e-00(--)&1.22e-00(0.70)&4.63e-01(1.38)&1.64e-01(1.49)&5.78e-02(1.51)\\
				\multirow{3}{*}{$q = 4$}&{A.-flux}&1.44e-00(--)&1.02e-01(3.82)&1.15e-02(3.14)&1.28e-03(3.17)&1.59e-04(3.01)\\
				\cline{2-2}
				~&{C.-flux}&1.17e-00(--)&2.38e-01(2.30)&2.70e-02(3.14)&2.99e-03(3.17)&3.76e-04(2.99)\\
				\cline{2-2}
				~&{U.-flux}&2.05e-00(--)&2.31e-01(3.15)&2.57e-02(3.17)&3.07e-03(3.07)&3.80e-04(3.02)\\
				\hline
				%\multirow{3}{*}{$q = 5$}&{A.-flux}&7.33e-01(--)&7.75e-02(3.38)&6.92e-03(3.47)&6.04e-04(3.49)&5.29e-05(3.50)\\
				\multirow{3}{*}{$q = 5$}&{A.-flux}&1.11e-01(--)&4.48e-03(4.63)&2.81e-04(3.99)&1.63e-05(4.11)&1.02e-06(4.00)\\
				\cline{2-2}
				~&{C.-flux}&7.23e-02(--)&3.48e-03(4.38)&1.36e-04(4.68)&8.22e-06(4.05)&5.10e-07(4.01)\\
				\cline{2-2}
				~&{U.-flux}&9.64e-02(--)&5.73e-03(4.07)&3.55e-04(4.01)&2.22e-05(4.00)&1.39e-06(4.00)\\
				\hline
				%\multirow{3}{*}{$q = 6$}&{A.-flux}&7.07e-02(--)&1.07e-02(2.77)&1.02e-03(3.40)&9.10e-05(3.49)&8.00e-06(3.51)\\
				\multirow{3}{*}{$q = 6$}&{A.-flux}&1.01e-02(--)&2.24e-04(5.50)&5.51e-06(5.34)&1.79e-07(4.95)&5.58e-09(5.00)\\
				\cline{2-2}
				~&{C.-flux}&3.95e-03(--)&1.52e-04(4.70)&5.84e-06(4.71)&1.87e-07(4.96)&5.90e-09(5.00)\\
				\cline{2-2}
				~&{U.-flux}&6.10e-03(--)&1.77e-04(5.11)&6.03e-06(4.88)&1.89e-07(5.00)&5.91e-09(5.00)\\
				\hline
			\end{tabular}
		}
	\end{center}
	\caption{\scriptsize{Energy norm errors $(\|v - v^h\|_{L^2}^2 + |u-u^h|_{H^2}^2)^{1/2}$ for problem 1 (\ref{1d_simu_prob2}) when $s = q-2$. $q$ is the degree of $u^h$, $s$ is the degree of $v^h$, and $N$ is the number of the cells with uniform mesh size $h = 10/N$.}}\label{variable_tab}
\end{table}

The numerical solution $u^h$ and the errors $u - u^h$ at time $t = 100$ with three different numerical fluxes are shown in Figure \ref{numerical_sol}. From this
figure we observe our numerical results profiles match well. In addition, the errors show no severe error localized at the element boundaries and the central flux has the best performance (relatively smaller errors) for this problem.

\begin{figure}[htbp]
	\centering
\includegraphics[width=0.32\textwidth]{u_al}
\includegraphics[width=0.32\textwidth]{u_central}
\includegraphics[width=0.32\textwidth]{u_up}\\
\includegraphics[width=0.32\textwidth]{error_al}
\includegraphics[width=0.32\textwidth]{error_central}
\includegraphics[width=0.32\textwidth]{error_up}
\caption{Top panel: numerical solution and exact solution at $t = 100$ for problem (\ref{1d_simu_prob2}) when the approximation order $q = 5$ and $s = 3$ on a uniform mesh of $N = 40$. Bottom panel: error $u - u^h$ as a function of $x$. From the left to the right are the alternating flux, the central flux and the upwind flux.
}\label{numerical_sol}
\end{figure}








==> optimal_1d.tex <==
%!TEX root = EDG_high_order.tex
\subsection{Optimal convergence when $s = q-2$} \label{sec_one_dimension} In this section, we consider the problems in one dimension with $\mu, D$ are positive constants 
\begin{equation}\label{original_1d}
\frac{\partial^2 u}{\partial t^2} =  -D_\mu\frac{\partial^4 u}{\partial x^4},\ \ \ x\in (0,L), \ \ t\in(0,T),
\end{equation}
where $D_\mu = D/ \mu$. We further assume that the degree of approximation spaces satisfy $s = q - 2$. To avoid the units of the fluxes parameters in (\ref{numerical_flux}), we introduce the dimensionless variables
\[X = \frac{x}{L}, \ \ \Gamma = \frac{t}{T},\ \  \Lambda = \frac{D_\mu T^2}{L^4}.\]
Then we can use the proposed DG scheme in Section \ref{sec_formula} to solve the following dimensionless problem
\begin{equation}\label{improve1d_formula}
\frac{\partial^2 u}{\partial \Gamma^2} = -\Lambda \frac{\partial^4 u}{\partial X^4},\ \ X\in(0,1),\ \ \Gamma\in(0,1).
\end{equation}

For the rest of the analysis in this section, we will focus on the dimensionless problem (\ref{improve1d_formula}), the results can be easily generated to the original problem (\ref{original_1d}).  As mentioned in Remark \ref{remark2}, the order reduction comes from the numerical fluxes terms at the boundaries. To circumvent this issue, as discussed in \cite{meng2016optimal, appelo2015new}, we seek $\tilde{u}^h$, $\tilde{v}^h$ to make $\delta^{v,\ast}, \left(\frac{\partial \delta^v}{\partial X}\right)^\ast,  \left(\frac{\partial^2\delta^u}{\partial X^2}\right)^\ast,  \left(\frac{\partial^3 \delta^u}{\partial X^3}\right)^\ast$ vanish at both interelement and physical boundaries, that is,
\begin{equation}\label{flux1d}
\delta^{v,\ast} = \left(\frac{\partial \delta^v}{\partial X}\right)^\ast = \left(\frac{\partial^2\delta^u}{\partial X^2}\right)^\ast = \left(\frac{\partial^3 \delta^u}{\partial X^3}\right)^\ast = 0.
\end{equation}

To this end, by analyzing the general form of the numerical fluxes in (\ref{numerical_flux}), we find that (\ref{flux1d}) can be achieved by the following conditions
\begin{equation}\label{choice_1d}
\alpha_1(1-\alpha_1) = \beta_1\tau_1,\ \ \alpha_2(1-\alpha_2) = \beta_2\tau_2.
\end{equation}
Note that (\ref{choice_1d}) is satisfied by the alternating flux and the upwind flux, but not the central flux.
We now substitute (\ref{choice_1d}) into (\ref{numerical_flux}) and use (\ref{flux1d}), then rewrite the resulting equations into independent equations only containing data from one single element, $I_j := [X_{j-1}, X_j]$,
\begin{equation}\label{eq1d}
\left\{
\begin{aligned}
(1 -\alpha_1 + \tau_1)\delta^v - (\alpha_1+\beta_1)\frac{\partial^3 \delta^u}{\partial X^3} &= 0,\ \ X = X_{j-1}\\
(1 -\alpha_2 +\tau_2)\frac{\partial \delta^v}{\partial X} + (\alpha_2+\beta_2) \frac{\partial^2 \delta^u}{\partial X^2} &= 0,\ \ X = X_{j-1,}\\
(\alpha_1+\tau_1) \delta_v + (1 - \alpha_1+\beta_1)\frac{\partial^3\delta^u}{\partial X^3} & = 0,\ \ X = X_j,\\
(\alpha_2+\tau_2) \frac{\partial \delta^v}{\partial X} - (1 - \alpha_2+\beta_2)\frac{\partial^2\delta^u}{\partial X^2} & = 0,\ \ X = X_j.
\end{aligned}
\right.
\end{equation}
Here, we have assumed that the choices of $\alpha_1$ and $\alpha_2$ are consistent, that is, the values for $\alpha_1$ and $\alpha_2$ are the same for all elements.
  (\ref{eq1d}) gives us four independent equations on $I_j$ to determine $\tilde{u}^h$ and $\tilde{v}^h$. We are now ready to construct $\delta^v$ and $\delta^u$ by requiring %As for the physical boundaries, we use the left boundary $X = 0$ and the simple supported boundary condition $\frac{\partial^2 u}{\partial X^2} = v = 0$ as an example, the other cases are analogue. In this situation, we can easily obtain
%\[\delta_v^\ast =\left(\frac{\partial^2 \delta_u}{\partial X^2}\right)^\ast =  0 \ \ \mbox{at}\ \  X = 0\]
%by the definition (\ref{physical_flux}). Then we need to choose $\tilde{u}^h$ and $\tilde{v}^h$ such that 
%\[\left(\frac{\partial \delta_v}{\partial X}\right)^\ast  =\left(\frac{\partial^3 \delta_u}{\partial X^3}\right)^\ast = 0 \ \ \mbox{at}\ \ X = 0,\]
%To this end, based on (\ref{physical_flux}), we need
%\begin{equation}\label{boundary_flux}
%\frac{\partial \delta_v}{\partial X} -\eta_1\frac{\partial^3 \delta_u}{\partial X^3} = 0\ \ \mbox{and} \ \ -\eta_2\frac{\partial \delta_v}{\partial X} + \frac{\partial^3 \delta_u}{\partial X^3} = 0 \ \ \mbox{at}\ \ X = 0.
%\end{equation}
%Since $\eta_1\leq 0$ and $\eta_2\geq 0$ for the simple supported boundary condition as stated in Theorem \ref{them2}, it is clear that the system (\ref{boundary_flux}) is uniquely solvable with zeros solutions. In conclusion, for the first element, $[X_0, X_1]$, we impose equations
%\begin{equation}\label{first_element}
%\left\{
%\begin{aligned}
%\frac{\partial \delta_v}{\partial X} -\eta_1\frac{\partial^3 \delta_u}{\partial X^3} &= 0,\ \  X = X_0 = 0,\\
%-\eta_2\frac{\partial \delta_v}{\partial X} + \frac{\partial^3 \delta_u}{\partial X^3} &= 0 ,\  \ X = X_0 = 0,\\
%(\beta_1 + \alpha_1)\delta_v - (1 + \tau_1 - \alpha_1)\frac{\partial^3\delta_u}{\partial X^3} & = 0,\ \ X = X_1,\\
%(\beta_2 + \alpha_2)\frac{\partial \delta_v}{\partial X} - (1 + \tau_2 - \alpha_2)\frac{\partial^2\delta_u}{\partial X^2} & = 0,\ \ X = X_1.
%\end{aligned}
%\right.
%\end{equation}

Case I : $q \geq 4$
\begin{itemize}
	\item For all $\phi\in\mathcal{P}^{q-4}(I_j)$
	\begin{equation}\label{eq1d1}
	\int_{X_{j-1}}^{X_j} \phi\frac{\partial^2\delta^u}{\partial X^2}\ dX = \int_{X_{j-1}}^{X_j} \phi \delta^v\ dX = 0,
	\end{equation}
	\item Zero average error of $\frac{\partial u}{\partial X}$
	\begin{equation}\label{averaged1}
	\int_{X_{j-1}}^{X_j} \frac{\partial\delta^u}{\partial X}\ dX = 0,
	\end{equation}\label{average}
	\item Zero average error of $u$
	\begin{equation}\label{eq1d2}
	\int_{X_{j-1}}^{X_j} \delta^u \ dX = 0,
	\end{equation}
	\item Equations (\ref{eq1d}) holds. %or (\ref{first_element}) holds.
\end{itemize}

Case II : $q = 3$
\begin{itemize}
	\item Equations (\ref{eq1d}), (\ref{averaged1}) and (\ref{eq1d2}) hold.
\end{itemize}


To show the uniqueness of $\tilde{u}^h$ and $\tilde{v}^h$ defined above, we further assume that
\begin{equation}\label{choice_1d_1}
\alpha_1(1 - \alpha_1) =  \alpha_2(1-\alpha_2)  = 0, \beta_1=\beta_2=\tau_1=\tau_2 = 0,
\end{equation}
that is we have alternating fluxes.
Now we are ready to state the following lemma.
\begin{lemma}\label{lemma2}
	The function $(\tilde{u}^h, \tilde{v}^h)$ is uniquely defined by (\ref{eq1d1})--(\ref{eq1d2}) combining with $(\ref{eq1d})$ 
	and $(u,v) \in
	H^{q+1}(0,1) \times H^{q-1}(0,1)$ when $q\geq4$; uniquely defined by (\ref{averaged1})--(\ref{eq1d2}) combining with (\ref{eq1d}) and $(u,v)\in H^4(0,1)\times H^2(0,1)$ when $q = 3$. In addition, there exists a constant $C$ such that for $h = \max |X_j - X_{j-1}|$
	\begin{equation}\label{lemma2eq}
	\left|\left|\frac{\partial \delta^u}{\partial \Gamma}\right|\right|_{H^2(0,1)} + \left|\left|\frac{\partial \delta^v}{\partial \Gamma}\right|\right|_{L^2(0,1)} \leq Ch^{q-1}\left(\left|\frac{\partial u }{\partial \Gamma}\right|_{H^{q+1}(0,1)} + \left|\frac{\partial v }{\partial \Gamma}\right|_{H^{q-1}(0,1)}\right).
	\end{equation}
\end{lemma}
\begin{proof}
	Case I : $q \geq 4$,
	
	The dimensionality of the local polynomial space $\mathcal{P}^{q}(I_j) \times \mathcal{P}^{q-2}(I_j)$ is $2q$, which matches the number of linear equations. Suppose $u = v = 0$, then on $I_j$ condition (\ref{eq1d1}) and the boundary condition (\ref{eq1d}) together with the condition (\ref{choice_1d_1}) imply that $\frac{\partial^2\tilde{u}^h}{\partial X^2}=\tilde{v}^h = 0$. A subsequent use
	of condition (\ref{averaged1}) implies $\frac{\partial\tilde{u}^h}{\partial X} = 0$. Further combine with the condition (\ref{eq1d2}), we have $\tilde{u}^h = 0$. Thus $(\tilde{u}^h,\tilde{v}^h)$ is uniquely defined and preserves the space $\mathcal{P}^{q}(I_j) \times \mathcal{P}^{q-2}(I_j)$ . 
	
	Case II : $q = 3$,
	
	The dimensionality of the local polynomial space $\mathcal{P}^{3}(I_j) \times \mathcal{P}^{1}(I_j)$ is $6$, which matches the number of linear equations. Suppose $u = v = 0$, then  $\frac{\partial^3\tilde{u}^h}{\partial X^3}$ and $\frac{\partial\tilde{v}^h}{\partial X}$ are constants on $I_j$. The condition (\ref{eq1d}) together with the condition (\ref{choice_1d_1}) imply that $\frac{\partial^3\tilde{u}^h}{\partial X^3} = \frac{\partial\tilde{v}^h}{\partial X} = 0$ on $I_j$. Thus we have $\frac{\partial^2\tilde{u}^h}{\partial X^2}$ and $\tilde{v}^h$ are constants on $I_j$. Using the boundary condition (\ref{eq1d}) and the condition (\ref{choice_1d_1}) one more time, we obtain $\frac{\partial^2\tilde{u}^h}{\partial X^2} = \tilde{v}^h = 0$ on $I_j$. Thus $\frac{\partial \tilde{u}^h}{\partial X}$ is a constant on $I_j$. A subsequent use
	of condition (\ref{averaged1}) implies $\frac{\partial\tilde{u}^h}{\partial X} = 0$. Further combine with the condition (\ref{eq1d2}), we have $\tilde{u}^h = 0$. Thus $(\tilde{u}^h,\tilde{v}^h)$ is uniquely defined and preserves the space $\mathcal{P}^{3}(I_j) \times \mathcal{P}^{1}(I_j)$ . 
	
	To derive the error estimates we note that the polynomial approximation system commutes with time differentiation. Using the Bramble–Hilbert lemma, the result follows.
\end{proof}

We now state an optimal error estimate in an energy norm.
\begin{truth}
Suppose that $s = q - 2, q \geq 3$, $\mu, D$ are positive constants, and the solution satisfies $(u, v) \in H^{q+1}(0,1)\times H^{q-1}(0,1)$. Suppose further that the initial condition for the discontinuous Galerkin solution satisfies error estimates commensurate with Lemma \ref{lemma2}. Then there exists $C$ independent of $u, v$ and $h$ such that
\begin{equation*}
\|e^v\|_{L^2(0,1)}^2 + \| e^u_{xx}\|_{L^2(0,1)}^2 \!\leq\! Ch^{2(q-1)}\!\max_{\Gamma\leq 1} \left(\left|\frac{\partial u }{\partial \Gamma}\right|_{H^{q+1}(0,1)}^2 \!\!\!\!+ \left|\frac{\partial v }{\partial \Gamma}\right|_{H^{q-1}(0,1)}^2\!\right)\!.
\end{equation*}
\end{truth}
\begin{proof}
	Repeating the proof of Theorem \ref{thm3}. Using $(\tilde{u}^h,\tilde{v}^h)$ defined by (\ref{eq1d}), (\ref{eq1d1})–(\ref{eq1d2}), we get
\begin{multline}\label{A1d}
\mathcal{A}^h = \sum_{j=1}^n\int_{X_{j-1}}^{X_j} \Lambda\frac{\partial^2\tilde{e}^u}{\partial X^2}\frac{\partial^2}{\partial X^2}\left(\frac{\partial \delta^u}{\partial \Gamma}\right) - \Lambda\frac{\partial^4\tilde{e}^u}{\partial X^4}\delta^v + \mu\tilde{e}^v\frac{\partial\delta^v}{\partial \Gamma}  + \Lambda\frac{\partial^2\tilde{e}^v}{\partial X^2}\frac{\partial^2\delta^u}{\partial X^2} \ dX \\
- \sum_{j=1}^n \bigg[-\Lambda\frac{\partial^3\tilde{e}^u}{\partial X^3}\delta_v^\ast + \Lambda\frac{\partial\tilde{e}^u}{\partial X^2}\left(\frac{\partial\delta^v}{\partial X}\right)^\ast - \Lambda\tilde{e}^v\left(\frac{\partial^3\delta^u}{\partial X^3}\right)^\ast + \Lambda\frac{\partial\tilde{e}^v}{\partial X}\left(\frac{\partial^2\delta^u}{\partial X^2}\right)^\ast\bigg]_{X_{j-1}}^{X_j}\\
= \sum_{j=1}^n\int_{X_{j-1}}^{X_j} \Lambda\frac{\partial^2\tilde{e}^u}{\partial X^2}\frac{\partial^2}{\partial X^2}\left(\frac{\partial \delta^u}{\partial \Gamma}\right)  + \mu\tilde{e}^v\frac{\partial\delta_v}{\partial \Gamma}  \ dX.
\end{multline}
Combining (\ref{dedt1}), (\ref{A1d}), the estimate (\ref{lemma2eq}) in Lemma \ref{lemma2} and the nonpositive boundary contribution, we have
\begin{equation*}
\frac{d\mathcal{E}^h}{d\Gamma}\leq Ch^{q-1}\sqrt{\mathcal{E}^h}\left(\left|\frac{\partial u }{\partial \Gamma}\right|_{H^{q+1}(0,1)} + \left|\frac{\partial v }{\partial \Gamma}\right|_{H^{q-1}(0,1)}\right).
\end{equation*}
Integrating in time, then using the triangle inequality with the relations $e^v = \tilde{e}^v -\delta^v$, $e^u = \tilde{e}^u - \delta^u$ completes the proof.
\end{proof}
%\begin{remark}
%	If $D$ is not constant, then $\int_{x_{j-1}}^{x_j}\frac{\partial D}{\partial x}\frac{\partial^3\tilde{e}_u}{\partial x^3}\delta_v\ dx$ in (\ref{A_ibp}) will not vanish, instead, we have
%	\begin{equation*}
%	\frac{d\mathcal{E}^h}{d\Gamma}\leq C\sqrt{\mathcal{E}^h}\left[h^{q-1}\left(\left|\frac{\partial u }{\partial \Gamma}\right|_{H^{q+1}(0,1)} + \left|\frac{\partial v }{\partial \Gamma}\right|_{H^{q-1}(0,1)}\right) + h^{q-2}|v|_{H^{q-1}(0,1)}\right],
%	\end{equation*}
%	that is, the convergence order is one order lower than the optimal convergence order.
%\end{remark}
\begin{remark}\label{remark3}
	Note that we are only able to prove an optimal convergence in an energy norm with alternating fluxes in the current work, but we observe an optimal convergence for both the upwind flux and the central flux in the numerical experiments. It will be a future work to understand the mechanism behind this.
\end{remark}


==> optimal_1d_old.tex <==
%!TEX root = EDG_high_order.tex
\subsection{Optimal convergence in one dimension} \label{sec_one_dimension} In this section, we consider the problems in one dimension with $\mu, k, D$ are positive constants 
\begin{equation}\label{original_1d}
\frac{\partial^2 u}{\partial t^2} = -k_\mu u -D_\mu\frac{\partial^4 u}{\partial x^4},\ \ \ x\in (0,L), \ \ t\in(0,T),
\end{equation}
where $D_\mu = D/ \mu$, $k_\mu = k/\mu$. We further assume that the degree of approximation spaces satisfy $s = q - 2$. To avoid the units of the fluxes parameters in (\ref{numerical_flux}), we introduce the dimensionless variables
\[X = \frac{x}{L}, \ \ \Gamma = \frac{t}{T},\ \  \Lambda = \frac{D_\mu T^2}{L^4}, \ \ \kappa = k_\mu T^2.\]
Then we can use the proposed DG scheme in Section \ref{sec_formula} to solve the following dimensionless problem
\begin{equation}\label{improve1d_formula}
\frac{\partial^2 u}{\partial \Gamma^2} =-\kappa u -\Lambda \frac{\partial^4 u}{\partial X^4},\ \ X\in(0,1),\ \ \Gamma\in(0,1).
\end{equation}

For the rest of the analysis in this section, we will focus on the dimensionless problem (\ref{improve1d_formula}), the results can be easily generated to the original problem (\ref{original_1d}).  As mentioned in Remark \ref{remark2}, the order reduction comes from the numerical fluxes terms at the boundaries. To circumvent this issue, as discussed in \cite{meng2016optimal, appelo2015new}, we seek $\tilde{u}^h$, $\tilde{v}^h$ to make $\delta_v^\ast, \left(\frac{\partial \delta_v}{\partial X}\right)^\ast,  \left(\frac{\partial^2\delta_u}{\partial X^2}\right)^\ast,  \left(\frac{\partial^3 \delta_u}{\partial X^3}\right)^\ast$ vanish at both interelement and physical boundaries, that is,
\begin{equation}\label{flux1d}
\delta_v^\ast = \left(\frac{\partial \delta_v}{\partial X}\right)^\ast = \left(\frac{\partial^2\delta_u}{\partial X^2}\right)^\ast = \left(\frac{\partial^3 \delta_u}{\partial X^3}\right)^\ast = 0.
\end{equation}

%We first consider the interelement boundaries. 
To this end, by analyzing the general form of the numerical fluxes in (\ref{numerical_flux}), we find that (\ref{flux1d}) can be achieved by the following conditions
\begin{equation}\label{condition1d}
\alpha_1(1-\alpha_1) = \beta_1\tau_1, \ \ \alpha_2(1-\alpha_2) = \beta_2\tau_2.
\end{equation}
Note that (\ref{condition1d}) is satisfied by the alternating flux and the upwind flux, but not the central flux. We now substitute $(\ref{condition1d})$ into (\ref{numerical_flux}) and use (\ref{flux1d}), then rewrite (\ref{flux1d}) into independent equations only containing data from one single element, $I_j := [X_{j-1}, X_j]$,
\begin{equation}\label{eq1d}
\left\{
\begin{aligned}
(1 -\alpha_1 + \tau_1)\delta_v - (\alpha_1+\beta_1)\frac{\partial^3 \delta_u}{\partial X^3} &= 0,\ \ X = X_{j-1}\\
(1 -\alpha_2 + \tau_2)\frac{\partial \delta_v}{\partial X} + (\alpha_2 + \beta_2)\frac{\partial^2 \delta_u}{\partial X^2} &= 0,\ \ X = X_{j-1,}\\
(\alpha_1 + \tau_1)\delta_v + (1 - \alpha_1 + \beta_1)\frac{\partial^3\delta_u}{\partial X^3} & = 0,\ \ X = X_j,\\
(\alpha_2 + \tau_2)\frac{\partial \delta_v}{\partial X} - (1 - \alpha_2 + \beta_2)\frac{\partial^2\delta_u}{\partial X^2} & = 0,\ \ X = X_j.
\end{aligned}
\right.
\end{equation}
  This gives us four independent equations on $\Omega_j$ to determine $\tilde{u}^h$ and $\tilde{v}^h$. %As for the physical boundaries, we use the left boundary $X = 0$ and the simple supported boundary condition $\frac{\partial^2 u}{\partial X^2} = v = 0$ as an example, the other cases are analogue. In this situation, we can easily obtain
%\[\delta_v^\ast =\left(\frac{\partial^2 \delta_u}{\partial X^2}\right)^\ast =  0 \ \ \mbox{at}\ \  X = 0\]
%by the definition (\ref{physical_flux}). Then we need to choose $\tilde{u}^h$ and $\tilde{v}^h$ such that 
%\[\left(\frac{\partial \delta_v}{\partial X}\right)^\ast  =\left(\frac{\partial^3 \delta_u}{\partial X^3}\right)^\ast = 0 \ \ \mbox{at}\ \ X = 0,\]
%To this end, based on (\ref{physical_flux}), we need
%\begin{equation}\label{boundary_flux}
%\frac{\partial \delta_v}{\partial X} -\eta_1\frac{\partial^3 \delta_u}{\partial X^3} = 0\ \ \mbox{and} \ \ -\eta_2\frac{\partial \delta_v}{\partial X} + \frac{\partial^3 \delta_u}{\partial X^3} = 0 \ \ \mbox{at}\ \ X = 0.
%\end{equation}
%Since $\eta_1\leq 0$ and $\eta_2\geq 0$ for the simple supported boundary condition as stated in Theorem \ref{them2}, it is clear that the system (\ref{boundary_flux}) is uniquely solvable with zeros solutions. In conclusion, for the first element, $[X_0, X_1]$, we impose equations
%\begin{equation}\label{first_element}
%\left\{
%\begin{aligned}
%\frac{\partial \delta_v}{\partial X} -\eta_1\frac{\partial^3 \delta_u}{\partial X^3} &= 0,\ \  X = X_0 = 0,\\
%-\eta_2\frac{\partial \delta_v}{\partial X} + \frac{\partial^3 \delta_u}{\partial X^3} &= 0 ,\  \ X = X_0 = 0,\\
%(\beta_1 + \alpha_1)\delta_v - (1 + \tau_1 - \alpha_1)\frac{\partial^3\delta_u}{\partial X^3} & = 0,\ \ X = X_1,\\
%(\beta_2 + \alpha_2)\frac{\partial \delta_v}{\partial X} - (1 + \tau_2 - \alpha_2)\frac{\partial^2\delta_u}{\partial X^2} & = 0,\ \ X = X_1.
%\end{aligned}
%\right.
%\end{equation}

We are now ready to construst $\delta_v$ and $\delta_u$ by requiring
\begin{itemize}
	\item For all $\phi\in\Pi^{q-4}(I_j)$
	\begin{equation}\label{eq1d1}
	\int_{X_{j-1}}^{X_j} \phi\frac{d^3\delta_u}{dX^3}\ dX = \int_{X_{j-1}}^{X_j} \phi\frac{d\delta_v}{dX}\ dX = 0,
	\end{equation}
	\item Zero average error of $\frac{\partial u}{\partial X}$
	\begin{equation}\label{averaged1}
	\int_{X_{j-1}}^{X_j} \frac{d\delta_u}{dX}\ dX = 0,
	\end{equation}\label{average}
	\item Zero average error of $u$
	\begin{equation}\label{eq1d2}
	\int_{X_{j-1}}^{X_j} \delta_u \ dX = 0,
	\end{equation}
	\item Equations (\ref{eq1d}) holds. %or (\ref{first_element}) holds.
\end{itemize}
Then we have the following Lemma.
\begin{lemma}\label{lemma2}
	The function $(\tilde{u}^h, \tilde{v}^h)$ is uniquely defined by (\ref{eq1d1})--(\ref{eq1d2}) combining with $(\ref{eq1d})$ 
	%for the interior elements, $(\ref{first_element})$ for the boundary elements with 
	and $(u,v) \in
	H^{q+1}(0,1) \times H^{q-1}(0,1)$, then there exists a constant $C$ such that for $h = \max |X_j - X_{j-1}|$
	\begin{equation}\label{lemma2eq}
	\left|\left|\frac{\partial \delta_u}{\partial \Gamma}\right|\right|_{H^2(0,1)} + \left|\left|\frac{\partial \delta_v}{\partial \Gamma}\right|\right|_{L^2(0,1)} \leq Ch^{q-1}\left(\left|\frac{\partial u }{\partial \Gamma}\right|_{H^{q+1}(0,1)} + \left|\frac{\partial v }{\partial \Gamma}\right|_{H^{q-1}(0,1)}\right).
	\end{equation}
\end{lemma}
\begin{proof}
	The dimensionality of the local polynomial space $\Pi^{q}(I_j) \times \Pi^{q-2}(I_j)$ is $2q$, which matches the number of linear equations. Suppose $u = v = 0$, then on $I_j$ conditions (\ref{eq1d1}) imply that $\frac{d^3\tilde{u}^h}{dX^3}$ and $\frac{d\tilde{v}^h}{dX}$ are degree $(q-3)$ polynomials orthogonal in the standard $L^2$ inner product to all polynomials of lower degree. 
	%As such, any nonzero linear combination must have all $q-3$ zeros in the interior of the interval. 
	Then both $\frac{d^3\tilde{u}^h}{dX^3}$ and $\frac{d\tilde{v}^h}{dX}$ have all $q-3$ zeros in the interior of interval. Hence, using the boundary conditions, it is obvious that $\frac{d^3\tilde{u}^h}{dX^3} = \frac{d\tilde{v}^h}{dX} = 0$ on $I_j$. Then use the boundary condition one more time, we have $\frac{d^2\tilde{u}^h}{dX^2} = \tilde{v}^h = 0$ on $I_j$. A subsequent use
	of condition (\ref{averaged1}) implies $\frac{d\tilde{u}^h}{dX} = 0$. Further combine with the condition (\ref{eq1d2}), we have $\tilde{u}^h = 0$. Thus $(\tilde{u}^h,\tilde{v}^h)$ is uniquely defined and preserves the space $\Pi^{q}(I_j) \times \Pi^{q-2}(I_j)$ . To derive the error estimates we note that the polynomial approximation system commutes with time differentiation. Using the Bramble–Hilbert lemma, the result follows.
\end{proof}

We now state an optimal error estimate in an energy norm.
\begin{theorem}
Suppose that $d = 1, s = q - 2$, $\mu, k, D$ are positive constants, and the solution satisfies $(u, v) \in H^{q+1}(0,1)\times H^{q-1}(0,1)$. Suppose further that the initial condition for the discontinuous Galerkin solution satisfies error estimates commensurate with Lemma \ref{lemma2}. Then there exists $C$ independent of $u, v$ and $h$ such that
\begin{equation*}
\|e_v\|_{L^2(0,1)}^2 + \|e_u\|_{L^2(0,1)}^2+ \|\Delta e_u\|_{L^2(0,1)}^2 \!\leq\! Ch^{2(q-1)}\!\max_{\Gamma\leq 1} \left(\left|\frac{\partial u }{\partial \Gamma}\right|_{H^{q+1}(0,1)}^2 \!\!\!\!+ \left|\frac{\partial v }{\partial \Gamma}\right|_{H^{q-1}(0,1)}^2\!\right)\!.
\end{equation*}
\end{theorem}
\begin{proof}
	Repeating the proof of Theorem \ref{them3} using $(\tilde{u}^h,\tilde{v}^h)$ defined by (\ref{eq1d}), (\ref{eq1d1})–(\ref{eq1d2}), we get
\begin{multline}\label{A1d}
\mathcal{A}^h = \sum_j\int_{X_{j-1}}^{X_j} \Lambda\frac{\partial^2\tilde{e}_u}{\partial X^2}\frac{\partial^2}{\partial X^2}\left(\frac{\partial \delta_u}{\partial \Gamma}\right) - \Lambda\frac{\partial^4\tilde{e}_u}{\partial X^4}\delta_v + \mu\tilde{e}_v\frac{\partial\delta_v}{\partial \Gamma} + \kappa\tilde{e}_u\frac{\partial \delta_u}{\partial \Gamma} + \kappa\tilde{e}_u\delta_v \\+ \kappa\tilde{e}_v\delta_u + \Lambda\frac{\partial^2\tilde{e}_v}{\partial X^2}\frac{\partial^2\delta_u}{\partial X^2} \ dX 
- \sum_j \bigg[-\Lambda\frac{\partial^3\tilde{e}_u}{\partial X^3}\delta_v^\ast + \Lambda\frac{\partial\tilde{e}_u}{\partial X^2}\left(\frac{\partial\delta_v}{\partial X}\right)^\ast - \Lambda\tilde{e}_v\left(\frac{\partial^3\delta_u}{\partial X^3}\right)^\ast \\+ \Lambda\frac{\partial\tilde{e}_v}{\partial X}\left(\frac{\partial^2\delta_u}{\partial X^2}\right)^\ast\bigg]_{X_{j-1}}^{X_j}
= \sum_j\int_{X_{j-1}}^{X_j} \Lambda\frac{\partial^2\tilde{e}_u}{\partial X^2}\frac{\partial^2}{\partial X^2}\left(\frac{\partial \delta_u}{\partial \Gamma}\right)  \\+ \mu\tilde{e}_v\frac{\partial\delta_v}{\partial \Gamma}+ \kappa\tilde{e}_u\frac{\partial \delta_u}{\partial \Gamma} + \kappa\tilde{e}_u\delta_v + \kappa\tilde{e}_v\delta_u  \ dX.
\end{multline}
Combining (\ref{dedt1}), (\ref{A1d}), the estimate (\ref{lemma2eq}) in Lemma \ref{lemma2} and the nonpositive boundary contribution, we have
\begin{equation*}
\frac{d\mathcal{E}^h}{d\Gamma}\leq Ch^{q-1}\sqrt{\mathcal{E}^h}\left(\left|\frac{\partial u }{\partial \Gamma}\right|_{H^{q+1}(0,1)} + \left|\frac{\partial v }{\partial \Gamma}\right|_{H^{q-1}(0,1)}\right).
\end{equation*}
Integrating in time, then using the triangle inequality with the relations $e_v = \tilde{e}_v -\delta_v$, $e_u = \tilde{e}_u - \delta_u$ completes the proof.
\end{proof}
%\begin{remark}
%	If $D$ is not constant, then $\int_{x_{j-1}}^{x_j}\frac{\partial D}{\partial x}\frac{\partial^3\tilde{e}_u}{\partial x^3}\delta_v\ dx$ in (\ref{A_ibp}) will not vanish, instead, we have
%	\begin{equation*}
%	\frac{d\mathcal{E}^h}{d\Gamma}\leq C\sqrt{\mathcal{E}^h}\left[h^{q-1}\left(\left|\frac{\partial u }{\partial \Gamma}\right|_{H^{q+1}(0,1)} + \left|\frac{\partial v }{\partial \Gamma}\right|_{H^{q-1}(0,1)}\right) + h^{q-2}|v|_{H^{q-1}(0,1)}\right],
%	\end{equation*}
%	that is, the convergence order is one order lower than the optimal convergence order.
%\end{remark}
